Forming spectroscopic massive proto-binaries by disk fragmentation

The surroundings of massive protostars constitute an accretion disc which has numerically been shown to be subject to fragmentation and responsible for luminous accretion-driven outbursts. Moreover, it is suspected to produce close binary companions which will later strongly influence the star's future evolution in the Hertzsprung-Russel diagram. We present three-dimensional gravitation-radiation-hydrodynamic numerical simulations of 100 Mo pre-stellar cores. We find that accretion discs of young massive stars violently fragment without preventing the (highly variable) accretion of gaseous clumps onto the protostars. While acquiring the characteristics of a nascent low-mass companion, some disc fragments migrate onto the central massive protostar with dynamical properties showing that its final Keplerian orbit is close enough to constitute a close massive proto-binary system, having a young high-mass and a low-mass component. We conclude on the viability of the disc fragmentation channel for the formation of such short-period binaries, and that both processes -close massive binary formation and accretion bursts- may happen at the same time. FU-Orionis-type bursts, such as observed in the young high-mass star S255IR-NIRS3, may not only indicate ongoing disc fragmentation, but also be considered as a tracer for the formation of close massive binaries - progenitors of the subsequent massive spectroscopic binaries - once the high-mass component of the system will enter the main-sequence phase of its evolution. Finally, we investigate the ALMA-observability of the disc fragments.

==> grid <==
@ARTICLE{Krumholz_sci_2009,
   author = {{Krumholz}, M.~R. and {Klein}, R.~I. and {McKee}, C.~F. and 
	{Offner}, S.~S.~R. and {Cunningham}, A.~J.},
    title = "{The Formation of Massive Star Systems by Accretion}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {0901.3157},
 primaryClass = "astro-ph.SR",
     year = 2009,
    month = feb,
   volume = 323,
    pages = {754},
      doi = {10.1126/science.1165857},
   adsurl = {http://adsabs.harvard.edu/abs/2009Sci...323..754K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ARA&A..45..339B,
   author = {{Bergin}, E.~A. and {Tafalla}, M.},
    title = "{Cold Dark Clouds: The Initial Conditions for Star Formation}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0705.3765},
     year = 2007,
    month = sep,
   volume = 45,
    pages = {339-396},
      doi = {10.1146/annurev.astro.45.071206.100404},
   adsurl = {http://adsabs.harvard.edu/abs/2007ARA%26A..45..339B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bonnell_mnras_362_2005,
   author = {{Bonnell}, I.~A. and {Bate}, M.~R.},
    title = "{Binary systems and stellar mergers in massive star formation}",
  journal = {\mnras},
   eprint = {astro-ph/0506689},
 keywords = {binaries: general, stars: formation, stars: luminosity function, mass function, open clusters and associations: general},
     year = 2005,
    month = sep,
   volume = 362,
    pages = {915-920},
      doi = {10.1111/j.1365-2966.2005.09360.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362..915B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ARA&A..37..311E,
   author = {{Evans}, II, N.~J.},
    title = "{Physical Conditions in Regions of Star Formation}",
  journal = {\araa},
   eprint = {astro-ph/9905050},
 keywords = {STAR FORMATION, INTERSTELLAR MOLECULES, MOLECULAR CLOUDS},
     year = 1999,
   volume = 37,
    pages = {311-362},
      doi = {10.1146/annurev.astro.37.1.311},
   adsurl = {http://adsabs.harvard.edu/abs/1999ARA%26A..37..311E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bae_apj_795_2014,
   author = {{Bae}, J. and {Hartmann}, L. and {Zhu}, Z. and {Nelson}, R.~P.
	},
    title = "{Accretion Outbursts in Self-gravitating Protoplanetary Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1409.3891},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, stars: formation, stars: pre-main sequence},
     year = 2014,
    month = nov,
   volume = 795,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/795/1/61},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014ApJ...795...61B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...777...46L,
   author = {{Le{\~a}o}, M.~R.~M. and {de Gouveia Dal Pino}, E.~M. and {Santos-Lima}, R. and 
	{Lazarian}, A.},
    title = "{The Collapse of Turbulent Cores and Reconnection Diffusion}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1209.1846},
 primaryClass = "astro-ph.HE",
 keywords = {diffusion, ISM: magnetic fields, magnetohydrodynamics: MHD, stars: formation, turbulence },
     year = 2013,
    month = nov,
   volume = 777,
      eid = {46},
    pages = {46},
      doi = {10.1088/0004-637X/777/1/46},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...777...46L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...668.1064E,
   author = {{Elmegreen}, B.~G.},
    title = "{On the Rapid Collapse and Evolution of Molecular Clouds}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0707.2252},
 keywords = {ISM: Magnetic Fields, ISM: Molecules, Stars: Formation},
     year = 2007,
    month = oct,
   volume = 668,
    pages = {1064-1082},
      doi = {10.1086/521327},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...668.1064E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998MNRAS.298...93B,
   author = {{Bonnell}, I.~A. and {Bate}, M.~R. and {Zinnecker}, H.},
    title = "{On the formation of massive stars}",
  journal = {\mnras},
   eprint = {astro-ph/9802332},
 keywords = {BINARIES: GENERAL, STARS: FORMATION, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, OPEN CLUSTERS AND ASSOCIATIONS: GENERAL},
     year = 1998,
    month = jul,
   volume = 298,
    pages = {93-102},
      doi = {10.1046/j.1365-8711.1998.01590.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.298...93B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...569..846Y,
   author = {{Yorke}, H.~W. and {Sonnhalter}, C.},
    title = "{On the Formation of Massive Stars}",
  journal = {\apj},
   eprint = {astro-ph/0201041},
 keywords = {Stars: Circumstellar Matter, Hydrodynamics, Radiative Transfer, Stars: Formation, Stars: Mass Loss},
     year = 2002,
    month = apr,
   volume = 569,
    pages = {846-862},
      doi = {10.1086/339264},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...569..846Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_apj_832_2016,
   author = {{Kuiper}, R. and {Turner}, N.~J. and {Yorke}, H.~W.},
    title = "{Protostellar Outflows and Radiative Feedback from Massive Stars. II. Feedback, Star-formation Efficiency, and Outflow Broadening}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1609.05208},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, methods: numerical, stars: formation, stars: jets, stars: massive, stars: winds, outflows },
     year = 2016,
    month = nov,
   volume = 832,
      eid = {40},
    pages = {40},
      doi = {10.3847/0004-637X/832/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...832...40K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170202153S,
   author = {{Sana}, H. and {Ramirez-Tannus}, M. and {de Koter}, A. and {Kaper}, L. and 
	{Tramper}, F. and {Bik}, A.},
    title = "{A dearth of short-period massive binaries in the young massive star forming region M17: Evidence for a large orbital separation at birth?}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1702.02153},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2017,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170202153S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJS..213...34K,
   author = {{Kobulnicky}, H.~A. and {Kiminki}, D.~C. and {Lundquist}, M.~J. and 
	{Burke}, J. and {Chapman}, J. and {Keller}, E. and {Lester}, K. and 
	{Rolen}, E.~K. and {Topel}, E. and {Bhattacharjee}, A. and {Smullen}, R.~A. and 
	{Vargas {\'A}lvarez}, C.~A. and {Runnoe}, J.~C. and {Dale}, D.~A. and 
	{Brotherton}, M.~M.},
    title = "{Toward Complete Statistics of Massive Binary Stars: Penultimate Results from the Cygnus OB2 Radial Velocity Survey}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1406.6655},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: close, binaries: general, binaries: spectroscopic, stars: early-type, stars: kinematics and dynamics, stars: massive, techniques: radial velocities},
     year = 2014,
    month = aug,
   volume = 213,
      eid = {34},
    pages = {34},
      doi = {10.1088/0067-0049/213/2/34},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..213...34K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{boss_apj_836_2017,
   author = {{Boss}, A.~P.},
    title = "{The Effect of Protoplanetary Disk Cooling Times on the Formation of Gas Giant Planets by Gravitational Instability}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1701.04892},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, planets and satellites: formation, protoplanetary disks },
     year = 2017,
    month = feb,
   volume = 836,
      eid = {53},
    pages = {53},
      doi = {10.3847/1538-4357/836/1/53},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...836...53B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meru_mnras_427_2012,
   author = {{Meru}, F. and {Bate}, M.~R.},
    title = "{On the convergence of the critical cooling time-scale for the fragmentation of self-gravitating discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.1107},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, gravitation, hydrodynamics, instabilities, planets and satellites: formation, protoplanetary discs},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {2022-2046},
      doi = {10.1111/j.1365-2966.2012.22035.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427.2022M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.411L...1M,
   author = {{Meru}, F. and {Bate}, M.~R.},
    title = "{Non-convergence of the critical cooling time-scale for fragmentation of self-gravitating discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1011.5896},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, gravitation, hydrodynamics, instabilities, planets and satellites: formation, protoplanetary discs},
     year = 2011,
    month = feb,
   volume = 411,
    pages = {L1-L5},
      doi = {10.1111/j.1745-3933.2010.00978.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.411L...1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...550A..27M,
   author = {{Mahy}, L. and {Rauw}, G. and {De Becker}, M. and {Eenens}, P. and 
	{Flores}, C.~A.},
    title = "{A spectroscopic investigation of the O-type star population in four Cygnus OB associations. I. Determination of the binary fraction}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1301.0500},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, binaries: spectroscopic, open clusters and associations: individual: Cygnus OB1, open clusters and associations: individual: Cygnus OB3, open clusters and associations: individual: Cygnus OB8, open clusters and associations: individual: Cygnus OB9},
     year = 2013,
    month = feb,
   volume = 550,
      eid = {A27},
    pages = {A27},
      doi = {10.1051/0004-6361/201219425},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...550A..27M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{furuya_apj_673_2008,
   author = {{Furuya}, R.~S. and {Cesaroni}, R. and {Takahashi}, S. and {Codella}, C. and 
	{Momose}, M. and {Beltr{\'a}n}, M.~T.},
    title = "{Candidate Rotating Toroids around High-Mass (Proto)Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0710.0029},
 keywords = {ISM: evolution, ISM: individual: G16.59{\ndash}0.05 G23.01{\ndash}0.41 G28.87+0.07, radio continuum: ISM, stars: early-type},
     year = 2008,
    month = jan,
   volume = 673,
      eid = {363-381},
    pages = {363-381},
      doi = {10.1086/523834},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673..363F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{campbell_apj_282_1984,
   author = {{Campbell}, B.},
    title = "{VLA observations of collimated outflow at NGC 7538 IRS 1}",
  journal = {\apjl},
 keywords = {Collimation, Nebulae, Radio Sources (Astronomy), Stellar Evolution, Astronomical Maps, Gas Flow, Radio Interferometers},
     year = 1984,
    month = jul,
   volume = 282,
    pages = {L27-L30},
      doi = {10.1086/184297},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...282L..27C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJS..143..469M,
   author = {{Mueller}, K.~E. and {Shirley}, Y.~L. and {Evans}, II, N.~J. and 
	{Jacobson}, H.~R.},
    title = "{The Physical Conditions for Massive Star Formation: Dust Continuum Maps and Modeling}",
  journal = {\apjs},
   eprint = {astro-ph/0207322},
 keywords = {ISM: Dust, Extinction, Stars: Early-Type, Stars: Formation, Submillimeter},
     year = 2002,
    month = dec,
   volume = 143,
    pages = {469-497},
      doi = {10.1086/342881},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJS..143..469M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2000ApJ...537..283V,
   author = {{van der Tak}, F.~F.~S. and {van Dishoeck}, E.~F. and {Evans}, II, N.~J. and 
	{Blake}, G.~A.},
    title = "{Structure and Evolution of the Envelopes of Deeply Embedded Massive Young Stars}",
  journal = {\apj},
   eprint = {astro-ph/0001527},
 keywords = {Stars: Circumstellar Matter, ISM: Dust, Extinction, ISM: Jets and Outflows, ISM: Molecules, Stars: Formation, Submillimeter},
     year = 2000,
    month = jul,
   volume = 537,
    pages = {283-303},
      doi = {10.1086/309011},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...537..283V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{francohernandez_apj_604_2004,
   author = {{Franco-Hern{\'a}ndez}, R. and {Rodr{\'{\i}}guez}, L.~F.},
    title = "{Time Variation in the Radio Flux Density from the Bipolar Ultracompact H II Region NGC 7538 IRS 1}",
  journal = {\apjl},
   eprint = {astro-ph/0402467},
 keywords = {ISM: H II Regions, ISM: Individual: NGC Number: NGC 7538 IRS 1, Stars: Pre-Main-Sequence},
     year = 2004,
    month = apr,
   volume = 604,
    pages = {L105-L108},
      doi = {10.1086/386282},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...604L.105F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{krumholz_apj_665_2007,
   author = {{Krumholz}, M.~R. and {Klein}, R.~I. and {McKee}, C.~F.},
    title = "{Molecular Line Emission from Massive Protostellar Disks: Predictions for ALMA and EVLA}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0705.0536},
 keywords = {Accretion, Accretion Disks, ISM: Clouds, Methods: Numerical, Radiative Transfer, Stars: Formation},
     year = 2007,
    month = aug,
   volume = 665,
    pages = {478-491},
      doi = {10.1086/519305},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665..478K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{purser_mnras_460_2016,
   author = {{Purser}, S.~J.~D. and {Lumsden}, S.~L. and {Hoare}, M.~G. and 
	{Urquhart}, J.~S. and {Cunningham}, N. and {Purcell}, C.~R. and 
	{Brooks}, K.~J. and {Garay}, G. and {G{\'u}zman}, A.~E. and 
	{Voronkov}, M.~A.},
    title = "{A search for ionized jets towards massive young stellar objects}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1605.01200},
 keywords = {stars: evolution, stars: formation, stars: massive, stars: protostars, ISM: jets and outflows, radio continuum: ISM},
     year = 2016,
    month = jul,
   volume = 460,
    pages = {1039-1053},
      doi = {10.1093/mnras/stw1027},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.460.1039P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{tanaka_apj_835_2017,
   author = {{Tanaka}, K.~E.~I. and {Tan}, J.~C. and {Zhang}, Y.},
    title = "{The Impact of Feedback During Massive Star Formation by Core Accretion}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1610.08856},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, stars: formation, stars: luminosity function, mass function, stars: massive, stars: Population III, stars: winds, outflows},
     year = 2017,
    month = jan,
   volume = 835,
      eid = {32},
    pages = {32},
      doi = {10.3847/1538-4357/835/1/32},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835...32T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170607444T,
   author = {{Tanaka}, K.~E.~I. and {Tan}, J.~C. and {Staff}, J.~E. and {Zhang}, Y.
	},
    title = "{Outflow-Confined HII regions. II. The Early Break-Out Phase}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1706.07444},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170607444T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170108637H,
   author = {{Hunter}, T.~R. and {Brogan}, C.~L. and {MacLeod}, G. and {Cyganowski}, C.~J. and 
	{Chandler}, C.~J. and {Chibueze}, J.~O. and {Friesen}, R. and 
	{Indebetouw}, R. and {Thesner}, C. and {Young}, K.~H.},
    title = "{An extraordinary outburst in the massive protostellar system NGC6334I-MM1: quadrupling of the millimeter continuum}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1701.08637},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170108637H},
  a

@ARTICLE{sanna_aa_596_2016,
   author = {{Sanna}, A. and {Moscadelli}, L. and {Cesaroni}, R. and {Caratti o Garatti}, A. and 
	{Goddi}, C. and {Carrasco-Gonz{\'a}lez}, C.},
    title = "{Momentum-driven outflow emission from an O-type YSO. Comparing the radio jet with the molecular outflow}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1611.00408},
 keywords = {radio continuum: stars, ISM: jets and outflows, stars: formation, stars: individual: G023.01-00.41},
     year = 2016,
    month = nov,
   volume = 596,
      eid = {L2},
    pages = {L2},
      doi = {10.1051/0004-6361/201629544},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...596L...2S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{flaig_mnras_420_2012,
   author = {{Flaig}, M. and {Ruoff}, P. and {Kley}, W. and {Kissmann}, R.
	},
    title = "{Global structure of magnetorotationally turbulent protoplanetary discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1111.5497},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, magnetic fields, MHD, radiative transfer, turbulence, protoplanetary discs},
     year = 2012,
    month = mar,
   volume = 420,
    pages = {2419-2428},
      doi = {10.1111/j.1365-2966.2011.20207.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012MNRAS.420.2419F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nelson_mnras_435_2013,
   author = {{Nelson}, R.~P. and {Gressel}, O. and {Umurhan}, O.~M.},
    title = "{Linear and non-linear evolution of the vertical shear instability in accretion discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.2753},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, hydrodynamics, instabilities, methods: analytical, methods: numerical, protoplanetary discs},
     year = 2013,
    month = nov,
   volume = 435,
    pages = {2610-2632},
      doi = {10.1093/mnras/stt1475},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013MNRAS.435.2610N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_apj_768_2013,
   author = {{Vorobyov}, E.~I. and {DeSouza}, A.~L. and {Basu}, S.},
    title = "{The Burst Mode of Accretion in Primordial Protostars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1303.3622},
 keywords = {accretion, accretion disks, cosmology: theory, hydrodynamics, stars: formation},
     year = 2013,
    month = may,
   volume = 768,
      eid = {131},
    pages = {131},
      doi = {10.1088/0004-637X/768/2/131},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768..131V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_aa_590_2016,
   author = {{Vorobyov}, E.~I.},
    title = "{Ejection of gaseous clumps from gravitationally unstable protostellar disks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1603.07761},
 primaryClass = "astro-ph.SR",
 keywords = {stars: protostars, circumstellar matter, brown dwarfs, hydrodynamics},
     year = 2016,
    month = may,
   volume = 590,
      eid = {A115},
    pages = {A115},
      doi = {10.1051/0004-6361/201628102},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...590A.115V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sakurai_mnras_549_2016,
   author = {{Sakurai}, Y. and {Vorobyov}, E.~I. and {Hosokawa}, T. and {Yoshida}, N. and 
	{Omukai}, K. and {Yorke}, H.~W.},
    title = "{Supermassive star formation via episodic accretion: protostellar disc instability and radiative feedback efficiency}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.06080},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, galaxies: formation, cosmology: theory, early Universe},
     year = 2016,
    month = jun,
   volume = 459,
    pages = {1137-1145},
      doi = {10.1093/mnras/stw637},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.459.1137S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_apj_719_2010,
   author = {{Vorobyov}, E.~I. and {Basu}, S.},
    title = "{The Burst Mode of Accretion and Disk Fragmentation in the Early Embedded Stages of Star Formation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1007.2993},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, ISM: clouds, stars: formation},
     year = 2010,
    month = aug,
   volume = 719,
    pages = {1896-1911},
      doi = {10.1088/0004-637X/719/2/1896},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...719.1896V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{machida_mnras_448_2015,
   author = {{Machida}, M.~N. and {Nakamura}, T.},
    title = "{Accretion phase of star formation in clouds with different metallicities}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1502.01808},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, binaries: general, stars: formation, stars: protostars, cosmology: theory, early Universe},
     year = 2015,
    month = apr,
   volume = 448,
    pages = {1405-1429},
      doi = {10.1093/mnras/stu2633},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.448.1405M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{machida_apj_729_2011,
   author = {{Machida}, M.~N. and {Inutsuka}, S.-i. and {Matsumoto}, T.},
    title = "{Recurrent Planet Formation and Intermittent Protostellar Outflows Induced by Episodic Mass Accretion}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1101.1997},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, brown dwarfs, ISM: clouds, protoplanetary disks, planetary systems, stars: low-mass},
     year = 2011,
    month = mar,
   volume = 729,
      eid = {42},
    pages = {42},
      doi = {10.1088/0004-637X/729/1/42},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...729...42M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_aa_552_2013,
   author = {{Vorobyov}, E.~I.},
    title = "{Formation of giant planets and brown dwarfs on wide orbits}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1302.1892},
 primaryClass = "astro-ph.EP",
 keywords = {protoplanetary disks, planets and satellites: formation, stars: formation, hydrodynamics, stars: protostars},
     year = 2013,
    month = apr,
   volume = 552,
      eid = {A129},
    pages = {A129},
      doi = {10.1051/0004-6361/201220601},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...552A.129V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stamatellos_mnras_392_2009,
   author = {{Stamatellos}, D. and {Whitworth}, A.~P.},
    title = "{The properties of brown dwarfs and low-mass hydrogen-burning stars formed by disc fragmentation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0810.1687},
 keywords = {accretion, accretion discs , hydrodynamics , radiative transfer , methods: numerical , stars: formation , stars: low-mass, brown dwarfs},
     year = 2009,
    month = jan,
   volume = 392,
    pages = {413-427},
      doi = {10.1111/j.1365-2966.2008.14069.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.392..413S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shu_jbaa_102_1992,
   author = {{Shu}, F.~H.},
    title = "{Books-Received - the Physics of Astrophysics - V.2 - Gas Dynamics}",
  journal = {Journal of the British Astronomical Association},
     year = 1992,
    month = aug,
   volume = 102,
    pages = {230},
   adsurl = {http://adsabs.harvard.edu/abs/1992JBAA..102..230S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{boss_2017arXiv170104892B,
   author = {{Boss}, A.~P.},
    title = "{The Effect of Protoplanetary Disk Cooling Times on the Formation of Gas Giant Planets by Gravitational Instability}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1701.04892},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2017,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170104892B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{durissen_prpl_607_2007,
   author = {{Durisen}, R.~H. and {Boss}, A.~P. and {Mayer}, L. and {Nelson}, A.~F. and 
	{Quinn}, T. and {Rice}, W.~K.~M.},
    title = "{Gravitational Instabilities in Gaseous Protoplanetary Disks and Implications for Giant Planet Formation}",
  journal = {Protostars and Planets V},
   eprint = {astro-ph/0603179},
     year = 2007,
    pages = {607-622},
   adsurl = {http://adsabs.harvard.edu/abs/2007prpl.conf..607D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{acke_aa_457_2006,
   author = {{Acke}, B. and {van den Ancker}, M.~E.},
    title = "{A survey for nanodiamond features in the 3 micron spectra of Herbig Ae/Be stars}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0606650},
 keywords = {circumstellar matter, stars: pre-main-sequence, planetary systems: protoplanetary disks},
     year = 2006,
    month = oct,
   volume = 457,
    pages = {171-181},
      doi = {10.1051/0004-6361:20065612},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...457..171A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{aschenbach_aa_341_1999,
   author = {{Aschenbach}, B. and {Leahy}, D.~A.},
    title = "{ROSAT all-sky survey map of the Cygnus Loop: Overall structure and comparison with radio map}",
  journal = {\aap},
 keywords = {SHOCK WAVES, ISM: CYGNUS LOOP, ISM: SUPERNOVA REMNANTS, X-RAYS: ISM},
     year = 1999,
    month = jan,
   volume = 341,
    pages = {602-609},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...341..602A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{arthur_apjs_165_2006,
   author = {{Arthur}, S.~J. and {Hoare}, M.~G.},
    title = "{Hydrodynamics of Cometary Compact H II Regions}",
  journal = {\apjs},
   eprint = {astro-ph/0511035},
 keywords = {ISM: H II Regions, ISM: Kinematics and Dynamics, Shock Waves, Stars: Formation, Stars: Winds, Outflows},
     year = 2006,
    month = jul,
   volume = 165,
    pages = {283-306},
      doi = {10.1086/503899},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..165..283A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{avedisova_saj_15_1972,
   author = {{Avedisova}, V.~S.},
    title = "{Formation of Nebulae by Wolf-Rayet Stars.}",
  journal = {\sovast},
     year = 1972,
    month = apr,
   volume = 15,
    pages = {708},
   adsurl = {http://adsabs.harvard.edu/abs/1972SvA....15..708A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{abbott_apj_242_1980,
   author = {{Abbott}, D.~C.},
    title = "{The theory of radiatively driven stellar winds. I - A physical interpretation}",
  journal = {\apj},
 keywords = {EARLY STARS, RADIATIVE TRANSFER, STELLAR MASS EJECTION, STELLAR WINDS, GAS PRESSURE, INTERSTELLAR MATTER, MATHEMATICAL MODELS, SOUND WAVES, STELLAR MAGNETIC FIELDS, STELLAR ROTATION, WAVE PROPAGATION},
     year = 1980,
    month = dec,
   volume = 242,
    pages = {1183-1207},
      doi = {10.1086/158550},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...242.1183A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{abbott_apl_311_1986,
   author = {{Friend}, D.~B. and {Abbott}, D.~C.},
    title = "{The theory of radiatively driven stellar winds. III - Wind models with finite disk correction and rotation}",
  journal = {\apj},
 keywords = {STELLAR MASS EJECTION, STELLAR MODELS, STELLAR ROTATION, STELLAR WINDS, CENTRIFUGAL FORCE, EQUATIONS OF MOTION, HOT STARS, WIND VELOCITY},
     year = 1986,
    month = dec,
   volume = 311,
    pages = {701-707},
      doi = {10.1086/164809},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...311..701F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{abbott_apj_259_1982,
   author = {{Abbott}, D.~C.},
    title = "{The theory of radiatively driven stellar winds. II - The line acceleration}",
  journal = {\apj},
 keywords = {LINE SPECTRA, RADIATION PRESSURE, STELLAR ENVELOPES, STELLAR MASS EJECTION, STELLAR SPECTRA, STELLAR WINDS, B STARS, EARLY STARS, O STARS, STELLAR TEMPERATURE, SUPERGIANT STARS, WOLF-RAYET STARS},
     year = 1982,
    month = aug,
   volume = 259,
    pages = {282-301},
      doi = {10.1086/160166},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...259..282A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{abdo_apj_722_2010,
   author = {{Abdo}, A.~A. and {Ackermann}, M. and {Ajello}, M.
	},
    title = "{Fermi-LAT Study of Gamma-ray Emission in the Direction of Supernova Remnant W49B}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1008.4190},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, ISM: individual objects: W49B, radiation mechanisms: non-thermal},
     year = 2010,
    month = oct,
   volume = 722,
    pages = {1303-1311},
      doi = {10.1088/0004-637X/722/2/1303},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...722.1303A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{alexiades_cnme_12_1996,
   author = {{Alexiades}, V. and {Amiez}, G. and {Gremaud}, P.-A.},
    title = "{Super-time-stepping acceleration of explicit schemes for parabolic problems}",
  journal = {Communication in Numerical Methods in Engineering},
     year = 1996,
   volume = 12,
    pages = {31-42},
}

@INPROCEEDINGS{arnaud_aspc_101_1996,
   author = {{Arnaud}, K.~A.},
    title = "{XSPEC: The First Ten Years}",
booktitle = {Astronomical Data Analysis Software and Systems V},
     year = 1996,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 101,
   editor = {{Jacoby}, G.~H. and {Barnes}, J.},
    pages = {17},
   adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..101...17A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{asplund_araa_47_2009,
   author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J. and {Scott}, P.
	},
    title = "{The Chemical Composition of the Sun}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0909.0948},
 primaryClass = "astro-ph.SR",
     year = 2009,
    month = sep,
   volume = 47,
    pages = {481-522},
      doi = {10.1146/annurev.astro.46.060407.145222},
   adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..481A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE B 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{baade_apj_88_1938,
   author = {{Baade}, W.},
    title = "{The Absolute Photographic Magnitude of Supernovae.}",
  journal = {\apj},
     year = 1938,
    month = oct,
   volume = 88,
    pages = {285},
      doi = {10.1086/143983},
   adsurl = {http://adsabs.harvard.edu/abs/1938ApJ....88..285B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{badenes_mnras_407_2010,
   author = {{Badenes}, C. and {Maoz}, D. and {Draine}, B.~T.},
    title = "{On the size distribution of supernova remnants in the Magellanic Clouds}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1003.3030},
 primaryClass = "astro-ph.GA",
 keywords = {supernovae: general, ISM: supernova remnants, galaxies: individual: LMC, galaxies: individual: SMC},
     year = 2010,
    month = sep,
   volume = 407,
    pages = {1301-1313},
      doi = {10.1111/j.1365-2966.2010.17023.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407.1301B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{balbus_apj_376_1991,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F.},
    title = "{A powerful local shear instability in weakly magnetized disks. I - Linear analysis. II - Nonlinear evolution}",
  journal = {\apj},
 keywords = {Accretion Disks, Magnetohydrodynamic Stability, Stellar Magnetic Fields, Stellar Mass Accretion, Boussinesq Approximation, Computational Astrophysics, Linear Systems},
     year = 1991,
    month = jul,
   volume = 376,
    pages = {214-233},
      doi = {10.1086/170270},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...376..214B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hawley_apj_367_1991,
   author = {{Hawley}, J.~F. and {Balbus}, S.~A.},
    title = "{A Powerful Local Shear Instability in Weakly Magnetized Disks. II. Nonlinear Evolution}",
  journal = {\apj},
 keywords = {HYDROMAGNETICS, INSTABILITIES, STARS: ACCRETION},
     year = 1991,
    month = jul,
   volume = 376,
    pages = {223},
      doi = {10.1086/170271},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...376..223H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hawley_apj_400_1992,
   author = {{Hawley}, J.~F. and {Balbus}, S.~A.},
    title = "{A powerful local shear instability in weakly magnetized disks. III - Long-term evolution in a shearing sheet}",
  journal = {\apj},
 keywords = {Accretion Disks, Angular Momentum, Magnetic Field Configurations, Magnetohydrodynamic Stability, Nonlinear Evolution Equations, Computer Animation, Finite Difference Theory, Shear Flow},
     year = 1992,
    month = dec,
   volume = 400,
    pages = {595-609},
      doi = {10.1086/172021},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...400..595H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balbus_apj_400_1992,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F.},
    title = "{A Powerful Local Shear Instability in Weakly Magnetized Disks. IV. Nonaxisymmetric Perturbations}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, INSTABILITIES, MAGNETOHYDRODYNAMICS: MHD},
     year = 1992,
    month = dec,
   volume = 400,
    pages = {610-621},
      doi = {10.1086/172022},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...400..610B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{banerjee_apj_641_2006,
   author = {{Banerjee}, R. and {Pudritz}, R.~E.},
    title = "{Outflows and Jets from Collapsing Magnetized Cloud Cores}",
  journal = {\apj},
   eprint = {astro-ph/0508374},
 keywords = {Accretion, Accretion Disks, ISM: Clouds, ISM: Evolution, Methods: Numerical, Magnetohydrodynamics: MHD},
     year = 2006,
    month = apr,
   volume = 641,
    pages = {949-960},
      doi = {10.1086/500496},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...641..949B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...461..933K,
   author = {{Kley}, W. and {Lin}, D.~N.~C.},
    title = "{The Structure of the Boundary Layer in Protostellar Disks}",
  journal = {\apj},
 keywords = {STARS: CIRCUMSTELLAR MATTER, HYDRODYNAMICS, STARS: FORMATION, STARS: PRE-MAIN-SEQUENCE},
     year = 1996,
    month = apr,
   volume = 461,
    pages = {933},
      doi = {10.1086/177115},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...461..933K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{banerjee_mnras_373_2006,
   author = {{Banerjee}, R. and {Pudritz}, R.~E. and {Anderson}, D.~W.},
    title = "{Supersonic turbulence, filamentary accretion and the rapid assembly of massive stars and discs}",
  journal = {\mnras},
   eprint = {astro-ph/0609428},
 keywords = {turbulence, methods: numerical, ISM: clouds, ISM: evolution},
     year = 2006,
    month = dec,
   volume = 373,
    pages = {1091-1106},
      doi = {10.1111/j.1365-2966.2006.11089.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.373.1091B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{benerjee_apj_660_2007,
   author = {{Banerjee}, R. and {Pudritz}, R.~E.},
    title = "{Massive Star Formation via High Accretion Rates and Early Disk-driven Outflows}",
  journal = {\apj},
   eprint = {astro-ph/0612674},
 keywords = {Accretion, Accretion Disks, ISM: Clouds, ISM: Evolution, Methods: Numerical, Magnetohydrodynamics: MHD},
     year = 2007,
    month = may,
   volume = 660,
    pages = {479-488},
      doi = {10.1086/512010},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660..479B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{banerjee_mnras_355_2004,
   author = {{Banerjee}, R. and {Pudritz}, R.~E. and {Holmes}, L.},
    title = "{The formation and evolution of protostellar discs; three-dimensional adaptive mesh refinement hydrosimulations of collapsing, rotating Bonnor-Ebert spheres}",
  journal = {\mnras},
   eprint = {astro-ph/0408277},
 keywords = {accretion, accretion discs, hydrodynamics, methods: numerical, ISM: clouds, ISM: evolution},
     year = 2004,
    month = nov,
   volume = 355,
    pages = {248-272},
      doi = {10.1111/j.1365-2966.2004.08316.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.355..248B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baranov_sovastronlett_1_1975,
   author = {{Baranov}, V.~B. and {Krasnobaev}, K.~V. and {Onishchenko}, O.~G.
	},
    title = "{Proposed experimental test of a model for interaction between the solar wind and the interstellar medium}",
  journal = {Soviet Astronomy Letters},
 keywords = {ASTRONOMICAL MODELS, INTERSTELLAR MATTER, PLASMA-PARTICLE INTERACTIONS, SOLAR WIND, PULSARS, QUASARS, RADIO ASTRONOMY, SCINTILLATION, SUPERSONIC FLOW},
     year = 1975,
    month = apr,
   volume = 1,
    pages = {81},
   adsurl = {http://adsabs.harvard.edu/abs/1975SvAL....1...81B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baranov_sphd_15_1971,
   author = {{Baranov}, V.~B. and {Krasnobaev}, K.~V. and {Kulikovskii}, A.~G.
	},
    title = "{A Model of the Interaction of the Solar Wind with the Interstellar Medium}",
  journal = {Soviet Physics Doklady},
     year = 1971,
    month = mar,
   volume = 15,
    pages = {791},
   adsurl = {http://adsabs.harvard.edu/abs/1971SPhD...15..791B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bonnell_mnras_271_1994,
   author = {{Bonnell}, I.~A. and {Bate}, M.~R.},
    title = "{The Formation of Close Binary Systems}",
  journal = {\mnras},
   eprint = {astro-ph/9411081},
 keywords = {ACCRETION DISKS, BINARY STARS, COMPUTATIONAL ASTROPHYSICS, STAR FORMATION, PRE-MAIN SEQUENCE STARS, PROTOSTARS, HYDRODYNAMICS},
     year = 1994,
    month = dec,
   volume = 271,
      doi = {10.1093/mnras/271.4.999},
   adsurl = {http://adsabs.harvard.edu/abs/1994MNRAS.271..999B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bate_mnras_336_2002,
   author = {{Bate}, M.~R. and {Bonnell}, I.~A. and {Bromm}, V.},
    title = "{The formation of close binary systems by dynamical interactions and orbital decay}",
  journal = {\mnras},
   eprint = {astro-ph/0212403},
 keywords = {accretion, accretion discs, hydrodynamics, binaries: close, binaries: spectroscopic, circumstellar matter, stars: formation},
     year = 2002,
    month = nov,
   volume = 336,
    pages = {705-713},
      doi = {10.1046/j.1365-8711.2002.05775.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.336..705B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bate_apj_508_1998,
   author = {{Bate}, M.~R.},
    title = "{Collapse of a Molecular Cloud Core to Stellar Densities: The First Three-dimensional Calculations}",
  journal = {\apjl},
   eprint = {astro-ph/9810397},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, ISM: CLOUDS, METHODS: NUMERICAL, STARS: FORMATION, Accretion, Accretion Disks, Hydrodynamics, ISM: Clouds, Methods: Numerical, Stars: Formation},
     year = 1998,
    month = nov,
   volume = 508,
    pages = {L95-L98},
      doi = {10.1086/311719},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...508L..95B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balsara_mnras_386_2008,
   author = {{Balsara}, D.~S. and {Tilley}, D.~A. and {Howk}, J.~C.},
    title = "{Simulating anisotropic thermal conduction in supernova remnants - I. Numerical methods}",
  journal = {\mnras},
 keywords = {conduction , MHD , methods: numerical , supernova remnants},
     year = 2008,
    month = may,
   volume = 386,
    pages = {627-641},
      doi = {10.1111/j.1365-2966.2008.13085.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008MNRAS.386..627B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balsara_MNRAS_386_2008a,
   author = {{Balsara}, D.~S. and {Bendinelli}, A.~J. and {Tilley}, D.~A. and 
	{Massari}, A.~R. and {Howk}, J.~C.},
    title = "{Simulating anisotropic thermal conduction in supernova remnants - II. Implications for the interstellar medium}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0711.2295},
 keywords = {conduction , MHD , ISM: evolution , supernova remnants , X-rays: ISM},
     year = 2008,
    month = may,
   volume = 386,
    pages = {642-656},
      doi = {10.1111/j.1365-2966.2008.13121.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..642B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balsara_MNRAS_386_2008b,
   author = {{Balsara}, D.~S. and {Tilley}, D.~A. and {Howk}, J.~C.},
    title = "{Simulating anisotropic thermal conduction in supernova remnants - I. Numerical methods}",
  journal = {\mnras},
 keywords = {conduction , MHD , methods: numerical , supernova remnants},
     year = 2008,
    month = may,
   volume = 386,
    pages = {627-641},
      doi = {10.1111/j.1365-2966.2008.13085.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..627B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bedogni_190_aa_1988,
   author = {{Bedogni}, R. and {D'Ercole}, A.},
    title = "{The electron thermal conduction in young supernova remnants}",
  journal = {\aap},
 keywords = {Astronomical Models, Conductive Heat Transfer, Supernova Remnants, Computational Astrophysics, Heat Flux, Hydrodynamic Equations, Plasma Turbulence, Shock Waves, Stellar Winds},
     year = 1988,
    month = jan,
   volume = 190,
    pages = {320-332},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...190..320B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{beuther_aa_538_2012,
   author = {{Beuther}, H. and {Tackenberg}, J. and {Linz}, H. and {Henning}, T. and 
	{Krause}, O. and {Ragan}, S. and {Nielbock}, M. and {Launhardt}, R. and 
	{Schmiedeke}, A. and {Schuller}, F. and {Carlhoff}, P. and {Nguyen-Luong}, Q. and 
	{Sakai}, T.},
    title = "{The onset of high-mass star formation in the direct vicinity of the Galactic mini-starburst W43}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1112.3543},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: early-type, stars: individual: W43, stars: individual: IRAS18454-0158, stars: evolution, stars: massive},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A11},
    pages = {A11},
      doi = {10.1051/0004-6361/201117850},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A..11B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{beuther_aa_503_2009,
   author = {{Beuther}, H. and {Henning}, T.},
    title = "{Multiple low-turbulence starless cores associated with intermediate- to high-mass star formation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.4565},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: individual: IRDC 19175-4, IRDC 19175-5, techniques: interferometric, line: formation, line: profiles, turbulence},
     year = 2009,
    month = sep,
   volume = 503,
    pages = {859-867},
      doi = {10.1051/0004-6361/200912036},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...503..859B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{beuther_aa_584_2015,
   author = {{Beuther}, H. and {Ragan}, S.~E. and {Johnston}, K. and {Henning}, T. and 
	{Hacar}, A. and {Kainulainen}, J.~T.},
    title = "{Filament fragmentation in high-mass star formation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1510.07063},
 keywords = {stars: formation, stars: early-type, stars: individual: IRDC 18223, stars: massive, ISM: clouds, ISM: structure},
     year = 2015,
    month = dec,
   volume = 584,
      eid = {A67},
    pages = {A67},
      doi = {10.1051/0004-6361/201527108},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...584A..67B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{beuther_aa_512_2010,
   author = {{Beuther}, H. and {Linz}, H. and {Bik}, A. and {Goto}, M. and 
	{Henning}, T.},
    title = "{Disk and outflow signatures in Orion-KL: the power of high-resolution thermal infrared spectroscopy}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1001.0650},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: early-type, accretion, , accretion disks, techniques: spectroscopic, ISM: jets and, outflows, stars: individual: Orion-BN, Orion source n},
     year = 2010,
    month = mar,
   volume = 512,
      eid = {A29},
    pages = {A29},
      doi = {10.1051/0004-6361/200913107},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...512A..29B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{beuther_aa_558_2013,
   author = {{Beuther}, H. and {Linz}, H. and {Henning}, T.},
    title = "{Fragmentation, infall, and outflow around the showcase massive protostar NGC 7538 IRS1 at 500 AU resolution}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1309.1018},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: early-type, stars: individual: NGC 7538IRS1, stars: massive},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A81},
    pages = {A81},
      doi = {10.1051/0004-6361/201321498},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558A..81B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{beuther_aa_543_2012,
   author = {{Beuther}, H. and {Linz}, H. and {Henning}, T.},
    title = "{The high-mass disk candidates NGC 7538IRS1 and NGC 7538S}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1205.5459},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: early-type, stars: individual: NGC 7538IRS1, stars: massive, stars: individual: NGC 7538S},
     year = 2012,
    month = jul,
   volume = 543,
      eid = {A88},
    pages = {A88},
      doi = {10.1051/0004-6361/201219128},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...543A..88B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{beuther_apjs_184_2009,
   author = {{Beuther}, H. and {Walsh}, A.~J. and {Longmore}, S.~N.},
    title = "{Hot High-Mass Accretion Disk Candidates}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0909.0691},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: kinematics and dynamics, stars: early-type, stars: formation, stars: individual: G305.21+0.21 G316.81{\ndash}0.06 G323.74{\ndash}0.26 G327.3{\ndash}0.6 G328.81+0.63 G331.28{\ndash}0.19 G336.02{\ndash}0.83 G345.00{\ndash}0.22 G351.77{\ndash}0.54 G0.55{\ndash}0.85 G19.47{\ndash}0.17 IRAS 18151{\ndash}1208, stars: rotation, techniques: interferometric},
     year = 2009,
    month = oct,
   volume = 184,
    pages = {366-386},
      doi = {10.1088/0067-0049/184/2/366},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..184..366B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blaauw_bain_15_1961,
   author = {{Blaauw}, A.},
    title = "{On the origin of the O- and B-type stars with high velocities (the ''run-away'' stars), and some related problems}",
  journal = {\bain},
     year = 1961,
    month = may,
   volume = 15,
    pages = {265},
   adsurl = {http://adsabs.harvard.edu/abs/1961BAN....15..265B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blandford_301_natur_1983,
   author = {{Blandford}, R.~D. and {Kennel}, C.~F. and {McKee}, C.~F. and 
	{Ostriker}, J.~P.},
    title = "{Trail of the Crab progenitor star}",
  journal = {\nat},
 keywords = {Astronomical Models, Crab Nebula, Red Giant Stars, Stellar Winds, Emission Spectra, H Lines, Jets, Oxygen, Stellar Mass Ejection},
     year = 1983,
    month = feb,
   volume = 301,
    pages = {586},
      doi = {10.1038/301586a0},
   adsurl = {http://adsabs.harvard.edu/abs/1983Natur.301..586B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{blau1993ASPC...35..207B,
   author = {{Blaauw}, A.},
    title = "{Massive Runaway Stars}",
booktitle = {Massive Stars:  Their Lives in the Interstellar Medium},
     year = 1993,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 35,
   editor = {{Cassinelli}, J.~P. and {Churchwell}, E.~B.},
    month = jan,
    pages = {207},
   adsurl = {http://adsabs.harvard.edu/abs/1993ASPC...35..207B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bjorkman_apj_409_1993,
   author = {{Bjorkman}, J.~E. and {Cassinelli}, J.~P.},
    title = "{Equatorial disk formation around rotating stars due to Ram pressure confinement by the stellar wind}",
  journal = {\apj},
 keywords = {B STARS, EARLY STARS, ROTATING DISKS, STELLAR ENVELOPES, STELLAR MASS EJECTION, STELLAR ROTATION, STELLAR WINDS, ANGULAR VELOCITY, EMISSION SPECTRA, LINE SPECTRA, STELLAR SPECTRA},
     year = 1993,
    month = may,
   volume = 409,
    pages = {429-449},
      doi = {10.1086/172676},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...409..429B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{benaglia_aa_517_2010,
   author = {{Benaglia}, P. and {Romero}, G.~E. and {Mart{\'{\i}}}, J. and 
	{Peri}, C.~S. and {Araudo}, A.~T.},
    title = "{Detection of nonthermal emission from the bow shock of a massive runaway star}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1007.3279},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, stars: individual: BD+43{\deg}3654, radio continuum: general, infrared: stars},
     year = 2010,
    month = jul,
   volume = 517,
      eid = {L10},
    pages = {L10},
      doi = {10.1051/0004-6361/201015232},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...517L..10B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{beuther_aa_503_2009,
   author = {{Beuther}, H. and {Henning}, T.},
    title = "{Multiple low-turbulence starless cores associated with intermediate- to high-mass star formation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.4565},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: individual: IRDC 19175-4, IRDC 19175-5, techniques: interferometric, line: formation, line: profiles, turbulence},
     year = 2009,
    month = sep,
   volume = 503,
    pages = {859-867},
      doi = {10.1051/0004-6361/200912036},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...503..859B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{boulanger_aa_312_1996,
   author = {{Boulanger}, F. and {Abergel}, A. and {Bernard}, J.-P. and {Burton}, W.~B. and 
	{Desert}, F.-X. and {Hartmann}, D. and {Lagache}, G. and {Puget}, J.-L.
	},
    title = "{The dust/gas correlation at high Galactic latitude.}",
  journal = {\aap},
 keywords = {ISM: ATOMS, ISM: DUST, EXTINCTION, ISM: MOLECULES, ISM: GENERAL, INFRARED: INTERSTELLAR: CONTINUUM},
     year = 1996,
    month = aug,
   volume = 312,
    pages = {256-262},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...312..256B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{bohren_book_1983,
   author = {{Bohren}, C.~F. and {Huffman}, D.~R.},
    title = "{Absorption and scattering of light by small particles}",
 keywords = {LIGHT SCATTERING, ABSORPTION, PARTICLES, DUST, THEORY},
booktitle = {New York: Wiley, 1983},
     year = 1983,
   adsurl = {http://adsabs.harvard.edu/abs/1983asls.book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{borkowski_apj_400_1992,
   author = {{Borkowski}, K.~J. and {Blondin}, J.~M. and {Sarazin}, C.~L.
	},
    title = "{Dynamics of Kepler's supernova remnant}",
  journal = {\apj},
 keywords = {Hydrodynamics, Interstellar Matter, Kepler Laws, Stellar Envelopes, Stellar Winds, Supernova Remnants, Milky Way Galaxy, Shock Wave Interaction, Stellar Mass Ejection, Taylor Instability},
     year = 1992,
    month = nov,
   volume = 400,
    pages = {222-237},
      doi = {10.1086/171989},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...400..222B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{boley_aa_547_2012,
   author = {{Boley}, P.~A. and {Linz}, H. and {van Boekel}, R. and {Bouwman}, J. and 
	{Henning}, T. and {Sobolev}, A.~M.},
    title = "{On the massive young stellar object AFGL 4176. High-spatial-resolution multi-wavelength observations and modeling}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1209.3583},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, techniques: interferometric, techniques: high angular resolution, radiative transfer, stars: individual: AFGL 4176},
     year = 2012,
    month = nov,
   volume = 547,
      eid = {A88},
    pages = {A88},
      doi = {10.1051/0004-6361/201218905},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...547A..88B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bowler_aj_137_2009,
   author = {{Bowler}, B.~P. and {Waller}, W.~H. and {Megeath}, S.~T. and 
	{Patten}, B.~M. and {Tamura}, M.},
    title = "{An Infrared Census of Star Formation in the Horsehead Nebula}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0901.0564},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, ISM: globules, ISM: individual: Horsehead Nebula, stars: formation, stars: pre-main sequence},
     year = 2009,
    month = mar,
   volume = 137,
    pages = {3685-3699},
      doi = {10.1088/0004-6256/137/3/3685},
   adsurl = {http://adsabs.harvard.edu/abs/2009AJ....137.3685B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blondin_apj_472_1996,
   author = {{Blondin}, J.~M. and {Lundqvist}, P. and {Chevalier}, R.~A.},
    title = "{Axisymmetric Circumstellar Interaction in Supernovae}",
  journal = {\apj},
   eprint = {astro-ph/9601137},
 keywords = {STARS: CIRCUMSTELLAR MATTER, HYDRODYNAMICS, ISM: STRUCTURE, SHOCK WAVES, ISM: SUPERNOVA REMNANTS, STARS: SUPERNOVAE: GENERAL},
     year = 1996,
    month = nov,
   volume = 472,
    pages = {257},
      doi = {10.1086/178060},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...472..257B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blondin_na_57_1998,
   author = {{Blondin}, J.~M. and {Koerwer}, J.~F.},
    title = "{Instability of isothermal stellar wind bowshocks}",
  journal = {\na},
 keywords = {Hydrodynamics, Instabilities, Shock waves, Circumstellar matter, Hydrodynamics, Circumstellar shells, clouds, and expanding envelopes; circumstellar masers, Mass loss and stellar winds},
     year = 1998,
    month = dec,
   volume = 3,
    pages = {571-582},
      doi = {10.1016/S1384-1076(98)00028-1},
   adsurl = {http://adsabs.harvard.edu/abs/1998NewA....3..571B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Unpublished{ braithwait_2011b,
	title = "An introduction to hydrodynamics and astrophysical manetohydrodynamics",
	author = "J. Braithwait",
	note = "Aifa lecture note",
	month = "March",
	year = "2011"
}

@Unpublished{braithwait_2011a,
	title = "An introduction to astrophysical manetohydrodynamics",
	author = "J. Braithwait",
	note = "Aifa lecture note"
}


@ARTICLE{brighenti_mnras_273_1995,
   author = {{Brighenti}, F. and {D'Ercole}, A.},
    title = "{Evolution of WR ring nebulae generated by moving central stars - I. The paradigm of G2.4+1.4}",
  journal = {\mnras},
 keywords = {STARS: MASS-LOSS, STARS: WOLF-RAYET, ISM: BUBBLES, ISM: INDIVIDUAL: G2.4+1.4.},
     year = 1995,
    month = mar,
   volume = 273,
    pages = {443-448},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.273..443B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brighenti_mnras_277_1995,
   author = {{Brighenti}, F. and {D'Ercole}, A.},
    title = "{Evolution of WR ring nebulae generated by a moving central star - II. The influence of the red supergiant bow shock}",
  journal = {\mnras},
 keywords = {HYDRODYNAMICS, INSTABILITIES, STARS: WOLF-RAYET, ISM: BUBBLES},
     year = 1995,
    month = nov,
   volume = 277,
    pages = {53-69},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.277...53B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{brighenti_mnras_270_1994,
   author = {{Brighenti}, F. and {D'Ercole}, A.},
    title = "{Evolution of Supernova Remnants Generated by Moving Massive Stars}",
  journal = {\mnras},
     year = 1994,
    month = sep,
   volume = 270,
    pages = {65},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1994MNRAS.270...65B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brott_aa_530_2011b,
   author = {{Brott}, I. and {Evans}, C.~J. and {Hunter}, I. and {de Koter}, A. and 
	{Langer}, N. and {Dufton}, P.~L. and {Cantiello}, M. and {Trundle}, C. and 
	{Lennon}, D.~J. and {de Mink}, S.~E. and {Yoon}, S.-C. and {Anders}, P.
	},
    title = "{Rotating massive main-sequence stars. II. Simulating a population of LMC early B-type stars as a test of rotational mixing}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1102.0766},
 primaryClass = "astro-ph.SR",
 keywords = {methods: statistical, stars: abundances, stars: evolution, stars: early-type, stars: massive, stars: rotation},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A116},
    pages = {A116},
      doi = {10.1051/0004-6361/201016114},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A.116B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brott_aa_530_2011a,
   author = {{Brott}, I. and {de Mink}, S.~E. and {Cantiello}, M. and {Langer}, N. and 
	{de Koter}, A. and {Evans}, C.~J. and {Hunter}, I. and {Trundle}, C. and 
	{Vink}, J.~S.},
    title = "{Rotating massive main-sequence stars. I. Grids of evolutionary models and isochrones}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1102.0530},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: evolution, stars: early-type, stars: rotation, stars: massive},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A115},
    pages = {A115},
      doi = {10.1051/0004-6361/201016113},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A.115B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bucciantini_aa_405_2003,
   author = {{Bucciantini}, N. and {Blondin}, J.~M. and {Del Zanna}, L. and 
	{Amato}, E.},
    title = "{Spherically symmetric relativistic MHD simulations of pulsar wind nebulae in supernova remnants}",
  journal = {\aap},
   eprint = {astro-ph/0303491},
 keywords = {ISM: supernova remnants, stars: pulsars: general, stars: winds, outflows, magnetohydrodynamics, shock waves, relativity},
     year = 2003,
    month = jul,
   volume = 405,
    pages = {617-626},
      doi = {10.1051/0004-6361:20030624},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...405..617B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{burns_mnras_460_2016,
   author = {{Burns}, R.~A. and {Handa}, T. and {Nagayama}, T. and {Sunada}, K. and 
	{Omodaka}, T.},
    title = "{H$_{2}$O masers in a jet-driven bow shock: episodic ejection from a massive young stellar object}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1604.05682},
 primaryClass = "astro-ph.SR",
 keywords = {masers, stars: individual: S255IR-SMA1, stars: massive, ISM: jets and outflows},
     year = 2016,
    month = jul,
   volume = 460,
    pages = {283-290},
      doi = {10.1093/mnras/stw958},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.460..283B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{buren_apj_329_1988,
   author = {{van Buren}, D. and {McCray}, R.},
    title = "{Bow shocks and bubbles are seen around hot stars by IRAS}",
  journal = {\apjl},
 keywords = {BOW WAVES, EARLY STARS, HOT STARS, INFRARED STARS, INTERSTELLAR MATTER, PLASMA BUBBLES, STELLAR WINDS, COSMIC DUST, H II REGIONS, INFRARED ASTRONOMY SATELLITE, RADIATION PRESSURE, STELLAR LUMINOSITY},
     year = 1988,
    month = jun,
   volume = 329,
    pages = {L93-L96},
      doi = {10.1086/185184},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...329L..93V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE C 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{caratti_nature_2016,
   author = { {Caratti o Garatti}, A.
and {Stecklum}, B.
and {Garcia Lopez}, R.
and {Eisloffel}, J.
and {Ray}, T.~P.
and {Sanna}, A.
and {Cesaroni}, R.
and {Walmsley}, C.~M.
and {Oudmaijer}, R.~D.
and {de Wit}, W.~J.
and {Moscadelli}, L.
and {Greiner}, J.
and {Krabbe}, A.
and {Fischer}, C.
and {Klein}, R.
and {Ibanez}, J.~M.},
    title = "{Disk-mediated accretion burst in a high-mass young stellar object}",
  journal = {Nature},
     year = 2016,
    month = nov,
    pages = {1745-2481},
      doi = {http://dx.doi.org/10.1038/nphys3942},
}

@ARTICLE{Carrasco_sci_348_2015,
   author = {{Carrasco-Gonz{\'a}lez}, C. and {Torrelles}, J.~M. and {Cant{\'o}}, J. and 
	{Curiel}, S. and {Surcis}, G. and {Vlemmings}, W.~H.~T. and 
	{van Langevelde}, H.~J. and {Goddi}, C. and {Anglada}, G. and 
	{Kim}, S.-W. and {Kim}, J.-S. and {G{\'o}mez}, J.~F.},
    title = "{Observing the onset of outflow collimation in a massive protostar}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1507.05285},
 primaryClass = "astro-ph.SR",
     year = 2015,
    month = apr,
   volume = 348,
    pages = {114-117},
      doi = {10.1126/science.aaa7216},
   adsurl = {http://adsabs.harvard.edu/abs/2015Sci...348..114C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{castor_apj_200_1975,
   author = {{Castor}, J.~I. and {McCray}, R. and {Weaver}, R.},
    title = "{Interstellar Bubbles}",
booktitle = {Bulletin of the American Astronomical Society},
     year = 1975,
   series = {Bulletin of the American Astronomical Society},
   volume = 7,
    month = jun,
    pages = {428},
   adsurl = {http://adsabs.harvard.edu/abs/1975BAAS....7..428C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cesaroni_natur_444_2006,
   author = {{Cesaroni}, R. and {Galli}, D. and {Lodato}, G. and {Walmsley}, M. and 
	{Zhang}, Q.},
    title = "{The critical role of disks in the formation of high-mass stars}",
  journal = {\nat},
     year = 2006,
    month = dec,
   volume = 444,
    pages = {703-706},
      doi = {10.1038/nature05344},
   adsurl = {http://adsabs.harvard.edu/abs/2006Natur.444..703C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cesaroni_aa_509_2010,
   author = {{Cesaroni}, R. and {Hofner}, P. and {Araya}, E. and {Kurtz}, S.
	},
    title = "{The structure of hot molecular cores over 1000 AU}",
  journal = {\aap},
 keywords = {stars: formation, Hii regions, ISM: individual objects: G10.47+0.03, G31.41+0.31, ISM: molecules},
     year = 2010,
    month = jan,
   volume = 509,
      eid = {A50},
    pages = {A50},
      doi = {10.1051/0004-6361/200912877},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...509A..50C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cesaroni_aa_549_2013,
   author = {{Cesaroni}, R. and {Massi}, F. and {Arcidiacono}, C. and {Beltr{\'a}n}, M.~T. and 
	{McCarthy}, D. and {Kulesa}, C. and {Boutsia}, K. and {Paris}, D. and 
	{Quir{\'o}s-Pacheco}, F. and {Xompero}, M.},
    title = "{A close-up view of a bipolar jet: Sub-arcsecond near-infrared imaging of the high-mass protostar IRAS 20126+4104}",
  journal = {\aap},
 keywords = {stars: formation, ISM: individual objects: IRAS 20126+4104, ISM: jets and outflows},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A146},
    pages = {A146},
      doi = {10.1051/0004-6361/201220609},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A.146C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cesaroni_aa_345_1999,
   author = {{Cesaroni}, R. and {Felli}, M. and {Jenness}, T. and {Neri}, R. and 
	{Olmi}, L. and {Robberto}, M. and {Testi}, L. and {Walmsley}, C.~M.
	},
    title = "{Unveiling the disk-jet system in the massive (proto)star IRAS 20126+4104}",
  journal = {\aap},
 keywords = {ISM: CLOUDS, ISM: INDIVIDUAL OBJECTS: IRAS 20126+4104, ISM: MOLECULES, RADIO LINES: ISM},
     year = 1999,
    month = may,
   volume = 345,
    pages = {949-964},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...345..949C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ciotti_aa_215_1989,
   author = {{Ciotti}, L. and {D'Ercole}, A.},
    title = "{SNR expansion in a pre-existent cavity}",
  journal = {\aap},
 keywords = {B STARS, COMPUTATIONAL ASTROPHYSICS, O STARS, STELLAR WINDS, SUPERNOVA REMNANTS, ASTRONOMICAL MODELS, STELLAR TEMPERATURE, WAVE PROPAGATION},
     year = 1989,
    month = may,
   volume = 215,
    pages = {347-359},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...215..347C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{hennebelle_743_apj_2011,
   author = {{Hennebelle}, P. and {Chabrier}, G.},
    title = "{Analytical Star Formation Rate from Gravoturbulent Fragmentation}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1110.0033},
 keywords = {ISM: clouds, turbulence, stars: formation},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {L29},
    pages = {L29},
      doi = {10.1088/2041-8205/743/2/L29},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743L..29H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{cherchneff_proc_232_1994,
   author = {{Cherchneff}, I. and {Tielens}, A.~G.~G.~M.},
    title = "{Mass loss from late type stars}",
booktitle = {Circumstellar Media in Late Stages of Stellar Evolution},
     year = 1994,
   editor = {{Clegg}, R.~E.~S. and {Stevens}, I.~R. and {Meikle}, W.~P.~S.
	},
    pages = {232},
   adsurl = {http://adsabs.harvard.edu/abs/1994cmls.conf..232C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chevalier_apj_344_1989,
   author = {{Chevalier}, R.~A. and {Liang}, E.~P.},
    title = "{The interaction of supernovae with circumstellar bubbles}",
  journal = {\apj},
 keywords = {STELLAR ENVELOPES, STELLAR WINDS, SUPERNOVA REMNANTS, SUPERNOVAE, RADIO SOURCES (ASTRONOMY), SHOCK WAVES, STELLAR EVOLUTION, STELLAR MASS, SUPERNOVA 1987A, X RAY SOURCES},
     year = 1989,
    month = sep,
   volume = 344,
    pages = {332-340},
      doi = {10.1086/167802},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...344..332C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{chevalier_apj_258_1982,
   author = {{Chevalier}, R.~A.},
    title = "{Self-similar solutions for the interaction of stellar ejecta with an external medium}",
  journal = {\apj},
 keywords = {Interstellar Matter, Stellar Mass Ejection, Supernova Remnants, Density Distribution, Gas Density, Gas-Gas Interactions, Gas-Solid Interactions, Light Curve, X Ray Spectra},
     year = 1982,
    month = jul,
   volume = 258,
    pages = {790-797},
      doi = {10.1086/160126},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...258..790C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PhDThesis{ chita_phd_2011,
	title = "Models for circumstellar nebulae around red and blue supergiant",
	author = "S. M. Chita",
	school = "Utrecht University",
	month = "September",
	year = "2011",
	address = "Netherland"
}

@INPROCEEDINGS{chita_revmexaa_30_2007,
   author = {{Chita}, S.~M. and {van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{The Evolution of Circumstellar Medium around Rotating Massive Stars}",
 keywords = {Hydrodynamics, ISM: bubbles, Stars: supergiants, Stars: winds, outflows},
booktitle = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
     year = 2007,
   series = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
   volume = 30,
    month = aug,
    pages = {80-83},
   adsurl = {http://adsabs.harvard.edu/abs/2007RMxAC..30...80C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chita_aa_488_2008,
   author = {{Chita}, S.~M. and {Langer}, N. and {van Marle}, A.~J. and {Garc{\'{\i}}a-Segura}, G. and 
	{Heger}, A.},
    title = "{Multiple ring nebulae around blue supergiants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0807.3049},
 keywords = {hydrodynamics, ISM: bubbles, stars: winds, outflows, stars: supergiants},
     year = 2008,
    month = sep,
   volume = 488,
    pages = {L37-L41},
      doi = {10.1051/0004-6361:200810087},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...488L..37C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{chiotellis_aa_537_2012,
   author = {{Chiotellis}, A. and {Schure}, K.~M. and {Vink}, J.},
    title = "{The imprint of a symbiotic binary progenitor on the properties of Kepler's supernova remnant}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1103.5487},
 primaryClass = "astro-ph.GA",
 keywords = {ISM: supernova remnants, hydrodynamics, binaries: symbiotic, supernovae: individual: SN1604},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A139},
    pages = {A139},
      doi = {10.1051/0004-6361/201014754},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A.139C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{clarke_mnras_381_2007,
   author = {{Clarke}, C.~J. and {Harper-Clark}, E. and {Lodato}, G.},
    title = "{The response of self-gravitating protostellar discs to slow reduction in cooling time-scale: the fragmentation boundary revisited}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0708.0742},
 keywords = {accretion, accretion discs, gravitation, instabilities, stars: formation},
     year = 2007,
    month = nov,
   volume = 381,
    pages = {1543-1547},
      doi = {10.1111/j.1365-2966.2007.12322.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.381.1543C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{commercon_apj_742_2011,
   author = {{Commer{\c c}on}, B. and {Hennebelle}, P. and {Henning}, T.},
    title = "{Collapse of Massive Magnetized Dense Cores Using Radiation Magnetohydrodynamics: Early Fragmentation Inhibition}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1110.2955},
 primaryClass = "astro-ph.SR",
 keywords = {magnetohydrodynamics: MHD, methods: numerical, radiative transfer, stars: formation, stars: massive, stars: kinematics and dynamics},
     year = 2011,
    month = nov,
   volume = 742,
      eid = {L9},
    pages = {L9},
      doi = {10.1088/2041-8205/742/1/L9},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742L...9C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{commercon_aa_510_2010,
   author = {{Commer{\c c}on}, B. and {Hennebelle}, P. and {Audit}, E. and 
	{Chabrier}, G. and {Teyssier}, R.},
    title = "{Protostellar collapse: radiative and magnetic feedbacks on small-scale fragmentation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0912.3138},
 primaryClass = "astro-ph.SR",
 keywords = {magnetohydrodynamics (MHD), radiative transfer, stars: formation, stars: low mass, ISM: clouds, ISM: kinematics and dynamics},
     year = 2010,
    month = feb,
   volume = 510,
      eid = {L3},
    pages = {L3},
      doi = {10.1051/0004-6361/200913597},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...510L...3C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{commercon_aa_545_2012,
   author = {{Commer{\c c}on}, B. and {Launhardt}, R. and {Dullemond}, C. and 
	{Henning}, T.},
    title = "{Synthetic observations of first hydrostatic cores in collapsing low-mass dense cores. I. Spectral energy distributions and evolutionary sequence}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1207.0656},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, magnetohydrodynamics (MHD), methods: numerical, stars: formation, stars: low-mass, stars: protostars},
     year = 2012,
    month = sep,
   volume = 545,
      eid = {A98},
    pages = {A98},
      doi = {10.1051/0004-6361/201118706},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...545A..98C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{commercon_aa_548_2012,
   author = {{Commer{\c c}on}, B. and {Levrier}, F. and {Maury}, A.~J. and 
	{Henning}, T. and {Launhardt}, R.},
    title = "{Synthetic observations of first hydrostatic cores in collapsing low-mass dense cores. II. Simulated ALMA dust emission maps}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1210.1023},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: low-mass, magnetohydrodynamics (MHD), radiative transfer, techniques: interferometric, methods: numerical},
     year = 2012,
    month = dec,
   volume = 548,
      eid = {A39},
    pages = {A39},
      doi = {10.1051/0004-6361/201220067},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...548A..39C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{comeron_aa_326_1997,
   author = {{Comer\`{o}n}, F.},
    title = "{Dynamical evolution of wind-driven HII regions in strong density gradients.}",
  journal = {\aap},
 keywords = {STARS: EARLY-TYPE, ISM: BUBBLES, CLOUDS, HII REGIONS, KINEMATICS AND DYNAMICS, HYDRODYNAMICS},
     year = 1997,
    month = oct,
   volume = 326,
    pages = {1195-1214},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...326.1195C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{comeron_aa_338_1998,
   author = {{Comer\'{o}n}, F. and {Kaper}, L.},
    title = "{Numerical simulations of wind bow shocks produced by runaway OB stars}",
  journal = {\aap},
 keywords = {SHOCK WAVES, STARS: EARLY-TYPE, ISM: BUBBLES, ISM: KINEMATICS AND DYNAMICS},
     year = 1998,
    month = oct,
   volume = 338,
    pages = {273-291},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...338..273C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ciardi_mnras_409_2010,
   author = {{Ciardi}, A. and {Hennebelle}, P.},
    title = "{Outflows and mass accretion in collapsing dense cores with misaligned rotation axis and magnetic field}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1009.0453},
 primaryClass = "astro-ph.SR",
 keywords = {instabilities, MHD, stars: formation, stars: winds, outflows, ISM: clouds, ISM: kinematics and dynamics},
     year = 2010,
    month = nov,
   volume = 409,
    pages = {L39-L43},
      doi = {10.1111/j.1745-3933.2010.00942.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.409L..39C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{compiegne_aa_491_2008,
   author = {{Compi{\`e}gne}, M. and {Abergel}, A. and {Verstraete}, L. and 
	{Habart}, E.},
    title = "{Dust processing in photodissociation regions. Mid-IR emission modelling}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0809.5026},
 keywords = {ISM: individual objects: Horsehead, ISM: individual objects: NGC 2023, ISM: dust, extinction, infrared: ISM},
     year = 2008,
    month = dec,
   volume = 491,
    pages = {797-807},
      doi = {10.1051/0004-6361:200809850},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...491..797C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{conlon_aa_236_1990,
   author = {{Conlon}, E.~S. and {Dufton}, P.~L. and {Keenan}, F.~P. and 
	{Leonard}, P.~J.~T.},
    title = "{The runaway nature of distant early-type stars in the galactic halo}",
  journal = {\aap},
 keywords = {B STARS, BINARY STARS, BLUE STARS, EARLY STARS, GALACTIC STRUCTURE, STELLAR EVOLUTION, MANY BODY PROBLEM, MASS TRANSFER, OPEN CLUSTERS, REFERENCE STARS, STELLAR MASS, SUPERNOVAE},
     year = 1990,
    month = sep,
   volume = 236,
    pages = {357-361},
   adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...236..357C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{couch_aspc_393_2008,
   author = {{Couch}, S.~M. and {Wheeler}, J.~C. and {Milosavljevi{\'c}}, M.
	},
    title = "{Hydrodynamic Instabilities in Jet-Induced Supernovae: Results of 2D Simulations}",
booktitle = {New Horizons in Astronomy},
     year = 2008,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 393,
   editor = "{A.~Frebel, J.~R.~Maund, J.~Shen, \& M.~H.~Siegel}",
    month = aug,
    pages = {183},
   adsurl = {http://adsabs.harvard.edu/abs/2008ASPC..393..183C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cox_apj_178_1974,
   author = {{Cox}, D.~P.},
    title = "{Cooling and Evolution of a Supernova Remnant}",
  journal = {\apj},
     year = 1972,
    month = nov,
   volume = 178,
    pages = {159-168},
      doi = {10.1086/151775},
   adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...178..159C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cox_aa_537_2012,
   author = {{Cox}, N.~L.~J. and {Kerschbaum}, F. and {van Marle}, A.~J. and {Decin}, L. and {Ladjal}, D. and {Mayer}, A.},
    title = "{A far-infrared survey of bow shocks and detached shells around AGB stars and red supergiants (Corrigendum)}",
  journal = {\aap},
 keywords = {stars: AGB and post-AGB, circumstellar matter, infrared: ISM, hydrodynamics, stars: mass-loss, errata, addenda},
     year = 2012,
    month = jul,
   volume = 543,
      eid = {C1},
    pages = {C1},
      doi = {10.1051/0004-6361/201117910e},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cox_mnras_250_1991,
   author = {{Cox}, C.~I. and {Gull}, S.~F. and {Green}, D.~A.},
    title = "{Numerical simulations of the 'jet' in the Crab nebula}",
  journal = {\mnras},
 keywords = {Crab Nebula, Stellar Models, Stellar Winds, Cool Stars, Cooling Flows (Astrophysics), Digital Simulation, Plasma Jets, Supernova Remnants},
     year = 1991,
    month = jun,
   volume = 250,
    pages = {750-759},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.250..750C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cowie_apj_211_1977,
   author = {{Cowie}, L.~L. and {McKee}, C.~F.},
    title = "{The evaporation of spherical clouds in a hot gas. I - Classical and saturated mass loss rates}",
  journal = {\apj},
 keywords = {EVAPORATION, HIGH TEMPERATURE GASES, INTERSTELLAR GAS, NEBULAE, SUPERNOVA REMNANTS, CONDUCTIVE HEAT TRANSFER, HEAT FLUX, MASS FLOW RATE, SOLAR WIND, TEMPERATURE PROFILES},
     year = 1977,
    month = jan,
   volume = 211,
    pages = {135-146},
      doi = {10.1086/154911},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...211..135C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE D 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{davies_apj_671_2007,
   author = {{Davies}, R.~I. and {M{\"u}ller S{\'a}nchez}, F. and {Genzel}, R. and 
	{Tacconi}, L.~J. and {Hicks}, E.~K.~S. and {Friedrich}, S. and 
	{Sternberg}, A.},
    title = "{A Close Look at Star Formation around Active Galactic Nuclei}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0704.1374},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Starburst, Infrared: Galaxies},
     year = 2007,
    month = dec,
   volume = 671,
    pages = {1388-1412},
      doi = {10.1086/523032},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...671.1388D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{decin_asr_50_2012,
   author = {{Decin}, L.},
    title = "{Late stages of stellar evolution - Herschel's contributions}",
  journal = {Advances in Space Research},
archivePrefix = "arXiv",
   eprint = {1212.4861},
 primaryClass = "astro-ph.SR",
     year = 2012,
    month = oct,
   volume = 50,
    pages = {843-863},
      doi = {10.1016/j.asr.2012.06.024},
   adsurl = {http://adsabs.harvard.edu/abs/2012AdSpR..50..843D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{decin_aa_548_2012,
   author = {{Decin}, L. and {
}, N.~L.~J. and {Royer}, P. and {Van Marle}, A.~J. and 
	{Vandenbussche}, B. and {Ladjal}, D. and {Kerschbaum}, F. and 
	{Ottensamer}, R. and {Barlow}, M.~J. and {Blommaert}, J.~A.~D.~L. and 
	{Gomez}, H.~L. and {Groenewegen}, M.~A.~T. and {Lim}, T. and 
	{Swinyard}, B.~M. and {Waelkens}, C. and {Tielens}, A.~G.~G.~M.
	},
    title = "{The enigmatic nature of the circumstellar envelope and bow shock surrounding Betelgeuse as revealed by Herschel. I. Evidence of clumps, multiple arcs, and a linear bar-like structure}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1212.4870},
 primaryClass = "astro-ph.SR",
 keywords = {stars: AGB and post-AGB, stars: mass-loss, circumstellar matter, stars: individual: Betelgeuse, methods: numerical, infrared: stars},
     year = 2012,
    month = dec,
   volume = 548,
      eid = {A113},
    pages = {A113},
      doi = {10.1051/0004-6361/201219792},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...548A.113D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dessart_aa_404_2003,
   author = {{Dessart}, L. and {Langer}, N. and {Petrovic}, J.},
    title = "{The impact of radiation and wind momenta on mass transfer  in massive close binary systems}",
  journal = {\aap},
 keywords = {stars: early-type, stars: winds, outflows, stars: binaries: general, hydrodynamics},
     year = 2003,
    month = jun,
   volume = 404,
    pages = {991-996},
      doi = {10.1051/0004-6361:20030534},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...404..991D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{diazmiller_apj_501_1998,
   author = {{Diaz-Miller}, R.~I. and {Franco}, J. and {Shore}, S.~N.},
    title = "{Photoionized and Photodissociated Regions around Main-Sequence Stars}",
  journal = {\apj},
 keywords = {ISM: CLOUDS, ISM: MOLECULES, RADIATIVE TRANSFER, STARS: FORMATION},
     year = 1998,
    month = jul,
   volume = 501,
    pages = {192},
      doi = {10.1086/305793},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...501..192D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dgani_apr_461_1996,
   author = {{Dgani}, R. and {van Buren}, D. and {Noriega-Crespo}, A.},
    title = "{The Transverse Acceleration Instability for Bow Shocks in the Nonlinear Regime}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, INSTABILITIES, SHOCK WAVES, STARS: INDIVIDUAL CONSTELLATION NAME: ALPHA CAMELOPARDALIS, TURBULENCE},
     year = 1996,
    month = apr,
   volume = 461,
    pages = {372},
      doi = {10.1086/177065},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...461..372D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dgani_apj_461_1996,
   author = {{Dgani}, R. and {van Buren}, D. and {Noriega-Crespo}, A.},
    title = "{Stability Analysis of Bow Shocks}",
  journal = {\apj},
 keywords = {SHOCK WAVES, STARS: MASS LOSS},
     year = 1996,
    month = apr,
   volume = 461,
    pages = {927},
      doi = {10.1086/177114},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...461..927D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dopita_aa_29_1973,
   author = {{Dopita}, M.~A.},
    title = "{Photoelectric Photometry of Gaseous Nebulae. I. The Temperature and lonisation Struc- ture of the Orion Nebula}",
  journal = {\aap},
     year = 1973,
    month = dec,
   volume = 29,
    pages = {387},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....29..387D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{draine_apj_285_1984,
   author = {{Draine}, B.~T. and {Lee}, H.~M.},
    title = "{Optical properties of interstellar graphite and silicate grains}",
  journal = {\apj},
 keywords = {GRANULAR MATERIALS, GRAPHITE, INTERSTELLAR MATTER, OPTICAL PROPERTIES, SILICATES, ABSORPTION CROSS SECTIONS, INFRARED ASTRONOMY, OPACITY, PARTICLE INTERACTIONS, SCATTERING CROSS SECTIONS},
     year = 1984,
    month = oct,
   volume = 285,
    pages = {89-108},
      doi = {10.1086/162480},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...285...89D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{durmann_aa_574_2015,
   author = {{D{\"u}rmann}, C. and {Kley}, W.},
    title = "{Migration of massive planets in accreting disks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1411.3190},
 primaryClass = "astro-ph.EP",
 keywords = {protoplanetary disks, planet-disk interactions},
     year = 2015,
    month = feb,
   volume = 574,
      eid = {A52},
    pages = {A52},
      doi = {10.1051/0004-6361/201424837},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...574A..52D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dyson_ass_35_1975,
   author = {{Dyson}, J.~E.},
    title = "{Stellar winds and globules in H II regions}",
  journal = {\apss},
 keywords = {H II REGIONS, PARTICLE INTERACTIONS, SHOCK WAVE PROPAGATION, STELLAR WINDS, ASTRONOMICAL MODELS, GAS FLOW, GLOBULES, STELLAR MASS EJECTION, SUPERSONIC FLOW},
     year = 1975,
    month = jul,
   volume = 35,
    pages = {299-312},
      doi = {10.1007/BF00636999},
   adsurl = {http://adsabs.harvard.edu/abs/1975Ap%26SS..35..299D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dyson_apss_37_1975,
   author = {{Dyson}, J.~E. and {Gulliford}, P.},
    title = "{The dynamical effects of supernovae on the interstellar medium. I - Spherical shock waves in an adiabatic medium}",
  journal = {\apss},
 keywords = {ADIABATIC CONDITIONS, INTERSTELLAR GAS, SHOCK WAVE PROPAGATION, SPHERICAL WAVES, SUPERNOVAE, ASTRONOMICAL MODELS, DYNAMIC MODELS, FINITE DIFFERENCE THEORY, NEBULAE, SHOCK HEATING, STELLAR MASS EJECTION},
     year = 1975,
    month = oct,
   volume = 37,
    pages = {477-498},
      doi = {10.1007/BF00640367},
   adsurl = {http://adsabs.harvard.edu/abs/1975Ap%26SS..37..477D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dwarkadas_apj_630_2005,
   author = {{Dwarkadas}, V.~V.},
    title = "{The Evolution of Supernovae in Circumstellar Wind-Blown Bubbles. I. Introduction and One-Dimensional Calculations}",
  journal = {\apj},
   eprint = {astro-ph/0410464},
 keywords = {Stars: Circumstellar Matter, Hydrodynamics, Shock Waves, ISM: Supernova Remnants, Stars: Supernovae: General, X-Rays: ISM},
     year = 2005,
    month = sep,
   volume = 630,
    pages = {892-910},
      doi = {10.1086/432109},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...630..892D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{dullemond_2012,
   author = {{Dullemond}, C.~P.},
    title = "{RADMC-3D: A multi-purpose radiative transfer tool}",
howpublished = {Astrophysics Source Code Library},
     year = 2012,
    month = feb,
archivePrefix = "ascl",
   eprint = {1202.015},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ascl.soft02015D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dwarkadas_apj_667_2007,
   author = {{Dwarkadas}, V.~V.},
    title = "{The Evolution of Supernovae in Circumstellar Wind Bubbles. II. Case of a Wolf-Rayet Star}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0706.1049},
 keywords = {Hydrodynamics, Instabilities, Shock Waves, Stars: Winds, Outflows, ISM: Supernova Remnants, Stars: Supernovae: General},
     year = 2007,
    month = sep,
   volume = 667,
    pages = {226-247},
      doi = {10.1086/520670},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...667..226D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE E 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{eldridge_mnras_367_2006,
   author = {{Eldridge}, J.~J. and {Genet}, F. and {Daigne}, F. and {Mochkovitch}, R.
	},
    title = "{The circumstellar environment of Wolf-Rayet stars and gamma-ray burst afterglows}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0509749},
 keywords = {circumstellar matter-stars: evolution-stars: winds, outflows-stars: Wolf-Rayet-gamma-rays: bursts},
     year = 2006,
    month = mar,
   volume = 367,
    pages = {186-200},
      doi = {10.1111/j.1365-2966.2005.09938.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.367..186E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{eldridge_mnras_414_2011,
   author = {{Eldridge}, J.~J. and {Langer}, N. and {Tout}, C.~A.},
    title = "{Runaway stars as progenitors of supernovae and gamma-ray bursts}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1103.1877},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: general, stars: evolution, gamma-ray burst: general, stars: massive, supernovae: general, stars: Wolf-Rayet},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {3501-3520},
      doi = {10.1111/j.1365-2966.2011.18650.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.3501E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{elmegreen_apj_229_1979,
   author = {{Elmegreen}, B.~G. and {Morris}, M.},
    title = "{Disk structure in protostellar H2O maser sources}",
  journal = {\apj},
 keywords = {Interstellar Masers, Protostars, Stellar Models, Stellar Structure, Stellar Winds, Water Masers, Infrared Astronomy, Kelvin-Helmholtz Instability, Kepler Laws, Stellar Atmospheres, Stellar Envelopes, Stellar Evolution, Stellar Radiation},
     year = 1979,
    month = apr,
   volume = 229,
    pages = {593-603},
      doi = {10.1086/156994},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJ...229..593E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{evans_iaus_30_1967,
   author = {{Evans}, D.~S.},
    title = "{The Revision of the General Catalogue of Radial Velocities}",
booktitle = {Determination of Radial Velocities and their Applications},
     year = 1967,
   series = {IAU Symposium},
   volume = 30,
   editor = {{Batten}, A.~H. and {Heard}, J.~F.},
    pages = {57},
   adsurl = {http://adsabs.harvard.edu/abs/1967IAUS...30...57E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{everet_apj_713_2010,
   author = {{Everett}, J.~E. and {Churchwell}, E.},
    title = "{Dusty Wind-blown Bubbles}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1003.0838},
 primaryClass = "astro-ph.SR",
 keywords = {dust, extinction, infrared: ISM, ISM: bubbles, stars: individual: N49},
     year = 2010,
    month = apr,
   volume = 713,
    pages = {592-602},
      doi = {10.1088/0004-637X/713/1/592},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713..592E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE F 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{falle_mnras_250_1991,
   author = {{Falle}, S.~A.~E.~G.},
    title = "{Self-similar jets}",
  journal = {\mnras},
 keywords = {EXTRAGALACTIC RADIO SOURCES, GALACTIC STRUCTURE, GAS JETS, RADIO JETS (ASTRONOMY), SUPERSONIC JET FLOW, HYDRODYNAMICS, MATHEMATICAL MODELS},
     year = 1991,
    month = jun,
   volume = 250,
    pages = {581-596},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.250..581F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{federrath_apj_713_2010,
   author = {{Federrath}, C. and {Banerjee}, R. and {Clark}, P.~C. and {Klessen}, R.~S.
	},
    title = "{Modeling Collapse and Accretion in Turbulent Gas Clouds: Implementation and Comparison of Sink Particles in AMR and SPH}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1001.4456},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, ISM: kinematics and dynamics, methods: numerical, shock waves, stars: formation},
     year = 2010,
    month = apr,
   volume = 713,
    pages = {269-290},
      doi = {10.1088/0004-637X/713/1/269},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713..269F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fendt_apj_737_2011,
   author = {{Fendt}, C.},
    title = "{Jet Rotation Driven by Magnetohydrodynamic Shocks in Helical Magnetic Fields}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1105.6232},
 keywords = {ISM: jets and outflows, magnetohydrodynamics: MHD, shock waves, stars: mass-loss},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {43},
    pages = {43},
      doi = {10.1088/0004-637X/737/1/43},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...43F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fendt_apj_774_2013,
   author = {{Fendt}, C. and {Sheikhnezami}, S.},
    title = "{Bipolar Jets Launched from Accretion Disks. II. The Formation of Asymmetric Jets and Counter Jets}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.1263},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, galaxies: active, galaxies: jets, ISM: jets and outflows, magnetohydrodynamics: MHD, stars: protostars},
     year = 2013,
    month = sep,
   volume = 774,
      eid = {12},
    pages = {12},
      doi = {10.1088/0004-637X/774/1/12},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...774...12F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fendt_apj_796_2014,
   author = {{Stepanovs}, D. and {Fendt}, C. and {Sheikhnezami}, S.},
    title = "{Modeling MHD Accretion-Ejection: Episodic Ejections of Jets Triggered by a Mean-field Disk Dynamo}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1409.7003},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, galaxies: jets, ISM: jets and outflows, magnetohydrodynamics: MHD, stars: mass-loss, stars: pre-main sequence },
     year = 2014,
    month = nov,
   volume = 796,
      eid = {29},
    pages = {29},
      doi = {10.1088/0004-637X/796/1/29},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...796...29S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{filipovi_mnras_364_2005,
   author = {{Filipovi{\'c}}, M.~D. and {Payne}, J.~L. and {Reid}, W. and 
	{Danforth}, C.~W. and {Staveley-Smith}, L. and {Jones}, P.~A. and 
	{White}, G.~L.},
    title = "{An ATCA radio-continuum study of the Small Magellanic Cloud - III. Supernova remnants and their environments}",
  journal = {\mnras},
 keywords = {H II regions, supernova remnants, Magellanic Clouds},
     year = 2005,
    month = nov,
   volume = 364,
    pages = {217-236},
      doi = {10.1111/j.1365-2966.2005.09554.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.364..217F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{filippenko_araa_35_1997,
   author = {{Filippenko}, A.~V.},
    title = "{Optical Spectra of Supernovae}",
  journal = {\araa},
     year = 1997,
   volume = 35,
    pages = {309-355},
      doi = {10.1146/annurev.astro.35.1.309},
   adsurl = {http://adsabs.harvard.edu/abs/1997ARA%26A..35..309F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fink_aa_476_2007,
   author = {{Fink}, M. and {Hillebrandt}, W. and {R{\"o}pke}, F.~K.},
    title = "{Double-detonation supernovae of sub-Chandrasekhar mass white dwarfs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0710.5486},
 keywords = {supernovae: general, nuclear reactions, nucleosynthesis, , abundances, hydrodynamics, methods: numerical},
     year = 2007,
    month = dec,
   volume = 476,
    pages = {1133-1143},
      doi = {10.1051/0004-6361:20078438},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...476.1133F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{frail_aj_111_1996,
   author = {{Frail}, D.~A. and {Goss}, W.~M. and {Reynoso}, E.~M. and {Giacani}, E.~B. and 
	{Green}, A.~J. and {Otrupcek}, R.},
    title = "{A Survey for OH (1720 MHz) Maser Emission Toward Supernova Remnants}",
  journal = {\aj},
 keywords = {SUPERNOVA REMNANTS, MASERS, CIRCUMSTELLAR MATTER, ISM: CLOUDS},
     year = 1996,
    month = apr,
   volume = 111,
    pages = {1651},
      doi = {10.1086/117904},
   adsurl = {http://adsabs.harvard.edu/abs/1996AJ....111.1651F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{frank_prpl_451_2014,
   author = {{Frank}, A. and {Ray}, T.~P. and {Cabrit}, S. and {Hartigan}, P. and 
	{Arce}, H.~G. and {Bacciotti}, F. and {Bally}, J. and {Benisty}, M. and 
	{Eisl{\"o}ffel}, J. and {G{\"u}del}, M. and {Lebedev}, S. and 
	{Nisini}, B. and {Raga}, A.},
    title = "{Jets and Outflows from Star to Cloud: Observations Confront Theory}",
  journal = {Protostars and Planets VI},
archivePrefix = "arXiv",
   eprint = {1402.3553},
 primaryClass = "astro-ph.SR",
     year = 2014,
    pages = {451-474},
      doi = {10.2458/azu_uapress_9780816531240-ch020},
   adsurl = {http://adsabs.harvard.edu/abs/2014prpl.conf..451F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{franco_pasp_103_1991,
   author = {{Franco}, J. and {Tenorio-Tagle}, G. and {Bodenheimer}, P. and 
	{Rozyczka}, M.},
    title = "{Evolution of supernova remnants inside preexisting wind-driven cavities}",
  journal = {\pasp},
 keywords = {CAVITIES, EJECTA, SHOCK WAVES, STELLAR EVOLUTION, STELLAR WINDS, SUPERNOVA REMNANTS, LIGHT EMISSION, STELLAR MASS EJECTION, X RAY SOURCES},
     year = 1991,
    month = aug,
   volume = 103,
    pages = {803-810},
      doi = {10.1086/132884},
   adsurl = {http://adsabs.harvard.edu/abs/1991PASP..103..803F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ferreira_478_aa_2008,
   author = {{Ferreira}, S.~E.~S. and {de Jager}, O.~C.},
    title = "{Supernova remnant evolution in uniform and non-uniform media}",
  journal = {\aap},
 keywords = {stars: supernovae: general, ISM: supernovae remnants, methods: numerical, magnetohydrodynamics (MHD), shock waves, ISM: cosmic rays},
     year = 2008,
    month = jan,
   volume = 478,
    pages = {17-29},
      doi = {10.1051/0004-6361:20077824},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...478...17F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fontani_aa_593_2016,
   author = {{Fontani}, F. and {Commer{\c c}on}, B. and {Giannetti}, A. and 
	{Beltr{\'a}n}, M.~T. and {S{\'a}nchez-Monge}, A. and {Testi}, L. and 
	{Brand}, J. and {Caselli}, P. and {Cesaroni}, R. and {Dodson}, R. and 
	{Longmore}, S. and {Rioja}, M. and {Tan}, J.~C. and {Walmsley}, C.~M.
	},
    title = "{Magnetically regulated fragmentation of a massive, dense, and turbulent clump}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1608.08083},
 keywords = {stars: formation, submillimeter: ISM, ISM: molecules, ISM: individual objects: IRAS 16061-5048c1},
     year = 2016,
    month = sep,
   volume = 593,
      eid = {L14},
    pages = {L14},
      doi = {10.1051/0004-6361/201629442},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...593L..14F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{foglizzo_apj_654_2007,
   author = {{Foglizzo}, T. and {Galletti}, P. and {Scheck}, L. and {Janka}, H.-T.
	},
    title = "{Instability of a Stalled Accretion Shock: Evidence for the Advective-Acoustic Cycle}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0606640},
 keywords = {Accretion, Accretion Disks, Hydrodynamics, Instabilities, Shock Waves, Stars: Supernovae: General},
     year = 2007,
    month = jan,
   volume = 654,
    pages = {1006-1021},
      doi = {10.1086/509612},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...654.1006F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{forgan_mnras_463_2016,
   author = {{Forgan}, D.~H. and {Ilee}, J.~D. and {Cyganowski}, C.~J. and 
	{Brogan}, C.~L. and {Hunter}, T.~R.},
    title = "{Self-gravitating disc candidates around massive young stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1608.05539},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: massive, stars: pre-main-sequence, stars: protostars, radio continuum: stars, submillimetre: stars},
     year = 2016,
    month = nov,
   volume = 463,
    pages = {957-964},
      doi = {10.1093/mnras/stw1917},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.463..957F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{forgan_mnras_420_2012,
   author = {{Forgan}, D. and {Rice}, K.},
    title = "{A lower angular momentum limit for self-gravitating protostellar disc fragmentation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1110.4212},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, hydrodynamics, radiative transfer, methods: numerical, stars: formation},
     year = 2012,
    month = feb,
   volume = 420,
    pages = {299-308},
      doi = {10.1111/j.1365-2966.2011.20034.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420..299F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{forgen_mntas_410_2011,
   author = {{Forgan}, D. and {Rice}, K. and {Cossins}, P. and {Lodato}, G.
	},
    title = "{The nature of angular momentum transport in radiative self-gravitating protostellar discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1008.1547},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, gravitation, instabilities, stars: formation, stars: general},
     year = 2011,
    month = jan,
   volume = 410,
    pages = {994-1006},
      doi = {10.1111/j.1365-2966.2010.17500.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.410..994F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fuente_aa_366_2001,
   author = {{Fuente}, A. and {Neri}, R. and {Mart{\'{\i}}n-Pintado}, J. and 
	{Bachiller}, R. and {Rodr{\'{\i}}guez-Franco}, A. and {Palla}, F.
	},
    title = "{Disks and outflows around intermediate-mass stars and protostars}",
  journal = {\aap},
 keywords = {STARS: FORMATION, FUNDAMENTAL PARAMETERS, PRE-MAIN SEQUENCE, ISM: ABUNDANCES, CLOUDS, MOLECULES},
     year = 2001,
    month = feb,
   volume = 366,
    pages = {873-890},
      doi = {10.1051/0004-6361:20000358},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...366..873F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE G 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@PHDTHESIS{gaensler_phd_1999,
   author = {{Gaensler}, B.~M.},
    title = "{Barrels, jets and smoke-rings: Understanding the bizarre shapes of radio supernova remnants}",
   school = {University of Sydney},
     year = 1999,
    month = May,
   adsurl = {http://adsabs.harvard.edu/abs/1999PhDT..........G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gaetz_apjs_155_1983,
   author = {{Gaetz}, T.~J. and {Salpeter}, E.~E.},
    title = "{Line radiation from a hot, optically thin plasma - Collision strengths and emissivities}",
  journal = {\apjs},
 keywords = {COLLISION RATES, EMISSIVITY, HIGH TEMPERATURE PLASMAS, LINE SPECTRA, PLASMA RADIATION, SOLAR CORONA, SUPERNOVA REMNANTS, ATOMIC COLLISIONS, COSMIC PLASMA, ELECTRON TRANSITIONS, FINE STRUCTURE, OPTICAL THICKNESS, TABLES (DATA), TEMPERATURE DEPENDENCE},
     year = 1983,
    month = jun,
   volume = 52,
    pages = {155-168},
      doi = {10.1086/190862},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJS...52..155G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gaensler_apj_493_1998,
   author = {{Gaensler}, B.~M.},
    title = "{The Nature of Bilateral Supernova Remnants}",
  journal = {\apj},
   eprint = {astro-ph/9707149},
 keywords = {ISM: STRUCTURE, ISM: INDIVIDUAL ALPHANUMERIC: G003.7-00.2, ISM: INDIVIDUAL ALPHANUMERIC: G350.0-02.0, ISM: MAGNETIC FIELDS, ISM: SUPERNOVA REMNANTS, RADIO CONTINUUM: ISM, ISM: Individual: Alphanumeric: G003.7-00.2, ISM: Individual: Alphanumeric: G350.0-02.0, ISM: Magnetic Fields, ISM: Structure, Radio Continuum: ISM, ISM: Supernova Remnants},
     year = 1998,
    month = jan,
   volume = 493,
    pages = {781-792},
      doi = {10.1086/305146},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...493..781G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gammie_apj_462_1996,
   author = {{Gammie}, C.~F.},
    title = "{Linear Theory of Magnetized, Viscous, Self-gravitating Gas Disks}",
  journal = {\apj},
 keywords = {GALAXIES: ISM, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: STRUCTURE, ISM: MAGNETIC FIELDS},
     year = 1996,
    month = may,
   volume = 462,
    pages = {725},
      doi = {10.1086/177185},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...462..725G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_1996_aa_316,
   author = {{Garcia-Segura}, G. and {Langer}, N. and {Mac Low}, M.-M.},
    title = "{The hydrodynamic evolution of circumstellar gas around massive stars. II. The impact of the time sequence O star -{\gt} RSG -{\gt} WR star.}",
  journal = {\aap},
 keywords = {HYDRODYNAMICS, STARS: MASS LOSS, ISM: BUBBLES, STARS: WOLF-RAYET, SUPERGIANTS, STARS: EVOLUTION},
     year = 1996,
    month = dec,
   volume = 316,
    pages = {133-146},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...316..133G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_1996_aa_305,
   author = {{Garcia-Segura}, G. and {Mac Low}, M.-M. and {Langer}, N.},
    title = "{The dynamical evolution of circumstellar gas around massive stars. I. The impact of the time sequence Ostar -{\gt} LBV -{\gt} WR star.}",
  journal = {\aap},
 keywords = {HYDRODYNAMICS, STARS: EVOLUTION, MASS LOSS, STARS: WOLF-RAYET, ISM: BUBBLES, ISM: INDIVIDUAL (RCW 58)},
     year = 1996,
    month = jan,
   volume = 305,
    pages = {229},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...305..229G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_apj_517_1999,
   author = {{Garc{\'{\i}}a-Segura}, G. and {Langer}, N. and {R{\'o}{\.z}yczka}, M. and 
	{Franco}, J.},
    title = "{Shaping Bipolar and Elliptical Planetary Nebulae: Effects of Stellar Rotation, Photoionization Heating, and Magnetic Fields}",
  journal = {\apj},
 keywords = {ISM: MAGNETIC FIELDS, ISM: STRUCTURE, MAGNETOHYDRODYNAMICS: MHD, ISM: PLANETARY NEBULAE: GENERAL, STARS: AGB AND POST-AGB, STARS: MASS LOSS},
     year = 1999,
    month = jun,
   volume = 517,
    pages = {767-781},
      doi = {10.1086/307205},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...517..767G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_aa_455_1995a,
   author = {{Garcia-Segura}, G. and {Mac Low}, M.-M.},
    title = "{Wolf-Rayet Bubbles. I. Analytic Solutions}",
  journal = {\apj},
 keywords = {ISM: BUBBLES, ISM: INDIVIDUAL NGC NUMBER: NGC 6888, ISM: STRUCTURE, STARS: MASS LOSS, STARS: WOLF-RAYET},
     year = 1995,
    month = dec,
   volume = 455,
    pages = {145},
      doi = {10.1086/176563},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...455..145G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_aa_455_1995b,
   author = {{Garcia-Segura}, G. and {Mac Low}, M.-M.},
    title = "{Wolf-Rayet Bubbles. II. Gasdynamical Simulations}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, ISM: BUBBLES, STARS: MASS LOSS, STARS: WOLF-RAYET},
     year = 1995,
    month = dec,
   volume = 455,
    pages = {160},
      doi = {10.1086/176564},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...455..160G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garmany_apj_242_1980,
   author = {{Garmany}, C.~D. and {Conti}, P.~S. and {Massey}, P.},
    title = "{Spectroscopic studies of O type stars. IX - Binary frequency}",
  journal = {\apj},
 keywords = {ASTRONOMICAL SPECTROSCOPY, BINARY STARS, EARLY STARS, O STARS, X RAY SOURCES, MASS RATIOS, STELLAR LUMINOSITY, STELLAR MOTIONS, TABLES (DATA)},
     year = 1980,
    month = dec,
   volume = 242,
    pages = {1063-1076},
      doi = {10.1086/158537},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...242.1063G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gies_apjs_64_1987,
   author = {{Gies}, D.~R.},
    title = "{The kinematical and binary properties of association and field O stars}",
  journal = {\apjs},
 keywords = {ASTRONOMICAL CATALOGS, BINARY STARS, MILKY WAY GALAXY, O STARS, STELLAR MOTIONS, VELOCITY DISTRIBUTION, EARLY STARS, GRAVITATIONAL EFFECTS, RADIAL VELOCITY, STAR CLUSTERS, STELLAR GRAVITATION},
     year = 1987,
    month = jul,
   volume = 64,
    pages = {545-563},
      doi = {10.1086/191208},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJS...64..545G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{giuliani_apj_277_1984,
   author = {{Giuliani}, Jr., J.~L.},
    title = "{On the dynamics in evaporating cloud envelopes}",
  journal = {\apj},
 keywords = {ASTROPHYSICS, CLOUDS, HYDRODYNAMICS, INTERSTELLAR GAS, HYDRODYNAMIC EQUATIONS, INVISCID FLOW, SHOCK WAVES, VISCOUS FLOW},
     year = 1984,
    month = feb,
   volume = 277,
    pages = {605-614},
      doi = {10.1086/161731},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...277..605G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{graham_apj_179_1973,
   author = {{Graham}, R. and {Langer}, W.~D.},
    title = "{Pressure Equilibrium of Finite-Size Clouds in the Interstellar Medium}",
  journal = {\apj},
     year = 1973,
    month = jan,
   volume = 179,
    pages = {469-482},
      doi = {10.1086/151887},
   adsurl = {http://adsabs.harvard.edu/abs/1973ApJ...179..469G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{green_lnp_598_2003,
   author = {{Green}, D.~A. and {Stephenson}, F.~R.},
    title = "{Historical Supernovae}",
booktitle = {Supernovae and Gamma-Ray Bursters},
     year = 2003,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 598,
   eprint = {astro-ph/0301603},
   editor = {{Weiler}, K.},
    pages = {7-19},
   adsurl = {http://adsabs.harvard.edu/abs/2003LNP...598....7G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{green_cat_2009,
   author = {{Green}, D.~A.},
    title = "{A Catalogue of Galactic Supernova Remnants (Green, 2009)}",
  journal = {VizieR Online Data Catalog},
 keywords = {Supernova remnants, Milky Way, Nonstellar objects},
     year = 2009,
    month = jun,
   volume = 7253,
    pages = {0},
   adsurl = {http://adsabs.harvard.edu/abs/2009yCat.7253....0G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{greif_mnras_424_2012,
   author = {{Greif}, T.~H. and {Bromm}, V. and {Clark}, P.~C. and {Glover}, S.~C.~O. and 
	{Smith}, R.~J. and {Klessen}, R.~S. and {Yoshida}, N. and {Springel}, V.
	},
    title = "{Formation and evolution of primordial protostellar systems}",
  journal = {\mnras},
 keywords = {hydrodynamics, stars: formation, galaxies: high-redshift, cosmology: theory, early Universe},
     year = 2012,
    month = jul,
   volume = 424,
    pages = {399-415},
      doi = {10.1111/j.1365-2966.2012.21212.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424..399G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{greif_apj_737_2011,
   author = {{Greif}, T.~H. and {Springel}, V. and {White}, S.~D.~M. and 
	{Glover}, S.~C.~O. and {Clark}, P.~C. and {Smith}, R.~J. and 
	{Klessen}, R.~S. and {Bromm}, V.},
    title = "{Simulations on a Moving Mesh: The Clustered Formation of Population III Protostars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1101.5491},
 keywords = {cosmology: theory, early universe, hydrodynamics, methods: numerical, stars: formation},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {75},
    pages = {75},
      doi = {10.1088/0004-637X/737/2/75},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...75G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{groh_aa_564_2014,
   author = {{Groh}, J.~H. and {Meynet}, G. and {Ekstr{\"o}m}, S. and {Georgy}, C.
	},
    title = "{The evolution of massive stars and their spectra. I. A non-rotating 60 M$_{⊙}$ star from the zero-age main sequence to the pre-supernova stage}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1401.7322},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: atmospheres, stars: mass-loss, stars: massive, supernovae: general, stars: winds, outflows},
     year = 2014,
    month = apr,
   volume = 564,
      eid = {A30},
    pages = {A30},
      doi = {10.1051/0004-6361/201322573},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...564A..30G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{grunhut_mnras_400_2009,
   author = {{Grunhut}, J.~H. and {Wade}, G.~A. and {Marcolino}, W.~L.~F. and 
	{Petit}, V. and {Henrichs}, H.~F. and {Cohen}, D.~H. and {Alecian}, E. and 
	{Bohlender}, D. and {Bouret}, J.-C. and {Kochukhov}, O. and 
	{Neiner}, C. and {St-Louis}, N. and {Townsend}, R.~H.~D.},
    title = "{Discovery of a magnetic field in the O9 sub-giant star HD 57682 by the MiMeS Collaboration}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0910.0214},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type , stars: individual: HD 57682 , stars: magnetic fields , stars: rotation , stars: winds, outflows},
     year = 2009,
    month = nov,
   volume = 400,
    pages = {L94-L98},
      doi = {10.1111/j.1745-3933.2009.00771.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.400L..94G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gotthelf_apj_552_2001,
   author = {{Gotthelf}, E.~V. and {Koralesky}, B. and {Rudnick}, L. and 
	{Jones}, T.~W. and {Hwang}, U. and {Petre}, R.},
    title = "{Chandra Detection of the Forward and Reverse Shocks in Cassiopeia A}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0104161},
 keywords = {ISM: Supernova Remnants, Stars: Supernovae: Individual: Name: Cassiopeia A, X-Rays: General},
     year = 2001,
    month = may,
   volume = 552,
    pages = {L39-L43},
      doi = {10.1086/320250},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...552L..39G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{guarcello_aa_521_2010,
   author = {{Guarcello}, M.~G. and {Micela}, G. and {Peres}, G. and {Prisinzano}, L. and 
	{Sciortino}, S.},
    title = "{Chronology of star formation and disk evolution in the Eagle Nebula}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1008.0422},
 primaryClass = "astro-ph.SR",
 keywords = {protoplanetary disks, stars: formation, stars: pre-main sequence, infrared: stars: X-rays: stars},
     year = 2010,
    month = oct,
   volume = 521,
      eid = {A61},
    pages = {A61},
      doi = {10.1051/0004-6361/201014351},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...521A..61G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gonzalezcasanova_apj_781_2014,
   author = {{Gonz{\'a}lez-Casanova}, D.~F. and {De Colle}, F. and {Ramirez-Ruiz}, E. and 
	{Lopez}, L.~A.},
    title = "{The Morphology and Dynamics of Jet-driven Supernova Remnants: The Case of W49B}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1309.7049},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, ISM: individual objects: W49B G43.3{\ndash}0.2, ISM: supernova remnants, methods: numerical, nuclear reactions, nucleosynthesis, abundances},
     year = 2014,
    month = feb,
   volume = 781,
      eid = {L26},
    pages = {L26},
      doi = {10.1088/2041-8205/781/2/L26},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...781L..26G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gull_apj_230_1979,
   author = {{Gull}, T.~R. and {Sofia}, S.},
    title = "{Discovery of two distorted interstellar bubbles}",
  journal = {\apj},
 keywords = {INTERSTELLAR GAS, NEBULAE, ORION NEBULA, ASTRONOMICAL SPECTROSCOPY, GALACTIC STRUCTURE, STELLAR LUMINOSITY, STELLAR MASS EJECTION},
     year = 1979,
    month = jun,
   volume = 230,
    pages = {782-785},
      doi = {10.1086/157137},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJ...230..782G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{gusdorf_iaus_296_2014,
   author = {{Gusdorf}, A. and {G{\"u}sten}, R. and {Anderl}, S. and {Hezareh}, T. and 
	{Wiesemeyer}, H.},
    title = "{The molecular emission from old supernova remnants}",
 keywords = {ISM: supernova remnants, Shock waves, Submillimeter: ISM, ISM: individual objects: W28, IC443 {\amp} 3C391, Stars: formation, cosmic rays,},
booktitle = {IAU Symposium},
     year = 2014,
   series = {IAU Symposium},
   volume = 296,
archivePrefix = "arXiv",
   eprint = {1403.5909},
   editor = {{Ray}, A. and {McCray}, R.~A.},
    month = jan,
    pages = {178-182},
      doi = {10.1017/S1743921313009435},
   adsurl = {http://adsabs.harvard.edu/abs/2014IAUS..296..178G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_424_mnras_2012,
   author = {{Gvaramadze}, V.~V. and {Weidner}, C. and {Kroupa}, P. and {Pflamm-Altenburg}, J.
	},
    title = "{Field O stars: formed in situ or as runaways?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1206.1596},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, stars: formation, stars: kinematics and dynamics, stars: massive, Magellanic Clouds, galaxies: star formation },
     year = 2012,
    month = aug,
   volume = 424,
    pages = {3037-3049},
      doi = {10.1111/j.1365-2966.2012.21452.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424.3037G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gvaramadze_aa_490_2008,
   author = {{Gvaramadze}, V.~V. and {Bomans}, D.~J.},
    title = "{Search for OB stars running away from young star clusters. I. NGC 6611}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0809.0650},
 keywords = {stars: individual: BD-14{\deg} 5040, stars: individual: HD 165319, open clusters and associations: general, open clusters and associations: individual: NGC 6611, ISM: individual objects: RCW 158},
     year = 2008,
    month = nov,
   volume = 490,
    pages = {1071-1077},
      doi = {10.1051/0004-6361:200810411},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...490.1071G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_aa_535_2011,
   author = {{Gvaramadze}, V.~V. and {Kniazev}, A.~Y. and {Kroupa}, P. and 
	{Oh}, S.},
    title = "{Search for OB stars running away from young star clusters. II. The NGC 6357 star-forming region}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.2116},
 primaryClass = "astro-ph.SR",
 keywords = {stars: kinematics and dynamics, stars: massive, open clusters and associations: general, open clusters and associations: individual: AH03 J1725-34.4, ISM: individual objects: NGC 6357},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A29},
    pages = {A29},
      doi = {10.1051/0004-6361/201117746},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...535A..29G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_mnras_410_2011,
   author = {{Gvaramadze}, V.~V. and {Gualandris}, A.},
    title = "{Very massive runaway stars from three-body encounters}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1007.5057},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, binaries: general, stars: individual: {$\lambda$} Cep, BD+43{\deg}3654, Sk -67{\deg}22, BI 237, 30 Dor 016, HD269928, stars: kinematics and dynamics, galaxies: star clusters: individual: 30 Doradus},
     year = 2011,
    month = jan,
   volume = 410,
    pages = {304-312},
      doi = {10.1111/j.1365-2966.2010.17446.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.410..304G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_aa_529_2011,
   author = {{Gvaramadze}, V.~V. and {R{\"o}ser}, S. and {Scholz}, R.-D. and 
	{Schilbach}, E.},
    title = "{4U 1907+09: an HMXB running away from the Galactic plane}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1102.2437},
 primaryClass = "astro-ph.SR",
 keywords = {proper motions, stars: early-type, stars: kinematics and dynamics, stars: individual: 4U 1907+09, stars: individual: Vela X-1, X-rays: binaries},
     year = 2011,
    month = may,
   volume = 529,
      eid = {A14},
    pages = {A14},
      doi = {10.1051/0004-6361/201016256},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529A..14G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_mnras_427_2012,
   author = {{Gvaramadze}, V.~V. and {Langer}, N. and {Mackey}, J.},
    title = "{{$\zeta$} Oph and the weak-wind problem}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.0455},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: {$\zeta$} Oph, stars: mass-loss, stars: winds, outflows, H II regions},
     year = 2012,
    month = nov,
   volume = 427,
    pages = {L50-L54},
      doi = {10.1111/j.1745-3933.2012.01343.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427L..50G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gvaramadze_2013,
   author = {{Gvaramadze}, V.~V. and {Menten}, K.~M. and {Kniazev}, A.~Y. and 
	{Langer}, N. and {Mackey}, J. and {Kraus}, A. and {Meyer}, D.~M.-A. and 
	{Kami{\'n}ski}, T.},
    title = "{IRC -10414: a bow-shock-producing red supergiant star}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.2245},
 primaryClass = "astro-ph.SR",
 keywords = {masers, shock waves, circumstellar matter, stars: individual: IRC -10414, stars: kinematics and dynamics, stars: massive},
     year = 2014,
    month = jan,
   volume = 437,
    pages = {843-856},
      doi = {10.1093/mnras/stt1943},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.437..843G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE H 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{harries_2017,
   author = {{Harries}, T.~J and {Douglas}, T.~A and {Ali}, A.},
    title = "{Radiation-hydrodynamical simulations of massive star formation using Monte Carlo radiative transfer II. The formation of a 25 solar-mass star}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1706.04017},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170604017H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{harries_mnras_448_2015,
   author = {{Harries}, T.~J.},
    title = "{Radiation-hydrodynamical simulations of massive star formation using Monte Carlo radiative transfer - I. Algorithms and numerical methods}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1501.05754},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, stars: formation},
     year = 2015,
    month = apr,
   volume = 448,
    pages = {3156-3166},
      doi = {10.1093/mnras/stv158},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.448.3156H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{haikala_aa_431_2005,
   author = {{Haikala}, L.~K. and {Harju}, J. and {Mattila}, K. and {Toriseva}, M.
	},
    title = "{Clumpy filaments of the Chamaeleon I cloud: C$^{18}$O mapping with the SEST}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0407608},
 keywords = {ISM: clouds, ISM: molecules, ISM: structure, ISM: individual objects: Chamaeleon I},
     year = 2005,
    month = feb,
   volume = 431,
    pages = {149-163},
      doi = {10.1051/0004-6361:200400057},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...431..149H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heiner_mnras_452_2015,
   author = {{Heiner}, J.~S. and {V{\'a}zquez-Semadeni}, E. and {Ballesteros-Paredes}, J.
	},
    title = "{Molecular cloud formation as seen in synthetic H I and molecular gas observations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1403.6417},
 keywords = {turbulence, ISM: clouds, ISM: evolution, ISM: kinematics and dynamics, ISM: structure},
     year = 2015,
    month = sep,
   volume = 452,
    pages = {1353-1374},
      doi = {10.1093/mnras/stv1153},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.452.1353H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hennebelle_apj_830_2016,
   author = {{Hennebelle}, P. and {Commer{\c c}on}, B. and {Chabrier}, G. and 
	{Marchand}, P.},
    title = "{Magnetically Self-regulated Formation of Early Protoplanetary Disks}",
  journal = {\apjl},
 keywords = {diffusion, gravitation, hydrodynamics, magnetohydrodynamics: MHD, protoplanetary disks, turbulence },
     year = 2016,
    month = oct,
   volume = 830,
      eid = {L8},
    pages = {L8},
      doi = {10.3847/2041-8205/830/1/L8},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...830L...8H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heger_apj_apj_2000,
   author = {{Heger}, A. and {Langer}, N. and {Woosley}, S.~E.},
    title = "{Presupernova Evolution of Rotating Massive Stars. I. Numerical Method and Evolution of the Internal Stellar Structure}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9904132},
 keywords = {HYDRODYNAMICS, METHODS: NUMERICAL, STARS EARLY-TYPE, STARS: EVOLUTION, STARS: INTERIORS, STARS ROTATION},
     year = 2000,
    month = jan,
   volume = 528,
    pages = {368-396},
      doi = {10.1086/308158},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...528..368H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{henney_mnras_398_2009,
   author = {{Henney}, W.~J. and {Arthur}, S.~J. and {de Colle}, F. and {Mellema}, G.
	},
    title = "{Radiation-magnetohydrodynamic simulations of the photoionization of magnetized globules}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0810.1531},
 keywords = {MHD , stars: formation , ISM: globules , HII regions},
     year = 2009,
    month = sep,
   volume = 398,
    pages = {157-175},
      doi = {10.1111/j.1365-2966.2009.15153.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.398..157H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{haemmerle_aa_602_2017,
   author = {{Haemmerl{\'e}}, L. and {Eggenberger}, P. and {Meynet}, G. and 
	{Maeder}, A. and {Charbonnel}, C. and {Klessen}, R.~S.},
    title = "{Massive star formation by accretion. II. Rotation: how to circumvent the angular momentum barrier?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1703.08357},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: evolution, accretion, accretion disks, stars: rotation, stars: massive, stars: pre-main sequence},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {A17},
    pages = {A17},
      doi = {10.1051/0004-6361/201630149},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017A%26A...602A..17H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{haemmerle_585_aa_2016,
   author = {{Haemmerl{\'e}}, L. and {Eggenberger}, P. and {Meynet}, G. and 
	{Maeder}, A. and {Charbonnel}, C.},
    title = "{Massive star formation by accretion. I. Disc accretion}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1511.07640},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: evolution, accretion, accretion disks},
     year = 2016,
    month = jan,
   volume = 585,
      eid = {A65},
    pages = {A65},
      doi = {10.1051/0004-6361/201527202},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...585A..65H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hirsch_apj_757_2012,
   author = {{Hirsch}, L. and {Adams}, J.~D. and {Herter}, T.~L. and {Hora}, J.~L. and 
	{De Buizer}, J.~M. and {Megeath}, S.~T. and {Gull}, G.~E. and 
	{Henderson}, C.~P. and {Keller}, L.~D. and {Schoenwald}, J. and 
	{Vacca}, W.},
    title = "{SOFIA/FORCAST and Spitzer/IRAC Imaging of the Ultracompact H II Region W3(OH) and Associated Protostars in W3}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1208.4124},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, H II regions, infrared: stars, radiative transfer, stars: formation},
     year = 2012,
    month = oct,
   volume = 757,
      eid = {113},
    pages = {113},
      doi = {10.1088/0004-637X/757/2/113},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757..113H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heemskerk_aa_260_1992,
   author = {{Heemskerk}, M.~H.~M. and {Papaloizou}, J.~C. and {Savonije}, G.~J.
	},
    title = "{Non-linear development of M = 1 instabilities in a self-gravitating gaseous disc}",
  journal = {\aap},
 keywords = {Accretion Disks, Hydrodynamic Equations, Perturbation Theory, Stellar Gravitation, Stellar Mass, Center Of Mass, Nonlinear Equations, Pressure Oscillations},
     year = 1992,
    month = jul,
   volume = 260,
    pages = {161-174},
   adsurl = {http://adsabs.harvard.edu/abs/1992A%26A...260..161H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hibbs_360_mnras_2005,
   author = {{Hobbs}, G. and {Lorimer}, D.~R. and {Lyne}, A.~G. and {Kramer}, M.
	},
    title = "{A statistical study of 233 pulsar proper motions}",
  journal = {\mnras},
   eprint = {astro-ph/0504584},
 keywords = {stars: kinematics, pulsars: general},
     year = 2005,
    month = jul,
   volume = 360,
    pages = {974-992},
      doi = {10.1111/j.1365-2966.2005.09087.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.360..974H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hennebelle_aa_528_2011,
   author = {{Hennebelle}, P. and {Commer{\c c}on}, B. and {Joos}, M. and 
	{Klessen}, R.~S. and {Krumholz}, M. and {Tan}, J.~C. and {Teyssier}, R.
	},
    title = "{Collapse, outflows and fragmentation of massive, turbulent and magnetized prestellar barotropic cores}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.1574},
 keywords = {magnetohydrodynamics (MHD), instabilities, ISM: kinematics and dynamics, ISM: clouds, stars: formation},
     year = 2011,
    month = apr,
   volume = 528,
      eid = {A72},
    pages = {A72},
      doi = {10.1051/0004-6361/201016052},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...528A..72H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hosokawa_apj_691_2009,
   author = {{Hosokawa}, T. and {Omukai}, K.},
    title = "{Evolution of Massive Protostars with High Accretion Rates}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0806.4122},
 keywords = {accretion, accretion disks, stars: early-type, stars: evolution, stars: formation, stars: pre-main sequence},
     year = 2009,
    month = jan,
   volume = 691,
    pages = {823-846},
      doi = {10.1088/0004-637X/691/1/823},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691..823H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hollenbach_apj_342_1989,
   author = {{Hollenbach}, D. and {McKee}, C.~F.},
    title = "{Molecule formation and infrared emission in fast interstellar shocks. III - Results for J shocks in molecular clouds}",
  journal = {\apj},
 keywords = {EMISSION SPECTRA, INFRARED SOURCES (ASTRONOMY), INTERSTELLAR CHEMISTRY, MOLECULAR CLOUDS, SHOCK FRONTS, COSMIC RAYS, FINE STRUCTURE, HERBIG-HARO OBJECTS, MOLECULAR GASES, SUPERNOVA REMNANTS, WATER MASERS},
     year = 1989,
    month = jul,
   volume = 342,
    pages = {306-336},
      doi = {10.1086/167595},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...342..306H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hummer_mnras_268_1994,
   author = {{Hummer}, D.~G.},
    title = "{Total Recombination and Energy Loss Coefficients for Hydrogenic Ions at Low Density for 10{\lt}T/E/Z/2{\lt}10/7K}",
  journal = {\mnras},
 keywords = {atomic data},
     year = 1994,
    month = may,
   volume = 268,
    pages = {109},
   adsurl = {http://adsabs.harvard.edu/abs/1994MNRAS.268..109H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{huthoff_aa_383_2002,
   author = {{Huthoff}, F. and {Kaper}, L.},
    title = "{On the absence of wind bow-shocks around OB-runaway stars: Probing the physical conditions of the interstellar medium}",
  journal = {\aap},
   eprint = {astro-ph/0112428},
 keywords = {STARS: EARLY-TYPE, STARS: KINEMATICS, STARS: MASS LOSS, ISM: BUBBLES, ISM: STRUCTURE -$\backslash$ X-RAYS: BINARIES},
     year = 2002,
    month = mar,
   volume = 383,
    pages = {999-1010},
      doi = {10.1051/0004-6361:20011793},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...383..999H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{neilson_apj_684_2008,
   author = {{Neilson}, H.~R. and {Lester}, J.~B.},
    title = "{On the Enhancement of Mass Loss in Cepheids Due to Radial Pulsation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0803.4198},
 keywords = {Stars: Variables: Cepheids, Stars: Circumstellar Matter, Stars: Mass Loss},
     year = 2008,
    month = sep,
   volume = 684,
    pages = {569-587},
      doi = {10.1086/588650},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...684..569N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{neilson_apj_690_2009,
   author = {{Neilson}, H.~R. and {Lester}, J.~B.},
    title = "{On the Enhancement of Mass Loss in Cepheids due to Radial Pulsation. II. The Effect of Metallicity}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.2793},
 keywords = {Cepheids, circumstellar matter, Magellanic Clouds, stars: mass loss},
     year = 2009,
    month = jan,
   volume = 690,
    pages = {1829-1838},
      doi = {10.1088/0004-637X/690/2/1829},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690.1829N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hollenbach_apj_208_1976,
   author = {{Hollenbach}, D. and {Chu}, S.-I. and {McCray}, R.},
    title = "{H2 in expanding circumstellar shells}",
  journal = {\apj},
 keywords = {EARLY STARS, HYDROGEN, MOLECULAR GASES, STELLAR ENVELOPES, GAS DENSITY, MOLECULAR EXCITATION, MOLECULAR ROTATION, STELLAR MODELS, STELLAR WINDS},
     year = 1976,
    month = sep,
   volume = 208,
    pages = {458-467},
      doi = {10.1086/154627},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...208..458H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hollenbach_apj_41_1979,
   author = {{Hollenbach}, D. and {McKee}, C.~F.},
    title = "{Molecule formation and infrared emission in fast interstellar shocks. I Physical processes}",
  journal = {\apjs},
 keywords = {ASTROPHYSICS, INFRARED RADIATION, INTERSTELLAR GAS, MOLECULAR GASES, SHOCK WAVES, CHEMICAL REACTIONS, DEUTERIUM, GAS DENSITY, GAS DISSOCIATION, GAS TEMPERATURE, MOLECULAR INTERACTIONS, SHOCK FRONTS},
     year = 1979,
    month = nov,
   volume = 41,
    pages = {555-592},
      doi = {10.1086/190631},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJS...41..555H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{hosokawa_2015,
   author = {{Hosokawa}, T. and {Hirano}, S. and {Kuiper}, R. and {Yorke}, H.~W. and 
	{Omukai}, K. and {Yoshida}, N.},
    title = "{Formation of Massive Primordial Stars: Intermittent UV Feedback with Episodic Mass Accretion}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1510.01407},
 keywords = {accretion, accretion disks, cosmology: theory, early universe, galaxies: formation, stars: formation},
     year = 2016,
    month = jun,
   volume = 824,
      eid = {119},
    pages = {119},
      doi = {10.3847/0004-637X/824/2/119},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...824..119H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{holzer_araa_8_1970,
   author = {{Holzer}, T.~E. and {Axford}, W.~I.},
    title = "{The Theory of Stellar Winds and Related Flows}",
  journal = {\araa},
     year = 1970,
   volume = 8,
    pages = {31},
      doi = {10.1146/annurev.aa.08.090170.000335},
   adsurl = {http://adsabs.harvard.edu/abs/1970ARA%26A...8...31H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{houk_1975,
   author = {{Houk}, N. and {Cowley}, A.~P.},
    title = "{University of Michigan Catalogue of two-dimensional spectral types for the HD stars. Volume I. Declinations -90\_ to -53\_{\fnof}0.}",
booktitle = {University of Michigan Catalogue of two-dimensional spectral types for the HD stars.~Volume I.~Declinations -90\_ to -53\_{\fnof}0., by Houk, N.; Cowley, A.~P..~ Ann Arbor, MI (USA): Department of Astronomy, University of Michigan, 19 + 452 p.},
     year = 1975,
   adsurl = {http://cdsads.u-strasbg.fr/abs/1975mcts.book.....H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE I 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{indebetouw_apj_619_2005,
   author = {{Indebetouw}, R. and {Mathis}, J.~S. and {Babler}, B.~L. and 
	{Meade}, M.~R. and {Watson}, C. and {Whitney}, B.~A. and {Wolff}, M.~J. and 
	{Wolfire}, M.~G. and {Cohen}, M. and {Bania}, T.~M. and {Benjamin}, R.~A. and 
	{Clemens}, D.~P. and {Dickey}, J.~M. and {Jackson}, J.~M. and 
	{Kobulnicky}, H.~A. and {Marston}, A.~P. and {Mercer}, E.~P. and 
	{Stauffer}, J.~R. and {Stolovy}, S.~R. and {Churchwell}, E.},
    title = "{The Wavelength Dependence of Interstellar Extinction from 1.25 to 8.0 {$\mu$}m Using GLIMPSE Data}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0406403},
 keywords = {ISM: Dust, Extinction, Infrared: ISM},
     year = 2005,
    month = feb,
   volume = 619,
    pages = {931-938},
      doi = {10.1086/426679},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619..931I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ingalls_apj_579_2002,
   author = {{Ingalls}, J.~G. and {Reach}, W.~T. and {Bania}, T.~M.},
    title = "{Photoelectric Heating and [C II] Cooling of High Galactic Latitude Translucent Clouds}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0207264},
 keywords = {ISM: Dust, Extinction, Infrared: ISM: Continuum, Infrared: ISM: Lines and Bands, ISM: Atoms, ISM: Clouds},
     year = 2002,
    month = nov,
   volume = 579,
    pages = {289-303},
      doi = {10.1086/342704},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...579..289I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ilee_mnras_462_2016,
   author = {{Ilee}, J.~D. and {Cyganowski}, C.~J. and {Nazari}, P. and {Hunter}, T.~R. and 
	{Brogan}, C.~L. and {Forgan}, D.~H. and {Zhang}, Q.},
    title = "{G11.92-0.61 MM1: a Keplerian disc around a massive young proto-O star}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1608.05561},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: G11.92-0.61, stars: massive, stars: pre-main-sequence, stars: protostars, radio continuum: stars, submillimetre: stars},
     year = 2016,
    month = nov,
   volume = 462,
    pages = {4386-4401},
      doi = {10.1093/mnras/stw1912},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.462.4386I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{isella_aa_438_2005,
   author = {{Isella}, A. and {Natta}, A.},
    title = "{The shape of the inner rim in proto-planetary disks}",
  journal = {\aap},
   eprint = {astro-ph/0503635},
 keywords = {accretion, accretion disks, radiative transfer, circumstellar matter, planetary systems: protoplanetary disks, stars: pre-main sequence, infrared: stars},
     year = 2005,
    month = aug,
   volume = 438,
    pages = {899-907},
      doi = {10.1051/0004-6361:20052773},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...438..899I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE J 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{james_aa_453_2006,
   author = {{James}, P.~A. and {Anderson}, J.~P.},
    title = "{The H{$\alpha$} Galaxy Survey . III. Constraints on supernova progenitors from spatial correlations with H{$\alpha$} emission}",
  journal = {\aap},
   eprint = {astro-ph/0602471},
 keywords = {galaxies: general, galaxies: spiral, galaxies: photometry, galaxies: statistics, stars: supernovae: general},
     year = 2006,
    month = jul,
   volume = 453,
    pages = {57-65},
      doi = {10.1051/0004-6361:20054509},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...453...57J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jorissen_532_aa_2011,
   author = {{Jorissen}, A. and {Mayer}, A. and {van Eck}, S. and {Ottensamer}, R. and 
	{Kerschbaum}, F. and {Ueta}, T. and {Bergman}, P. and {Blommaert}, J.~A.~D.~L. and 
	{Decin}, L. and {Groenewegen}, M.~A.~T. and {Hron}, J. and {Nowotny}, W. and 
	{Olofsson}, H. and {Posch}, T. and {Sjouwerman}, L.~O. and {Vandenbussche}, B. and 
	{Waelkens}, C.},
    title = "{X Herculis and TX Piscium: two cases of ISM interaction with stellar winds observed by Herschel}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1106.3645},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: general, stars: AGB and post-AGB, stars: mass-loss, infrared: stars, stars: carbon},
     year = 2011,
    month = aug,
   volume = 532,
      eid = {A135},
    pages = {A135},
      doi = {10.1051/0004-6361/201116927},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532A.135J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{juvela_aa_397_2003,
   author = {{Juvela}, M. and {Padoan}, P.},
    title = "{Dust emission from inhomogeneous interstellar clouds: Radiative transfer in 3D with transiently heated particles}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0207379},
 keywords = {ISM: clouds, infrared: ISM, radiative transfer},
     year = 2003,
    month = jan,
   volume = 397,
    pages = {201-212},
      doi = {10.1051/0004-6361:20021433},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...397..201J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jager_aas_72_1988,
   author = {{de Jager}, C. and {Nieuwenhuijzen}, H. and {van der Hucht}, K.~A.
	},
    title = "{Mass loss rates in the Hertzsprung-Russell diagram}",
  journal = {\aaps},
 keywords = {HERTZSPRUNG-RUSSELL DIAGRAM, O STARS, PLANETARY NEBULAE, STELLAR LUMINOSITY, STELLAR MASS EJECTION, WOLF-RAYET STARS, B STARS, CARBON STARS, COMPUTATIONAL ASTROPHYSICS, HIGH TEMPERATURE, HOT STARS, STELLAR MASS},
     year = 1988,
    month = feb,
   volume = 72,
    pages = {259-289},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26AS...72..259D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{johnston_mnras_415_2011,
   author = {{Johnston}, K.~G. and {Keto}, E. and {Robitaille}, T.~P. and 
	{Wood}, K.},
    title = "{The standard model of low-mass star formation applied to massive stars: multiwavelength modelling of IRAS 20126+4104}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1104.3580},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, radiative transfer, stars: formation, ISM: jets and outflows, infrared: stars},
     year = 2011,
    month = aug,
   volume = 415,
    pages = {2953-2968},
      doi = {10.1111/j.1365-2966.2011.18913.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.415.2953J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{johnston_apj_813_2015,
   author = {{Johnston}, K.~G. and {Robitaille}, T.~P. and {Beuther}, H. and 
	{Linz}, H. and {Boley}, P. and {Kuiper}, R. and {Keto}, E. and 
	{Hoare}, M.~G. and {van Boekel}, R.},
    title = "{A Keplerian-like Disk around the Forming O-type Star AFGL 4176}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1509.08469},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, ISM: jets and outflows, radiative transfer, stars: formation, stars: massive, techniques: interferometric},
     year = 2015,
    month = nov,
   volume = 813,
      eid = {L19},
    pages = {L19},
      doi = {10.1088/2041-8205/813/1/L19},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...813L..19J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{joos_aa_543_2012,
   author = {{Joos}, M. and {Hennebelle}, P. and {Ciardi}, A.},
    title = "{Protostellar disk formation and transport of angular momentum during magnetized core collapse}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1203.1193},
 primaryClass = "astro-ph.SR",
 keywords = {magnetohydrodynamics (MHD), stars: formation, stars: low-mass},
     year = 2012,
    month = jul,
   volume = 543,
      eid = {A128},
    pages = {A128},
      doi = {10.1051/0004-6361/201118730},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...543A.128J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE K 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{klassen_apj_797_2014,
   author = {{Klassen}, M. and {Kuiper}, R. and {Pudritz}, R.~E. and {Peters}, T. and 
	{Banerjee}, R. and {Buntemeyer}, L.},
    title = "{A General Hybrid Radiation Transport Scheme for Star Formation Simulations on an Adaptive Grid}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1410.4259},
 keywords = {hydrodynamics, methods: numerical, radiative transfer},
     year = 2014,
    month = dec,
   volume = 797,
      eid = {4},
    pages = {4},
      doi = {10.1088/0004-637X/797/1/4},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...797....4K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{katsuda_apj_754_2012,
   author = {{Katsuda}, S. and {Tsunemi}, H. and {Mori}, K. and {Uchida}, H. and 
	{Petre}, R. and {Yamada}, S. and {Tamagawa}, T.},
    title = "{Discovery of a Pulsar Wind Nebula Candidate in the Cygnus Loop}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1206.4367},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: individual objects: Cygnus Loop, ISM: supernova remnants, pulsars: general, stars: neutron, stars: winds, outflows, X-rays: ISM},
     year = 2012,
    month = jul,
   volume = 754,
      eid = {L7},
    pages = {L7},
      doi = {10.1088/2041-8205/754/1/L7},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...754L...7K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kane_apj_511_1999,
   author = {{Kane}, J. and {Drake}, R.~P. and {Remington}, B.~A.},
    title = "{An Evaluation of the Richtmyer-Meshkov Instability in Supernova Remnant Formation}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, INSTABILITIES, ISM: SUPERNOVA REMNANTS, STARS: SUPERNOVAE: GENERAL, Hydrodynamics, Instabilities, ISM: Supernova Remnants, Stars: Supernovae: General},
     year = 1999,
    month = jan,
   volume = 511,
    pages = {335-340},
      doi = {10.1086/306685},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...511..335K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kahn_mnras_212_1985,
   author = {{Kahn}, F.~D. and {West}, K.~A.},
    title = "{Shapes of planetary nebulae}",
  journal = {\mnras},
 keywords = {PLANETARY NEBULAE, STELLAR WINDS, ANGULAR MOMENTUM, GAS PRESSURE, STELLAR MASS EJECTION, STELLAR MODELS},
     year = 1985,
    month = feb,
   volume = 212,
    pages = {837-850},
   adsurl = {http://adsabs.harvard.edu/abs/1985MNRAS.212..837K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kaper_apj_475_1997,
   author = {{Kaper}, L. and {van Loon}, J.~T. and {Augusteijn}, T. and {Goudfrooij}, P. and 
	{Patat}, F. and {Waters}, L.~B.~F.~M. and {Zijlstra}, A.~A.},
    title = "{Discovery of a Bow Shock around VELA X-1}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/9611017},
 keywords = {STARS: BINARIES: CLOSE, GALAXY: OPEN CLUSTERS AND ASSOCIATIONS: INDIVIDUAL NAME: VEL OB1, STARS: INDIVIDUAL HENRY DRAPER NUMBER: HD 77581, STARS: MASS LOSS, STARS: PULSARS: INDIVIDUAL NAME: VELA X-1, STARS: SUPERNOVAE: GENERAL},
     year = 1997,
    month = jan,
   volume = 475,
    pages = {L37},
      doi = {10.1086/310454},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...475L..37K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kee_mnras_458_2016,
   author = {{Kee}, N.~D. and {Owocki}, S. and {Sundqvist}, J.~O.},
    title = "{Line-driven ablation of circumstellar discs - I. Optically thin decretion discs of classical Oe/Be stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1602.07874},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, circumstellar matter, stars: early-type, stars: emission-line, Be, stars: mass-loss, stars: winds, outflows},
     year = 2016,
    month = may,
   volume = 458,
    pages = {2323-2335},
      doi = {10.1093/mnras/stw471},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.458.2323K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kaufman_EAS2009,
author = {Kaufman,M.J. and Kaufman,M.J.},
title = {Physical and Chemical Processes in the Diffuse and Dense Neutral ISM},
journal = {EAS Publications Series},
volume = {34},
month = {1},
year = {2009},
issn = {1638-1963},
pages = {151--161},
numpages = {11},
doi = {10.1051/eas:0934011},
URL = {http://www.eas-journal.org/article_S1633476009340119},
}


@ARTICLE{keto_apj_678_2008,
   author = {{Keto}, E. and {Klaassen}, P.},
    title = "{The Ionization of Accretion Flows in High-Mass Star Formation: W51e2}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0804.0514},
 keywords = {H II regions},
     year = 2008,
    month = may,
   volume = 678,
      eid = {L109},
    pages = {L109},
      doi = {10.1086/588657},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...678L.109K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{keto_apj_637_2006,
   author = {{Keto}, E. and {Wood}, K.},
    title = "{Observations on the Formation of Massive Stars by Accretion}",
  journal = {\apj},
   eprint = {astro-ph/0510176},
 keywords = {ISM: individual (G10.6-0.4), Stars: Formation},
     year = 2006,
    month = feb,
   volume = 637,
    pages = {850-859},
      doi = {10.1086/498611},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...637..850K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kessel_aa_337_1998,
   author = {{Kessel}, O. and {Yorke}, H.~W. and {Richling}, S.},
    title = "{Photoevaporation of protostellar disks. III. The appearance of photoevaporating disks around young intermediate mass stars}",
  journal = {\aap},
   eprint = {astro-ph/9806218},
 keywords = {RADIATION TRANSFER, LINE: PROFILES, STARS: CIRCUMSTELLAR MATTER, ISM: H$\backslash$TS II REGIONS, ISM: JETS AND OUTFLOWS},
     year = 1998,
    month = sep,
   volume = 337,
    pages = {832-846},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...337..832K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kesteven_aa_183_1987,
   author = {{Kesteven}, M.~J. and {Caswell}, J.~L.},
    title = "{Barrel-shaped supernova remnants}",
  journal = {\aap},
 keywords = {Astronomical Maps, Supernova Remnants, Morphology, Statistical Analysis, X Ray Astronomy},
     year = 1987,
    month = sep,
   volume = 183,
    pages = {118-128},
   adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...183..118K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kwak_apj_739_2011,
   author = {{Kwak}, K. and {Henley}, D.~B. and {Shelton}, R.~L.},
    title = "{Simulations of High-velocity Clouds. I. Hydrodynamics and High-velocity High Ions}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.6326},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: halo, hydrodynamics, ISM: clouds, methods: numerical, turbulence, ultraviolet: ISM},
     year = 2011,
    month = sep,
   volume = 739,
      eid = {30},
    pages = {30},
      doi = {10.1088/0004-637X/739/1/30},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...739...30K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{klahr_apj_606_2004,
   author = {{Klahr}, H.},
    title = "{The Global Baroclinic Instability in Accretion Disks. II. Local Linear Analysis}",
  journal = {\apj},
   eprint = {astro-ph/0401449},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter, Hydrodynamics, Instabilities, Methods: Numerical, Turbulence},
     year = 2004,
    month = may,
   volume = 606,
    pages = {1070-1082},
      doi = {10.1086/383119},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...606.1070K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{klahr_apj_582_2003,
   author = {{Klahr}, H.~H. and {Bodenheimer}, P.},
    title = "{Turbulence in Accretion Disks: Vorticity Generation and Angular Momentum Transport via the Global Baroclinic Instability}",
  journal = {\apj},
   eprint = {astro-ph/0211629},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter, Hydrodynamics, Instabilities, Methods: Numerical, Turbulence},
     year = 2003,
    month = jan,
   volume = 582,
    pages = {869-892},
      doi = {10.1086/344743},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...582..869K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{klassen_apj_823_2016,
   author = {{Klassen}, M. and {Pudritz}, R.~E. and {Kuiper}, R. and {Peters}, T. and 
	{Banerjee}, R.},
    title = "{Simulating the Formation of Massive Protostars. I. Radiative Feedback and Accretion Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1603.07345},
 keywords = {accretion, accretion disks, hydrodynamics, methods: numerical, radiative transfer, stars: formation},
     year = 2016,
    month = may,
   volume = 823,
      eid = {28},
    pages = {28},
      doi = {10.3847/0004-637X/823/1/28},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...823...28K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kley_apj_397_1992,
   author = {{Kley}, W. and {Lin}, D.~N.~C.},
    title = "{Two-dimensional viscous accretion disk models. I - On meridional circulations in radiative regions}",
  journal = {\apj},
 keywords = {Accretion Disks, Astronomical Models, Computational Astrophysics, Two Dimensional Models, Viscous Fluids, Angular Momentum, Flow Geometry, Hydrodynamic Equations, Mass Flow, Thermodynamic Equilibrium, Velocity Distribution},
     year = 1992,
    month = oct,
   volume = 397,
    pages = {600-612},
      doi = {10.1086/171818},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...397..600K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kley_apj_409_1993,
   author = {{Kley}, W. and {Papaloizou}, J.~C.~B. and {Lin}, D.~N.~C.},
    title = "{Two-dimensional viscous accretion disk models. II - On viscous overstability}",
  journal = {\apj},
 keywords = {Accretion Disks, Astronomical Models, Flow Stability, Two Dimensional Models, Viscosity, Hydrodynamic Equations, Nonlinear Equations},
     year = 1993,
    month = jun,
   volume = 409,
    pages = {739-747},
      doi = {10.1086/172703},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...409..739K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kley_apj_416_1993,
   author = {{Kley}, W. and {Papaloizou}, J.~C.~B. and {Lin}, D.~N.~C.},
    title = "{On the Angular Momentum Transport Associated with Convective Eddies in Accretion Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, CONVECTION, HYDRODYNAMICS, STARS: FORMATION},
     year = 1993,
    month = oct,
   volume = 416,
    pages = {679},
      doi = {10.1086/173268},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...416..679K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kothes_aa_457_2006,
   author = {{Kothes}, R. and {Fedotov}, K. and {Foster}, T.~J. and {Uyan{\i}ker}, B.
	},
    title = "{A catalogue of Galactic supernova remnants from the Canadian Galactic plane survey. I. Flux densities, spectra, and polarization characteristics}",
  journal = {\aap},
 keywords = {atlases, catalogs, polarization, ISM: supernova remnants},
     year = 2006,
    month = oct,
   volume = 457,
    pages = {1081-1093},
      doi = {10.1051/0004-6361:20065062},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...457.1081K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kwok_apj_198_1975,
   author = {{Kwok}, S.},
    title = "{Radiation pressure on grains as a mechanism for mass loss in red giants}",
  journal = {\apj},
 keywords = {GIANT STARS, LATE STARS, M STARS, RADIATION PRESSURE, STELLAR MASS EJECTION, ABSORPTION SPECTRA, COSMIC DUST, MOMENTUM TRANSFER, RADIATIVE TRANSFER, STELLAR ENVELOPES, STELLAR SPECTRA},
     year = 1975,
    month = jun,
   volume = 198,
    pages = {583-591},
      doi = {10.1086/153637},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...198..583K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kudritzki_aa_219_1989,
   author = {{Kudritzki}, R.~P. and {Pauldrach}, A. and {Puls}, J. and {Abbott}, D.~C.
	},
    title = "{Radiation-driven winds of hot stars. VI - Analytical solutions for wind models including the finite cone angle effect}",
  journal = {\aap},
 keywords = {HOT STARS, STELLAR RADIATION, STELLAR WINDS, EQUATIONS OF MOTION, O STARS, PHOTOSPHERE, PLANETARY NEBULAE, STELLAR MASS EJECTION},
     year = 1989,
    month = jul,
   volume = 219,
    pages = {205-218},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...219..205K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_apj_722_2010,
   author = {{Kuiper}, R. and {Klahr}, H. and {Beuther}, H. and {Henning}, T.
	},
    title = "{Circumventing the Radiation Pressure Barrier in the Formation of Massive Stars via Disk Accretion}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1008.4516},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, circumstellar matter, hydrodynamics, methods: numerical, radiative transfer, stars: formation, stars: massive},
     year = 2010,
    month = oct,
   volume = 722,
    pages = {1556-1576},
      doi = {10.1088/0004-637X/722/2/1556},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...722.1556K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_aa_511_2010,
   author = {{Kuiper}, R. and {Klahr}, H. and {Dullemond}, C. and {Kley}, W. and 
	{Henning}, T.},
    title = "{Fast and accurate frequency-dependent radiation transport for hydrodynamics simulations in massive star formation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1001.3301},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, hydrodynamics, stars: formation, circumstellar matter, accretion, accretion disks, methods: numerical},
     year = 2010,
    month = feb,
   volume = 511,
      eid = {A81},
    pages = {A81},
      doi = {10.1051/0004-6361/200912355},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...511A..81K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_apj_772_2013,
   author = {{Kuiper}, R. and {Yorke}, H.~W.},
    title = "{On the Simultaneous Evolution of Massive Protostars and Their Host Cores}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.6310},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, methods: numerical, stars: evolution, stars: formation, stars: pre-main sequence },
     year = 2013,
    month = jul,
   volume = 772,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/772/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772...61K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_apj_732_2011,
   author = {{Kuiper}, R. and {Klahr}, H. and {Beuther}, H. and {Henning}, T.
	},
    title = "{Three-dimensional Simulation of Massive Star Formation in the Disk Accretion Scenario}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1102.4090},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, methods: numerical, stars: formation, stars: massive},
     year = 2011,
    month = may,
   volume = 732,
      eid = {20},
    pages = {20},
      doi = {10.1088/0004-637X/732/1/20},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...732...20K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_apj_800_2015,
   author = {{Kuiper}, R. and {Yorke}, H.~W. and {Turner}, N.~J.},
    title = "{Protostellar Outflows and Radiative Feedback from Massive Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1412.6528},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, methods: numerical, stars: formation, stars: jets, stars: massive, stars: winds, outflows },
     year = 2015,
    month = feb,
   volume = 800,
      eid = {86},
    pages = {86},
      doi = {10.1088/0004-637X/800/2/86},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...800...86K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_apj_763_2013,
   author = {{Kuiper}, R. and {Yorke}, H.~W.},
    title = "{On the Effects of Optically Thick Gas (Disks) around Massive Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1211.6432},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, dust, extinction, ISM: molecules, methods: numerical, stars: formation, stars: winds, outflows },
     year = 2013,
    month = feb,
   volume = 763,
      eid = {104},
    pages = {104},
      doi = {10.1088/0004-637X/763/2/104},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763..104K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_aa_555_2013,
   author = {{Kuiper}, R. and {Klessen}, R.~S.},
    title = "{The reliability of approximate radiation transport methods for irradiated disk studies}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1305.2197},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, accretion, accretion disks, circumstellar, matter, stars: formation, methods:, numerical, hydrodynamics},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A7},
    pages = {A7},
      doi = {10.1051/0004-6361/201321404},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A...7K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuiper_aa_537_2012,
   author = {{Kuiper}, R. and {Klahr}, H. and {Beuther}, H. and {Henning}, T.
	},
    title = "{On the stability of radiation-pressure-dominated cavities}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.5625},
 primaryClass = "astro-ph.SR",
 keywords = {stars: winds, outflows, stars: massive, stars: formation, radiative transfer, hydrodynamics, methods: numerical},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A122},
    pages = {A122},
      doi = {10.1051/0004-6361/201117808},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A.122K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kraus_apj_835_2017,
   author = {{Kraus}, S. and {Kluska}, J. and {Kreplin}, A. and {Bate}, M. and 
	{Harries}, T.~J. and {Hofmann}, K.-H. and {Hone}, E. and {Monnier}, J.~D. and 
	{Weigelt}, G. and {Anugu}, A. and {de Wit}, W.~J. and {Wittkowski}, M.
	},
    title = "{A High-mass Protobinary System with Spatially Resolved Circumstellar Accretion Disks and Circumbinary Disk}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1612.07804},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, binaries: close, stars: formation, stars: individual: IRAS 17216-3801, stars: massive, techniques: interferometric},
     year = 2017,
    month = jan,
   volume = 835,
      eid = {L5},
    pages = {L5},
      doi = {10.3847/2041-8213/835/1/L5},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835L...5K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{krumholz_apj_656_2007,
   author = {{Krumholz}, M.~R. and {Klein}, R.~I. and {McKee}, C.~F.},
    title = "{Radiation-Hydrodynamic Simulations of Collapse and Fragmentation in Massive Protostellar Cores}",
  journal = {\apj},
   eprint = {astro-ph/0609798},
 keywords = {Accretion, Accretion Disks, Equation of State, ISM: Clouds, Methods: Numerical, Radiative Transfer, Stars: Formation},
     year = 2007,
    month = feb,
   volume = 656,
    pages = {959-979},
      doi = {10.1086/510664},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...656..959K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kratter_mnras_373_2006,
   author = {{Kratter}, K.~M. and {Matzner}, C.~D.},
    title = "{Fragmentation of massive protostellar discs}",
  journal = {\mnras},
   eprint = {astro-ph/0609692},
 keywords = {accretion, accretion discs, instabilities, stars: early-type, stars: formation},
     year = 2006,
    month = dec,
   volume = 373,
    pages = {1563-1576},
      doi = {10.1111/j.1365-2966.2006.11103.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.373.1563K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kratter_apj_708_2010,
   author = {{Kratter}, K.~M. and {Matzner}, C.~D. and {Krumholz}, M.~R. and 
	{Klein}, R.~I.},
    title = "{On the Role of Disks in the Formation of Stellar Systems: A Numerical Parameter Study of Rapid Accretion}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0907.3476},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, binaries: general, stars: formation, stars: low-mass, brown dwarfs},
     year = 2010,
    month = jan,
   volume = 708,
    pages = {1585-1597},
      doi = {10.1088/0004-637X/708/2/1585},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...708.1585K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{krumholz_sci_323_2009,
   author = {{Krumholz}, M.~R. and {Klein}, R.~I. and {McKee}, C.~F. and 
	{Offner}, S.~S.~R. and {Cunningham}, A.~J.},
    title = "{The Formation of Massive Star Systems by Accretion}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {0901.3157},
 primaryClass = "astro-ph.SR",
     year = 2009,
    month = feb,
   volume = 323,
    pages = {754},
      doi = {10.1126/science.1165857},
   adsurl = {http://adsabs.harvard.edu/abs/2009Sci...323..754K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{offner_apj_725_2010,
   author = {{Offner}, S.~S.~R. and {Kratter}, K.~M. and {Matzner}, C.~D. and 
	{Krumholz}, M.~R. and {Klein}, R.~I.},
    title = "{The Formation of Low-mass Binary Star Systems Via Turbulent Fragmentation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1010.3702},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, binaries: general, radiative transfer, turbulence},
     year = 2010,
    month = dec,
   volume = 725,
    pages = {1485-1494},
      doi = {10.1088/0004-637X/725/2/1485},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...725.1485O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE L 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{laor_apj_402_1993,
   author = {{Laor}, A. and {Draine}, B.~T.},
    title = "{Spectroscopic constraints on the properties of dust in active galactic nuclei}",
  journal = {\apj},
 keywords = {Active Galactic Nuclei, Astronomical Models, Astronomical Spectroscopy, Computational Astrophysics, Cosmic Dust, Emission Spectra, Grain Size, Graphite, Interstellar Extinction, Optical Properties, Optical Thickness, Silicon Carbides},
     year = 1993,
    month = jan,
   volume = 402,
    pages = {441-468},
      doi = {10.1086/172149},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...402..441L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lagache_aa_333_1998,
   author = {{Lagache}, G. and {Abergel}, A. and {Boulanger}, F. and {Puget}, J.-L.
	},
    title = "{The interstellar cold dust observed by COBE}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/9812474},
 keywords = {ISM: CLOUDS, DUST, EXTINCTION, STRUCTURE, GENERAL, INFRARED: ISM: CONTINUUM, RADIO CONTINUUM: ISM},
     year = 1998,
    month = may,
   volume = 333,
    pages = {709-720},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...333..709L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{langer_ApJ_520_1999,
   author = {{Langer}, N. and {Garc{\'{\i}}a-Segura}, G. and {Mac Low}, M.-M.
	},
    title = "{Giant Outbursts of Luminous Blue Variables and the Formation of the Homunculus Nebula around eta Carinae}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/9905025},
 keywords = {STARS: CIRCUMSTELLAR MATTER, HYDRODYNAMICS, STARS: EVOLUTION, STARS: INDIVIDUAL: CONSTELLATION NAME: ETA CARINAE, STARS: MASS LOSS, STARS: ROTATION},
     year = 1999,
    month = jul,
   volume = 520,
    pages = {L49-L53},
      doi = {10.1086/312131},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...520L..49L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{langer_araa_50_2012,
   author = {{Langer}, N.},
    title = "{Presupernova Evolution of Massive Single and Binary Stars}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1206.5443},
 primaryClass = "astro-ph.SR",
     year = 2012,
    month = sep,
   volume = 50,
    pages = {107-164},
      doi = {10.1146/annurev-astro-081811-125534},
   adsurl = {http://adsabs.harvard.edu/abs/2012ARA%26A..50..107L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@TechReport{langer_dfg_2011,
	title = "DFG Priority Programme 1573 : the physics of the interstellar medium",
	author = "N. Langer",
	institution = "Argelander Institut fur Astronomie",
	month = "February",
	year = "2011"
}

@ARTICLE{lallement_aa_411_2003,
   author = {{Lallement}, R. and {Welsh}, B.~Y. and {Vergely}, J.~L. and 
	{Crifo}, F. and {Sfeir}, D.},
    title = "{3D mapping of the dense interstellar gas around the Local Bubble}",
  journal = {\aap},
 keywords = {Galaxy: solar neighborhood, ISM: atoms, ISM: clouds},
     year = 2003,
    month = dec,
   volume = 411,
    pages = {447-464},
      doi = {10.1051/0004-6361:20031214},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411..447L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{lamer_cassinelli_1999,
   author = {{Lamers}, H.~J.~G.~L.~M. and {Cassinelli}, J.~P.},
    title = "{Introduction to Stellar Winds}",
booktitle = {Introduction to Stellar Winds, by Henny J.~G.~L.~M.~Lamers and Joseph P.~Cassinelli, pp.~452.~ISBN 0521593980.~Cambridge, UK: Cambridge University Press, June 1999.},
     year = 1999,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/1999isw..book.....L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{laughlin_apj_456_1996,
   author = {{Laughlin}, G. and {Rozyczka}, M.},
    title = "{The Effect of Gravitational Instabilities on Protostellar Disks}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, INSTABILITIES, ACCRETION, ACCRETION DISKS, STARS: CIRCUMSTELLAR MATTER},
     year = 1996,
    month = jan,
   volume = 456,
    pages = {279},
      doi = {10.1086/176648},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...456..279L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{laughlin_apj_460_1996,
   author = {{Laughlin}, G. and {Korchagin}, V.},
    title = "{Nonlinear Generation of One-armed Spirals in Self-gravitating Disks}",
  journal = {\apj},
 keywords = {STARS: CIRCUMSTELLAR MATTER, HYDRODYNAMICS, INSTABILITIES, SOLAR SYSTEM: FORMATION},
     year = 1996,
    month = apr,
   volume = 460,
    pages = {855},
      doi = {10.1086/177015},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...460..855L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{lequeux_springerverlag,
   author = {{Lequeux}, J.},
    title = "{The Interstellar Medium}",
booktitle = {The interstellar medium, Translation from the French language edition 
of: Le Milieu Interstellaire by James Lequeux, EDP Sciences, 2003 Edited by J.~Lequeux.~ Astronomy and astrophysics library, Berlin: Springer, 2005},
     year = 2005,
      doi = {10.1007/b137959},
   adsurl = {http://adsabs.harvard.edu/abs/2005ism..book.....L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Book{lequeux_edp,
	title = "Le milieu interstellaire",
	author = "J. Lequeux",
	publisher = "CNRS Editions",
	edition = "EDP sciences",
	month = "March",
	year = "2002",
	isbn = "2 86889 533 3"
}

@ARTICLE{leeuwen_aa_474_2007,
   author = {{van Leeuwen}, F.},
    title = "{Validation of the new Hipparcos reduction}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0708.1752},
 keywords = {space vehicles: instruments, methods: data analysis, catalogs, astrometry, instrumentation: miscellaneous},
     year = 2007,
    month = nov,
   volume = 474,
    pages = {653-664},
      doi = {10.1051/0004-6361:20078357},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...474..653V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lichtenberg_aa_579_2015,
   author = {{Lichtenberg}, T. and {Schleicher}, D.~R.~G.},
    title = "{Modeling gravitational instabilities in self-gravitating protoplanetary disks with adaptive mesh refinement techniques}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1505.01154},
 primaryClass = "astro-ph.EP",
 keywords = {protoplanetary disks, hydrodynamics, instabilities, planets and satellites: formation, methods: numerical},
     year = 2015,
    month = jul,
   volume = 579,
      eid = {A32},
    pages = {A32},
      doi = {10.1051/0004-6361/201424528},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...579A..32L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lin_apj_416_1993,
   author = {{Lin}, D.~N.~C. and {Papaloizou}, J.~C.~B. and {Kley}, W.},
    title = "{On the Nonaxisymmetric Convective Instabilities in Accretion Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, CONVECTION, HYDRODYNAMICS, STARS: FORMATION},
     year = 1993,
    month = oct,
   volume = 416,
    pages = {689},
      doi = {10.1086/173269},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...416..689L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{liszt_499_aa_2009,
   author = {{Liszt}, H.~S. and {Pety}, J. and {Tachihara}, K.},
    title = "{Imaging galactic diffuse clouds: CO emission, reddening and turbulent flow in the gas around {$\zeta$} Ophiuchi}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0901.1111},
 keywords = {astrochemistry, ISM: molecules, ISM: clouds},
     year = 2009,
    month = may,
   volume = 499,
    pages = {503-513},
      doi = {10.1051/0004-6361:200810905},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...499..503L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lockett_apj_511_1999,
   author = {{Lockett}, P. and {Gauthier}, E. and {Elitzur}, M.},
    title = "{OH 1720 Megahertz Masers in Supernova Remnants: C-Shock Indicators}",
  journal = {\apj},
   eprint = {astro-ph/9809019},
 keywords = {ISM: CLOUDS, MASERS, SHOCK WAVES, ISM: SUPERNOVA REMNANTS, ISM: Clouds, Masers, Shock Waves, ISM: Supernova Remnants},
     year = 1999,
    month = jan,
   volume = 511,
    pages = {235-241},
      doi = {10.1086/306667},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...511..235L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lodato_mc_30_2007,
   author = {{Lodato}, G.},
    title = "{Self-gravitating accretion discs}",
  journal = {Nuovo Cimento Rivista Serie},
archivePrefix = "arXiv",
   eprint = {0801.3848},
     year = 2007,
   volume = 30,
      doi = {10.1393/ncr/i2007-10022-x},
   adsurl = {http://adsabs.harvard.edu/abs/2007NCimR..30..293L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lodato_mnras_413_2011,
   author = {{Lodato}, G. and {Clarke}, C.~J.},
    title = "{Resolution requirements for smoothed particle hydrodynamics simulations of self-gravitating accretion discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1101.2448},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, gravitation, instabilities, stars: formation, galaxies: active},
     year = 2011,
    month = jun,
   volume = 413,
    pages = {2735-2740},
      doi = {10.1111/j.1365-2966.2011.18344.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413.2735L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lodders_apj_591_2003,
   author = {{Lodders}, K.},
    title = "{Solar System Abundances and Condensation Temperatures of the Elements}",
  journal = {\apj},
 keywords = {Astrochemistry, Meteors, Meteoroids, Solar System: Formation- Sun: Abundances, Sun: Photosphere},
     year = 2003,
    month = jul,
   volume = 591,
    pages = {1220-1247},
      doi = {10.1086/375492},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...591.1220L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lopez_apj_757_2012,
   author = {{L{\'o}pez-Santiago}, J. and {Miceli}, M. and {del Valle}, M.~V. and 
	{Romero}, G.~E. and {Bonito}, R. and {Albacete-Colombo}, J.~F. and 
	{Pereira}, V. and {de Castro}, E. and {Damiani}, F.},
    title = "{AE Aurigae: First Detection of Non-thermal X-Ray Emission from a Bow Shock Produced by a Runaway Star}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1208.6511},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: clouds, radiation mechanisms: non-thermal, stars: individual: AE Aur, stars: kinematics and dynamics, stars: massive, X-rays: general },
     year = 2012,
    month = sep,
   volume = 757,
      eid = {L6},
    pages = {L6},
      doi = {10.1088/2041-8205/757/1/L6},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757L...6L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{lyne_natur_369_1994,
   author = {{Lyne}, A.~G. and {Lorimer}, D.~R.},
    title = "{High birth velocities of radio pulsars}",
  journal = {\nat},
     year = 1994,
    month = may,
   volume = 369,
    pages = {127-129},
      doi = {10.1038/369127a0},
   adsurl = {http://adsabs.harvard.edu/abs/1994Natur.369..127L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE M 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{macdomald_mnras_197_1981,
   author = {{MacDonald}, J. and {Bailey}, M.~E.},
    title = "{The evolution of flows of stellar mass loss in active galaxies}",
  journal = {\mnras},
 keywords = {Active Galaxies, Astronomical Models, Elliptical Galaxies, Flow Characteristics, Galactic Evolution, Gas Flow, Stellar Winds, Equations Of State, Galactic Radiation, Galactic Structure, Numerical Analysis, Stellar Evolution, Supernovae},
     year = 1981,
    month = dec,
   volume = 197,
    pages = {995-1019},
   adsurl = {http://adsabs.harvard.edu/abs/1981MNRAS.197..995M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{machida_mnras_435_2013,
   author = {{Machida}, M.~N. and {Doi}, K.},
    title = "{The formation of Population III stars in gas accretion stage: effects of magnetic fields}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1308.2754},
 keywords = {accretion, accretion discs, binaries: general, stars: formation, ISM: magnetic fields, cosmology: theory, early universe},
     year = 2013,
    month = nov,
   volume = 435,
    pages = {3283-3305},
      doi = {10.1093/mnras/stt1524},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435.3283M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{matsumoto_apj_839_2017,
   author = {{Matsumoto}, T. and {Machida}, M.~N. and {Inutsuka}, S.-i.},
    title = "{Circumstellar Disks and Outflows in Turbulent Molecular Cloud Cores: Possible Formation Mechanism for Misaligned Systems}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1703.09139},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, ISM: kinematics and dynamics, magnetohydrodynamics: MHD, stars: formation, turbulence },
     year = 2017,
    month = apr,
   volume = 839,
      eid = {69},
    pages = {69},
      doi = {10.3847/1538-4357/aa6a1c},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...839...69M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{machida_mnras_438_2014,
   author = {{Machida}, M.~N. and {Inutsuka}, S.-i. and {Matsumoto}, T.},
    title = "{Conditions for circumstellar disc formation: effects of initial cloud configuration and sink treatment}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1307.1747},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, MHD, stars: formation, stars: low-mass, ISM: jets and outflows, ISM: magnetic fields},
     year = 2014,
    month = mar,
   volume = 438,
    pages = {2278-2306},
      doi = {10.1093/mnras/stt2343},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.2278M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{machida_mnras_431_2013,
   author = {{Machida}, M.~N. and {Hosokawa}, T.},
    title = "{Evolution of protostellar outflow around low-mass protostar}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1302.4176},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, MHD, stars: formation, stars: low-mass, ISM: jets and outflows, ISM: magnetic fields},
     year = 2013,
    month = may,
   volume = 431,
    pages = {1719-1744},
      doi = {10.1093/mnras/stt291},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.431.1719M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maclow_apr_407_1993,
   author = {{Mac Low}, M.-M. and {Norman}, M.~L.},
    title = "{Nonlinear growth of dynamical overstabilities in blast waves}",
  journal = {\apj},
 keywords = {DYNAMIC STABILITY, INTERSTELLAR MATTER, SHOCK WAVES, SUPERNOVA REMNANTS, ASTRONOMICAL MODELS, HYDRODYNAMICS},
     year = 1993,
    month = apr,
   volume = 407,
    pages = {207-218},
      doi = {10.1086/172506},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...407..207M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maclow_apj_369_1991,
   author = {{Mac Low}, M.-M. and {van Buren}, D. and {Wood}, D.~O.~S. and 
	{Churchwell}, E.},
    title = "{Bow shock models of ultracompact H II regions}",
  journal = {\apj},
 keywords = {ASTRONOMICAL MODELS, H II REGIONS, MOLECULAR CLOUDS, SHOCK WAVE PROPAGATION, STELLAR WINDS, ASTRONOMICAL MAPS, DIGITAL SIMULATION, INFRARED ASTRONOMY SATELLITE, INTERSTELLAR MATTER, MILKY WAY GALAXY, RADIATIVE TRANSFER},
     year = 1991,
    month = mar,
   volume = 369,
    pages = {395-409},
      doi = {10.1086/169769},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...369..395M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mackey_mnras_412_2010,
   author = {{Mackey}, J. and {Lim}, A.~J.},
    title = "{Effects of magnetic fields on photoionized pillars and globules}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1012.1500},
 primaryClass = "astro-ph.GA",
 keywords = {MHD, radiative transfer, methods: numerical, H II regions, ISM: magnetic fields},
     year = 2011,
    month = apr,
   volume = 412,
    pages = {2079-2094},
      doi = {10.1111/j.1365-2966.2010.18043.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.412.2079M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mackey_bsrsl_2011,
   author = {{Mackey}, J. and {Lim}, A.~J.},
    title = "{Radiation-MHD models of elephant trunks and globules in HII regions}",
  journal = {Bulletin de la Societe Royale des Sciences de Liege},
archivePrefix = "arXiv",
   eprint = {1104.1073},
 primaryClass = "astro-ph.GA",
     year = 2011,
    month = jan,
   volume = 80,
    pages = {391-395},
   adsurl = {http://adsabs.harvard.edu/abs/2011BSRSL..80..391M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mackey_mnras_403_2010,
   author = {{Mackey}, J. and {Lim}, A.~J.},
    title = "{Dynamical models for the formation of elephant trunks in HII regions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0912.1499},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, radiative transfer, methods: numerical, HII regions},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {714-730},
      doi = {10.1111/j.1365-2966.2009.16181.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403..714M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mackey_apjlett_751_2012,
   author = {{Mackey}, J. and {Mohamed}, S. and {Neilson}, H.~R. and {Langer}, N. and 
	{Meyer}, D.~M.-A.},
    title = "{Double Bow Shocks around Young, Runaway Red Supergiants: Application to Betelgeuse}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1204.3925},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, hydrodynamics, stars: evolution, stars: individual: Betelgeuse, stars: winds, outflows },
     year = 2012,
    month = may,
   volume = 751,
      eid = {L10},
    pages = {L10},
      doi = {10.1088/2041-8205/751/1/L10},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751L..10M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mackey_sept_2014,
   author = {{Mackey}, J. and {Gvaramadze}, V.~V. and {Mohamed}, S. and {Langer}, N.
	},
    title = "{Wind bubbles within H II regions around slowly moving stars}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1410.0019},
 keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
     year = 2014,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1410.0019M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{mackey_2013,
   author = {{Mackey}, J.},
    title = "{Moving HII regions around massive stars: Application to Betelgeuse}",
     year = 2013
}

@ARTICLE{mackey_mnras_2013,
   author = {{Mackey}, J. and {Langer}, N. and {Gvaramadze}, V.~V.},
    title = "{Dynamics of H II regions around exiled O stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1308.5192},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, radiative transfer, methods: numerical, stars: early-type, stars: individual: {$\zeta$} Oph, H II regions},
     year = 2013,
    month = sep,
      doi = {10.1093/mnras/stt1621},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.tmp.2269M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maeder_rvmp_84_2012,
   author = {{Maeder}, A. and {Meynet}, G.},
    title = "{Rotating massive stars: From first stars to gamma ray bursts}",
  journal = {Reviews of Modern Physics},
 keywords = {Stellar rotation, Mass loss and stellar winds, Abundances, chemical composition, Main-sequence: early-type stars},
     year = 2012,
    month = jan,
   volume = 84,
    pages = {25-63},
      doi = {10.1103/RevModPhys.84.25},
   adsurl = {http://adsabs.harvard.edu/abs/2012RvMP...84...25M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Book{ maeder_2009,
	title = "Physics, Formation and Evolution of Rotating Stars",
	author = "A. Maeder",
	publisher = "Astronomy and Astrophysics Library",
	edition = "SPringer-Verlag",
	year = "2009"
}

@ARTICLE{manchester_aa_171_1987,
   author = {{Manchester}, R.~N.},
    title = "{The radio structure of supernova remnants}",
  journal = {\aap},
 keywords = {Radio Spectra, Spectral Energy Distribution, Stellar Models, Stellar Structure, Supernova Remnants, Astronomical Maps, Binary Stars, Pulsars, Stellar Evolution},
     year = 1987,
    month = jan,
   volume = 171,
    pages = {205-215},
   adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...171..205M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tomida_apj_801_2015,
   author = {{Tomida}, K. and {Okuzumi}, S. and {Machida}, M.~N.},
    title = "{Radiation Magnetohydrodynamic Simulations of Protostellar Collapse: Nonideal Magnetohydrodynamic Effects and Early Formation of Circumstellar Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1501.04102},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, ISM: jets and outflows, magnetohydrodynamics: MHD, radiative transfer, stars: formation},
     year = 2015,
    month = mar,
   volume = 801,
      eid = {117},
    pages = {117},
      doi = {10.1088/0004-637X/801/2/117},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...801..117T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{masson_apjs_201_2012,
   author = {{Masson}, J. and {Teyssier}, R. and {Mulet-Marquis}, C. and 
	{Hennebelle}, P. and {Chabrier}, G.},
    title = "{Incorporating Ambipolar and Ohmic Diffusion in the AMR MHD Code RAMSES}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1206.2476},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: magnetic fields, methods: numerical, stars: formation},
     year = 2012,
    month = aug,
   volume = 201,
      eid = {24},
    pages = {24},
      doi = {10.1088/0067-0049/201/2/24},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..201...24M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{masson_aa_587_2016,
   author = {{Masson}, J. and {Chabrier}, G. and {Hennebelle}, P. and {Vaytet}, N. and 
	{Commer{\c c}on}, B.},
    title = "{Ambipolar diffusion in low-mass star formation. I. General comparison with the ideal magnetohydrodynamic case}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1509.05630},
 primaryClass = "astro-ph.SR",
 keywords = {astrochemistry, diffusion, magnetohydrodynamics, protoplanetary disks, stars: formation, stars: magnetic field},
     year = 2016,
    month = mar,
   volume = 587,
      eid = {A32},
    pages = {A32},
      doi = {10.1051/0004-6361/201526371},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...587A..32M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martins_aa_538_2012,
   author = {{Martins}, F. and {Escolano}, C. and {Wade}, G.~A. and {Donati}, J.~F. and 
	{Bouret}, J.~C. and {Mimes Collaboration}},
    title = "{Observational effects of magnetism in O stars: surface nitrogen abundances}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1112.2497},
 primaryClass = "astro-ph.SR",
 keywords = {stars: massive, stars: atmospheres, stars: fundamental parameters, stars: abundances, stars: magnetic field},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A29},
    pages = {A29},
      doi = {10.1051/0004-6361/201118039},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A..29M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martin_aa_538b_2012,
   author = {{Martins}, F. and {Mahy}, L. and {Hillier}, D.~J. and {Rauw}, G.
	},
    title = "{A quantitative study of O stars in NGC 2244 and the Monoceros OB2 association}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.4509},
 primaryClass = "astro-ph.SR",
 keywords = {stars: fundamental parameters, stars: winds, outflows, stars: early-type, Hii regions},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A39},
    pages = {A39},
      doi = {10.1051/0004-6361/201117458},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...538A..39M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mckee_apj_195_1975,
   author = {{McKee}, C.~F. and {Ostriker}, J.~P.},
    title = "{A theory of the interstellar medium - Three components regulated by supernova explosions in an inhomogeneous substrate}",
  journal = {\apj},
 keywords = {INTERSTELLAR MATTER, NEBULAE, SUPERNOVA REMNANTS, X RAY SOURCES, ABSORPTION SPECTRA, ADIABATIC CONDITIONS, ASTRONOMICAL MODELS, BACKGROUND RADIATION, CLOUDS, EVAPORATION, HIGH TEMPERATURE GASES, RAREFIED GASES},
     year = 1977,
    month = nov,
   volume = 218,
    pages = {148-169},
      doi = {10.1086/155667},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...218..148M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975ApJ...195..715M,
   author = {{McKee}, C.~F. and {Cowie}, L.~L.},
    title = "{The interaction between the blast wave of a supernova remnant and interstellar clouds}",
  journal = {\apj},
 keywords = {INTERSTELLAR GAS, SHOCK HEATING, SHOCK WAVE INTERACTION, SUPERNOVA REMNANTS, ABUNDANCE, ASTRONOMICAL MODELS, CLOUD PHYSICS, LIGHT EMISSION, STELLAR EVOLUTION, X RAY ASTRONOMY},
     year = 1975,
    month = feb,
   volume = 195,
    pages = {715-725},
      doi = {10.1086/153373},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...195..715M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{marchand_aa_592_2016,
   author = {{Marchand}, P. and {Masson}, J. and {Chabrier}, G. and {Hennebelle}, P. and 
	{Commer{\c c}on}, B. and {Vaytet}, N.},
    title = "{Chemical solver to compute molecule and grain abundances and non-ideal MHD resistivities in prestellar core-collapse calculations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1604.05613},
 keywords = {magnetohydrodynamics (MHD), ISM: molecules, stars: formation},
     year = 2016,
    month = jul,
   volume = 592,
      eid = {A18},
    pages = {A18},
      doi = {10.1051/0004-6361/201526780},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...592A..18M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martins_aa_436_2005,
   author = {{Martins}, F. and {Schaerer}, D. and {Hillier}, D.~J.},
    title = "{A new calibration of stellar parameters of Galactic O stars}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0503346},
 keywords = {stars: fundamental parameters, stars: atmospheres, stars: early-type},
     year = 2005,
    month = jun,
   volume = 436,
    pages = {1049-1065},
      doi = {10.1051/0004-6361:20042386},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...436.1049M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mathis_apj_217_1977,
   author = {{Mathis}, J.~S. and {Rumpl}, W. and {Nordsieck}, K.~H.},
    title = "{The size distribution of interstellar grains}",
  journal = {\apj},
 keywords = {COSMIC DUST, INTERSTELLAR EXTINCTION, INTERSTELLAR MATTER, PARTICLE SIZE DISTRIBUTION, ENSTATITE, GRAPHITE, MAGNETITE, OLIVINE, POLARIZATION CHARACTERISTICS, ULTRAVIOLET ASTRONOMY},
     year = 1977,
    month = oct,
   volume = 217,
    pages = {425-433},
      doi = {10.1086/155591},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...217..425M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PROCEEDINGS{massaglia_lnp_754_2008,
   editor = {{Massaglia}, S. and {Bodo}, G. and {Mignone}, A. and {Rossi}, P.
	},
    title = "{Jets From Young Stars III}",
 keywords = {Physics, Astrophysics, Numerical and Computational Methods},
booktitle = {Jets From Young Stars III},
     year = 2008,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 754,
      doi = {10.1007/978-3-540-76967-5},
   adsurl = {http://adsabs.harvard.edu/abs/2008LNP...754.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mignone_apj_170_2007,
   author = {{Mignone}, A. and {Bodo}, G. and {Massaglia}, S. and {Matsakos}, T. and 
	{Tesileanu}, O. and {Zanni}, C. and {Ferrari}, A.},
    title = "{PLUTO: A Numerical Code for Computational Astrophysics}",
  journal = {\apjs},
   eprint = {arXiv:astro-ph/0701854},
 keywords = {Hydrodynamics, Methods: Numerical, Magnetohydrodynamics: MHD, Relativity, Shock Waves},
     year = 2007,
    month = may,
   volume = 170,
    pages = {228-242},
      doi = {10.1086/513316},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..170..228M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mazzotta_aaps_133_1998,
   author = {{Mazzotta}, P. and {Mazzitelli}, G. and {Colafrancesco}, S. and 
	{Vittorio}, N.},
    title = "{Ionization balance for optically thin plasmas: Rate coefficients for all atoms and ions of the elements H to NI}",
  journal = {\aaps},
   eprint = {arXiv:astro-ph/9806391},
 keywords = {ATOMIC DATA, PLASMAS, RADIATION MECHANISMS: THERMAL, X-RAYS: GENERAL},
     year = 1998,
    month = dec,
   volume = 133,
    pages = {403-409},
      doi = {10.1051/aas:1998330},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26AS..133..403M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{McMullin_aspc_376_2007,
   author = {{McMullin}, J.~P. and {Waters}, B. and {Schiebel}, D. and {Young}, W. and 
	{Golap}, K.},
    title = "{CASA Architecture and Applications}",
booktitle = {Astronomical Data Analysis Software and Systems XVI},
     year = 2007,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 376,
   editor = {{Shaw}, R.~A. and {Hill}, F. and {Bell}, D.~J.},
    month = oct,
    pages = {127},
   adsurl = {http://adsabs.harvard.edu/abs/2007ASPC..376..127M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PROCEEDINGS{2008LNP...754.....M,
   editor = {{Massaglia}, S. and {Bodo}, G. and {Mignone}, A. and {Rossi}, P.
	},
    title = "{Jets From Young Stars III}",
 keywords = {Physics, Astrophysics, Numerical and Computational Methods},
booktitle = {Jets From Young Stars III},
     year = 2008,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 754,
      doi = {10.1007/978-3-540-76967-5},
   adsurl = {http://adsabs.harvard.edu/abs/2008LNP...754.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{medina_791_apj_2014,
   author = {{Medina}, A.~A. and {Raymond}, J.~C. and {Edgar}, R.~J. and 
	{Caldwell}, N. and {Fesen}, R.~A. and {Milisavljevic}, D.},
    title = "{Electron-Ion Equilibrium and Shock Precursors in the Northeast Limb of the Cygnus Loop}",
  journal = {\apj},
 keywords = {acceleration of particles, ISM: individual objects: Cygnus Loop, ISM: supernova remnants, shock waves},
     year = 2014,
    month = aug,
   volume = 791,
      eid = {30},
    pages = {30},
      doi = {10.1088/0004-637X/791/1/30},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...791...30M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mercer_2016arXiv161008248M,
   author = {{Mercer}, A. and {Stamatellos}, D.},
    title = "{The effect of radiative feedback on disc fragmentation}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.08248},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2016,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161008248M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meru_mnras_406_2010,
   author = {{Meru}, F. and {Bate}, M.~R.},
    title = "{Exploring the conditions required to form giant planets via gravitational instability in massive protoplanetary discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1004.3766},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, gravitation, hydrodynamics, instabilities, planetary systems, protoplanetary discs},
     year = 2010,
    month = aug,
   volume = 406,
    pages = {2279-2288},
      doi = {10.1111/j.1365-2966.2010.16867.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.406.2279M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meru_mnras_411_2011,
   author = {{Meru}, F. and {Bate}, M.~R.},
    title = "{Non-convergence of the critical cooling time-scale for fragmentation of self-gravitating discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1011.5896},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, gravitation, hydrodynamics, instabilities, planets and satellites: formation, protoplanetary discs},
     year = 2011,
    month = feb,
   volume = 411,
    pages = {L1-L5},
      doi = {10.1111/j.1745-3933.2010.00978.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.411L...1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meru_mnras_454_2015,
   author = {{Meru}, F.},
    title = "{Triggered fragmentation in self-gravitating discs: forming fragments at small radii}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1509.03635},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, gravitation, hydrodynamics, instabilities, planets and satellites: formation, protoplanetary discs},
     year = 2015,
    month = dec,
   volume = 454,
    pages = {2529-2538},
      doi = {10.1093/mnras/stv2128},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015MNRAS.454.2529M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{masset_aa_141_2000,
   author = {{Masset}, F.},
    title = "{FARGO: A fast eulerian transport algorithm for differentially rotating disks}",
  journal = {\aaps},
   eprint = {astro-ph/9910390},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, METHODS: NUMERICAL},
     year = 2000,
    month = jan,
   volume = 141,
    pages = {165-173},
      doi = {10.1051/aas:2000116},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26AS..141..165M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meyer_mnras_2013,
   author = {{Meyer}, D.~M.-A. and {Gvaramadze}, V.~V. and {Langer}, N. and 
	{Mackey}, J. and {Boumis}, P. and {Mohamed}, S.},
    title = "{On the stability of bow shocks generated by red supergiants: the case of IRC -10414}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1312.1687},
 primaryClass = "astro-ph.SR",
 keywords = {shock waves, methods: numerical, circumstellar matter, stars: individual: IRC -10414, stars: massive},
     year = 2014,
    month = mar,
   volume = 439,
    pages = {L41-L45},
      doi = {10.1093/mnrasl/slt176},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439L..41M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meyer_mnras_450_2015,
   author = {{Meyer}, D.~M.-A. and {Langer}, N. and {Mackey}, J. and {Vel{\'a}zquez}, P.~F. and 
	{Gusdorf}, A.},
    title = "{Asymmetric supernova remnants generated by Galactic, massive runaway stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1508.03347},
 primaryClass = "astro-ph.HE",
 keywords = {shock waves, methods: numerical, stars: massive, ISM: supernova remnants},
     year = 2015,
    month = jul,
   volume = 450,
    pages = {3080-3100},
      doi = {10.1093/mnras/stv898},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.450.3080M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meyer,
   author = {{Meyer}, D.~M.-A. and {Mackey}, J. and {Langer}, N. and {Gvaramadze}, V.~V. and 
	{Mignone}, A. and {Izzard}, R.~G. and {Kaper}, L.},
    title = "{Models of the circumstellar medium of evolving, massive runaway stars moving through the Galactic plane}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1408.2828},
 primaryClass = "astro-ph.SR",
 keywords = {shock waves, methods: numerical, circumstellar matter, stars: massive},
     year = 2014,
    month = nov,
   volume = 444,
    pages = {2754-2775},
      doi = {10.1093/mnras/stu1629},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.444.2754M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meyer_mnras_464_2017,
   author = {{Meyer}, D.~M.-A. and {Vorobyov}, E.~I. and {Kuiper}, R. and 
	{Kley}, W.},
    title = "{On the existence of accretion-driven bursts in massive star formation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1609.03402},
 primaryClass = "astro-ph.SR",
     year = 2017,
    month = jan,
   volume = 464,
    pages = {L90-L94},
      doi = {10.1093/mnrasl/slw187},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.464L..90M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{mignone_lnp_754b_2008,
   author = {{Mignone}, A. and {Bodo}, G.},
    title = "{Shock-Capturing Schemes in Computational MHD}",
booktitle = {Jets From Young Stars III},
     year = 2008,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 754,
   editor = "{S.~Massaglia, G.~Bodo, A.~Mignone, \& P.~Rossi}",
    pages = {71-101},
      doi = {10.1007/978-3-540-76967-5_2},
   adsurl = {http://adsabs.harvard.edu/abs/2008LNP...754...71M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{mignone_lnp_754a_2008,
   author = {{Toro}, E.~F.},
    title = "{Computational Methods for Hyperbolic Equations}",
booktitle = {Jets From Young Stars III},
     year = 2008,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 754,
   editor = "{S.~Massaglia, G.~Bodo, A.~Mignone, \& P.~Rossi}",
    pages = {3-69},
      doi = {10.1007/978-3-540-76967-5_1},
   adsurl = {http://adsabs.harvard.edu/abs/2008LNP...754....3T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@Manual{mignone_user_guide_pluto_2011,
	title = "Pluto User's Guide",
	author = "A. Mignone and P. Tzeferacos and G. Bodo and T. Matsakos and O. Tesileanu and C. Zanni",
	month = "April",
	year = "2011"
}

@ARTICLE{mitchell_mnras_362_2005,
   author = {{Mitchell}, D.~L. and {Bryce}, M. and {Meaburn}, J. and {L{\'o}pez}, J.~A. and 
	{Redman}, M.~P. and {Harman}, D. and {Richer}, M.~G. and {Riesgo}, H.
	},
    title = "{The kinematics of the large western knot in the halo of the young planetary nebula NGC 6543}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0507204},
 keywords = {circumstellar matter, stars: kinematics, stars: mass-loss, stars: winds, outflows, ISM: planetary nebulae: individual: NGC 6543},
     year = 2005,
    month = oct,
   volume = 362,
    pages = {1286-1294},
      doi = {10.1111/j.1365-2966.2005.09399.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362.1286M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mohamed_aa_541_2012,
   author = {{Mohamed}, S. and {Mackey}, J. and {Langer}, N.},
    title = "{3D simulations of Betelgeuse's bow shock}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.1555},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, instabilities, circumstellar matter, stars: winds, outflows, supergiants, ISM: structure},
     year = 2012,
    month = may,
   volume = 541,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201118002},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...541A...1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mokiem_aa_465_2007,
   author = {{Mokiem}, M.~R. and {de Koter}, A. and {Evans}, C.~J. and {Puls}, J. and 
	{Smartt}, S.~J. and {Crowther}, P.~A. and {Herrero}, A. and 
	{Langer}, N. and {Lennon}, D.~J. and {Najarro}, F. and {Villamariz}, M.~R. and 
	{Vink}, J.~S.},
    title = "{The VLT-FLAMES survey of massive stars: wind properties and evolution of hot massive stars in the Large Magellanic Cloud}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.1113},
 keywords = {galaxies: Magellanic Clouds, stars: atmospheres, stars:, early-type, stars: fundamental parameters, stars: mass loss, stars: evolution},
     year = 2007,
    month = apr,
   volume = 465,
    pages = {1003-1019},
      doi = {10.1051/0004-6361:20066489},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...465.1003M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Manual{mignone_developer_guide_pluto_2011,
	title = "Pluto Developer's Guide",
	author = "A. Mignone",
	month = "April",
	year = "2011"
}


@ARTICLE{migmone_apjs_198_2012,
   author = {{Mignone}, A. and {Zanni}, C. and {Tzeferacos}, P. and {van Straalen}, B. and 
	{Colella}, P. and {Bodo}, G.},
    title = "{The PLUTO Code for Adaptive Mesh Computations in Astrophysical Fluid Dynamics}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1110.0740},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, magnetohydrodynamics: MHD, methods: numerical },
     year = 2012,
    month = jan,
   volume = 198,
      eid = {7},
    pages = {7},
      doi = {10.1088/0067-0049/198/1/7},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..198....7M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{myers_apj_766_2013,
   author = {{Myers}, A.~T. and {McKee}, C.~F. and {Cunningham}, A.~J. and 
	{Klein}, R.~I. and {Krumholz}, M.~R.},
    title = "{The Fragmentation of Magnetized, Massive Star-forming Cores with Radiative Feedback}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1211.3467},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, magnetohydrodynamics: MHD, radiative transfer, stars: formation, stars: luminosity function, mass function, turbulence},
     year = 2013,
    month = apr,
   volume = 766,
      eid = {97},
    pages = {97},
      doi = {10.1088/0004-637X/766/2/97},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...766...97M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{myers_mnras_439_2014,
   author = {{Myers}, A.~T. and {Klein}, R.~I. and {Krumholz}, M.~R. and 
	{McKee}, C.~F.},
    title = "{Star cluster formation in turbulent, magnetized dense clumps with radiative and outflow feedback}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1401.6096},
 keywords = {magnetic fields, radiative transfer, turbulence, stars: formation, stars: luminosity function, mass function, stars: protostars},
     year = 2014,
    month = apr,
   volume = 439,
    pages = {3420-3438},
      doi = {10.1093/mnras/stu190},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.3420M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE N 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{neufeld_apj_781_2014,
   author = {{Neufeld}, D.~A. and {Gusdorf}, A. and {G{\"u}sten}, R. and 
	{Herczeg}, G.~J. and {Kristensen}, L. and {Melnick}, G.~J. and 
	{Nisini}, B. and {Ossenkopf}, V. and {Tafalla}, M. and {van Dishoeck}, E.~F.
	},
    title = "{The Water Abundance behind Interstellar Shocks: Results from Herschel/PACS and Spitzer/IRS Observations of H$_{2}$O, CO, and H$_{2}$}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1312.6703},
 primaryClass = "astro-ph.GA",
 keywords = {infrared: ISM, ISM: abundances, ISM: molecules, molecular processes, shock waves},
     year = 2014,
    month = feb,
   volume = 781,
      eid = {102},
    pages = {102},
      doi = {10.1088/0004-637X/781/2/102},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...781..102N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{neilson_apj_716_2010,
   author = {{Neilson}, H.~R. and {Ngeow}, C.-C. and {Kanbur}, S.~M. and 
	{Lester}, J.~B.},
    title = "{Testing Mass Loss in Large Magellanic Cloud Cepheids using Infrared and Optical Observations. II. Predictions and Tests of the OGLE-III Fundamental-mode Cepheids}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1005.0622},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, Magellanic Clouds, stars: mass-loss, stars: variables: Cepheids},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {1136-1150},
      doi = {10.1088/0004-637X/716/2/1136},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716.1136N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...537A..35C,
   author = {{Cox}, N.~L.~J. and {Kerschbaum}, F. and {van Marle}, A.-J. and 
	{Decin}, L. and {Ladjal}, D. and {Mayer}, A. and {Groenewegen}, M.~A.~T. and 
	{van Eck}, S. and {Royer}, P. and {Ottensamer}, R. and {Ueta}, T. and 
	{Jorissen}, A. and {Mecina}, M. and {Meliani}, Z. and {Luntzer}, A. and 
	{Blommaert}, J.~A.~D.~L. and {Posch}, T. and {Vandenbussche}, B. and 
	{Waelkens}, C.},
    title = "{A far-infrared survey of bow shocks and detached shells around AGB stars and red supergiants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.5486},
 primaryClass = "astro-ph.GA",
 keywords = {stars: AGB and post-AGB, circumstellar matter, infrared: ISM, hydrodynamics, stars: mass-loss, stars: winds, outflows},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A35},
    pages = {A35},
      doi = {10.1051/0004-6361/201117910},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A..35C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{neilson_aa_529_2011,
   author = {{Neilson}, H.~R. and {Cantiello}, M. and {Langer}, N.},
    title = "{The Cepheid mass discrepancy and pulsation-driven mass loss}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1104.1638},
 primaryClass = "astro-ph.SR",
 keywords = {stars: mass-loss, stars: variables: Cepheids, stars: fundamental parameters},
     year = 2011,
    month = may,
   volume = 529,
      eid = {L9},
    pages = {L9},
      doi = {10.1051/0004-6361/201116920},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529L...9N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{noriegacrespo_aj_114_1997,
   author = {{Noriega-Crespo}, A. and {van Buren}, D. and {Cao}, Y. and {Dgani}, R.
	},
    title = "{A Parsec-Size Bow Shock around Betelgeuse}",
  journal = {\aj},
 keywords = {TURBULENCE, ISM: STRUCTURE, STARS: INDIVIDUAL: BETELGEUSE},
     year = 1997,
    month = aug,
   volume = 114,
    pages = {837-840},
      doi = {10.1086/118517},
   adsurl = {http://adsabs.harvard.edu/abs/1997AJ....114..837N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ntormousi_aa_589_2016,
   author = {{Ntormousi}, E. and {Hennebelle}, P. and {Andr{\'e}}, P. and 
	{Masson}, J.},
    title = "{The effect of ambipolar diffusion on low-density molecular ISM filaments}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1602.04737},
 keywords = {turbulence, magnetohydrodynamics (MHD), stars: formation, ISM: clouds, ISM: structure, ISM: magnetic fields},
     year = 2016,
    month = may,
   volume = 589,
      eid = {A24},
    pages = {A24},
      doi = {10.1051/0004-6361/201527400},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...589A..24N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE O 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{omukai_apj_722_2010,
   author = {{Omukai}, K. and {Hosokawa}, T. and {Yoshida}, N.},
    title = "{Low-metallicity Star Formation: Prestellar Collapse and Protostellar Accretion in the Spherical Symmetry}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1008.4262},
 keywords = {galaxies: formation, stars: formation, stars: Population II},
     year = 2010,
    month = oct,
   volume = 722,
    pages = {1793-1815},
      doi = {10.1088/0004-637X/722/2/1793},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...722.1793O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{orlando_aa_470_2007,
   author = {{Orlando}, S. and {Bocchino}, F. and {Reale}, F. and {Peres}, G. and 
	{Petruk}, O.},
    title = "{On the origin of asymmetries in bilateral supernova remnants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.0890},
 keywords = {magnetohydrodynamics (MHD), shock waves, ISM: supernova remnants, ISM: magnetic fields, radio continuum: ISM},
     year = 2007,
    month = aug,
   volume = 470,
    pages = {927-939},
      doi = {10.1051/0004-6361:20066045},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...470..927O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{orlando_apj_749_2012,
   author = {{Orlando}, S. and {Bocchino}, F. and {Miceli}, M. and {Petruk}, O. and 
	{Pumo}, M.~L.},
    title = "{Role of Ejecta Clumping and Back-reaction of Accelerated Cosmic Rays in the Evolution of Type Ia Supernova Remnants}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1202.3593},
 primaryClass = "astro-ph.HE",
 keywords = {cosmic rays, instabilities, ISM: supernova remnants, magnetohydrodynamics: MHD, shock waves, supernovae: individual: SN 1006},
     year = 2012,
    month = apr,
   volume = 749,
      eid = {156},
    pages = {156},
      doi = {10.1088/0004-637X/749/2/156},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...749..156O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ostriker_apj_184_1973,
   author = {{Ostriker}, J. and {Silk}, J.},
    title = "{Dust Cooling of Hot Gas}",
  journal = {\apjl},
     year = 1973,
    month = sep,
   volume = 184,
    pages = {L113},
      doi = {10.1086/181301},
   adsurl = {http://adsabs.harvard.edu/abs/1973ApJ...184L.113O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{offner_703_apj_2009,
   author = {{Offner}, S.~S.~R. and {Klein}, R.~I. and {McKee}, C.~F. and 
	{Krumholz}, M.~R.},
    title = "{The Effects of Radiative Transfer on Low-Mass Star Formation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0904.2004},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, ISM: clouds, ISM: kinematics and dynamics, methods: numerical, radiative transfer, stars: formation, turbulence},
     year = 2009,
    month = sep,
   volume = 703,
    pages = {131-149},
      doi = {10.1088/0004-637X/703/1/131},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703..131O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ostriker_revmodphys_60_1988,
   author = {{Ostriker}, J.~P. and {McKee}, C.~F.},
    title = "{Astrophysical blastwaves}",
  journal = {Reviews of Modern Physics},
     year = 1988,
   volume = 60,
    pages = {1-68},
      doi = {10.1103/RevModPhys.60.1},
   adsurl = {http://adsabs.harvard.edu/abs/1988RvMP...60....1O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{orlando_aa_444_2005,
   author = {{Orlando}, S. and {Peres}, G. and {Reale}, F. and {Bocchino}, F. and 
	{Rosner}, R. and {Plewa}, T. and {Siegel}, A.},
    title = "{Crushing of interstellar gas clouds in supernova remnants. I. The role of thermal conduction and radiative losses}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0508638},
 keywords = {hydrodynamics, shock waves, ISM: clouds, ISM: supernova remnants},
     year = 2005,
    month = dec,
   volume = 444,
    pages = {505-519},
      doi = {10.1051/0004-6361:20052896},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...444..505O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{orlando_apj_678_2008,
   author = {{Orlando}, S. and {Bocchino}, F. and {Reale}, F. and {Peres}, G. and 
	{Pagano}, P.},
    title = "{The Importance of Magnetic-Field-Oriented Thermal Conduction in the Interaction of SNR Shocks with Interstellar Clouds}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.1403},
 keywords = {Conduction, ISM: Clouds, ISM: Magnetic Fields, Magnetohydrodynamics: MHD, Shock Waves, ISM: Supernova Remnants},
     year = 2008,
    month = may,
   volume = 678,
    pages = {274-286},
      doi = {10.1086/529420},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...678..274O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ormel_mnras_447_2015,
   author = {{Ormel}, C.~W. and {Shi}, J.-M. and {Kuiper}, R.},
    title = "{Hydrodynamics of embedded planets' first atmospheres - II. A rapid recycling of atmospheric gas}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1410.4659},
 primaryClass = "astro-ph.EP",
 keywords = {hydrodynamics, planets and satellites: atmospheres, planets and satellites: formation, protoplanetary discs},
     year = 2015,
    month = mar,
   volume = 447,
    pages = {3512-3525},
      doi = {10.1093/mnras/stu2704},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447.3512O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{osterbrock_1989,
   author = {{Osterbrock}, D.~E. and {Bochkarev}, N.~G.},
    title = "{Book-Review - Astrophysics of Gaseous Nebulae and Active Galactic Nuclei}",
  journal = {\sovast},
     year = 1989,
    month = nov,
   volume = 33,
    pages = {694},
   adsurl = {http://adsabs.harvard.edu/abs/1989SvA....33..694O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE P 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{papaloizou_mnras_248_1991,
   author = {{Papaloizou}, J.~C. and {Savonije}, G.~J.},
    title = "{Instabilities in self-gravitating gaseous discs}",
  journal = {\mnras},
 keywords = {Accretion Disks, Cosmic Gases, Gravitational Effects, Rotating Fluids, Vorticity, Angular Momentum, Computational Astrophysics, Eigenvalues, Equations Of Motion, Planetary Rings},
     year = 1991,
    month = feb,
   volume = 248,
    pages = {353-369},
      doi = {10.1093/mnras/248.3.353},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.248..353P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{padoan_apj_730_2011,
   author = {{Padoan}, P. and {Nordlund}, {\AA}.},
    title = "{The Star Formation Rate of Supersonic Magnetohydrodynamic Turbulence}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0907.0248},
 primaryClass = "astro-ph.GA",
 keywords = {ISM: kinematics and dynamics, magnetohydrodynamics: MHD, stars: formation, turbulence},
     year = 2011,
    month = mar,
   volume = 730,
      eid = {40},
    pages = {40},
      doi = {10.1088/0004-637X/730/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...730...40P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{paardekooper_mnras_421_2012,
   author = {{Paardekooper}, S.-J.},
    title = "{Numerical convergence in self-gravitating shearing sheet simulations and the stochastic nature of disc fragmentation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.3371},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, hydrodynamics, instabilities, planets and satellites: formation, protoplanetary discs},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {3286-3299},
      doi = {10.1111/j.1365-2966.2012.20553.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012MNRAS.421.3286P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pannuti_147_aj_2014,
   author = {{Pannuti}, T.~G. and {Rho}, J. and {Heinke}, C.~O. and {Moffitt}, W.~P.
	},
    title = "{The X-Ray Properties of Five Galactic Supernova Remnants Detected by the Spitzer GLIMPSE Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1312.3929},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: individual objects: SNR 304.6+0.1 SNR 311.5{\ndash}0.3 SNR 346.6{\ndash}0.2 SNR 348.5+0.1 SNR 348.5{\ndash}0.0, ISM: supernova remnants, X-rays: ISM},
     year = 2014,
    month = mar,
   volume = 147,
      eid = {55},
    pages = {55},
      doi = {10.1088/0004-6256/147/3/55},
   adsurl = {http://adsabs.harvard.edu/abs/2014AJ....147...55P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{panic_aa_501_2005,
   author = {{Pani{\'c}}, O. and {Hogerheijde}, M.~R. and {Wilner}, D. and 
	{Qi}, C.},
    title = "{A break in the gas and dust surface density of the disc around the T Tauri star IM Lupi}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0904.1127},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems: protoplanetary disks, stars:, individual: IM Lup, stars: pre-main sequence, circumstellar matter},
     year = 2009,
    month = jul,
   volume = 501,
    pages = {269-278},
      doi = {10.1051/0004-6361/200911883},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...501..269P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{pagani_aa_429_2005,
   author = {{Pagani}, L. and {Apponi}, A.~J. and {Bacmann}, A. and {Cabrit}, S. and 
	{Cambr{\'e}sy}, L. and {Lagache}, G. and {Motte}, F. and {Pardo}, J.-R.
	},
    title = "{L183 (=L134N) revisited}",
 keywords = {L183, Depletion, CO},
booktitle = {ESA Special Publication},
     year = 2005,
   series = {ESA Special Publication},
   volume = 577,
   editor = "{A.~Wilson}",
    month = jan,
    pages = {403-404},
   adsurl = {http://adsabs.harvard.edu/abs/2005ESASP.577..403P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{parker_1963,
   author = {{Parker}, E.~N.},
    title = "{Interplanetary dynamical processes.}",
 keywords = {SOLAR SYSTEM, SOLAR RADIATION, SUN: CORONA},
booktitle = {New York, Interscience Publishers, 1963.},
     year = 1963,
   adsurl = {http://adsabs.harvard.edu/abs/1963QB505.P3.......},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{parker_mnras_362_2005,
   author = {{Parker}, Q.~A. and {Phillipps}, S. and {Pierce}, M.~J. and 
	{Hartley}, M. and {Hambly}, N.~C. and {Read}, M.~A. and {MacGillivray}},
    title = "{The AAO/UKST SuperCOSMOS H{$\alpha$} survey}",
  journal = {\mnras},
   eprint = {astro-ph/0506599},
 keywords = {astronomical data bases: miscellaneous, catalogues, surveys, stars: emission line, photometry},
     year = 2005,
    month = sep,
   volume = 362,
    pages = {689-710},
      doi = {10.1111/j.1365-2966.2005.09350.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005MNRAS.362..689P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pellegrini_bsrsl_80_2011,
   author = {{Pellegrini}, E.~W. and {Oey}, M.~S. and {Winkler}, P.~F. and 
	{Smith}, R.~C. and {Points}, S.},
    title = "{Escaping Radiation from Massive Star HII regions in the Magellanic Clouds}",
  journal = {Bulletin de la Societe Royale des Sciences de Liege},
     year = 2011,
    month = jan,
   volume = 80,
    pages = {410-414},
   adsurl = {http://adsabs.harvard.edu/abs/2011BSRSL..80..410P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{peresrendon_aa_506_2009,
   author = {{P{\'e}rez-Rend{\'o}n}, B. and {Garc{\'{\i}}a-Segura}, G. and 
	{Langer}, N.},
    title = "{Supernova progenitor stars in the initial range of 23 to 33 solar masses and their relation with the SNR Cassiopeia A}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0905.1101},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, ISM: kinematics and dynamics, ISM: supernova remnants, ISM: bubbles, ISM: individual objects: Cassiopeia A},
     year = 2009,
    month = nov,
   volume = 506,
    pages = {1249-1259},
      doi = {10.1051/0004-6361/200809913},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...506.1249P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{peri_aa_538_2012,
   author = {{Peri}, C.~S. and {Benaglia}, P. and {Brookes}, D.~P. and {Stevens}, I.~R. and 
	{Isequilla}, N.~L.},
    title = "{E-BOSS: an Extensive stellar BOw Shock Survey. I. Methods and first catalogue}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.3689},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: ISM, infrared: stars, stars: early-type, catalogs},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A108},
    pages = {A108},
      doi = {10.1051/0004-6361/201118116},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A.108P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{peters_apj_711_2010,
   author = {{Peters}, T. and {Banerjee}, R. and {Klessen}, R.~S. and {Mac Low}, M.-M. and 
	{Galv{\'a}n-Madrid}, R. and {Keto}, E.~R.},
    title = "{H II Regions: Witnesses to Massive Star Formation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1001.2470},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, H II regions, radiative transfer, stars: massive},
     year = 2010,
    month = mar,
   volume = 711,
    pages = {1017-1028},
      doi = {10.1088/0004-637X/711/2/1017},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...711.1017P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petri_aa_439_2005,
   author = {{P{\'e}tri}, J.},
    title = "{An explanation for the kHz-QPO twin peaks separation in slow and fast rotators}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0507167},
 keywords = {accretion, accretion disks, hydrodynamics, methods:, analytical, relativity, stars: neutron, X-rays: binaries},
     year = 2005,
    month = aug,
   volume = 439,
    pages = {L27-L30},
      doi = {10.1051/0004-6361:200500151},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...439L..27P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{petri_apr_302_2006,
   author = {{P'etri}, J.},
    title = "{Forced oscillations in a hydrodynamical accretion disk and QPOs}",
  journal = {\apss},
   eprint = {arXiv:astro-ph/0509668},
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, methods: analytical, methods: numerical, Stars: neutrongoodbreak},
     year = 2006,
    month = apr,
   volume = 302,
    pages = {117-139},
      doi = {10.1007/s10509-005-9013-8},
   adsurl = {http://adsabs.harvard.edu/abs/2006Ap%26SS.302..117P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PHDTHESIS{petrovic_phdt_2004,
   author = {{Petrovi{\'c}}, J.},
    title = "{On the evolution of massive close binary systems}",
 keywords = {magnetic fields, rotating stars, gamma-ray bursts, close binary stars, stellar evolution},
   school = {Utrecht University},
     year = 2004,
    month = October,
   adsurl = {http://adsabs.harvard.edu/abs/2004PhDT.......180P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petruk_393_mnras_2009,
   author = {{Petruk}, O. and {Dubner}, G. and {Castelletti}, G. and {Bocchino}, F. and 
	{Iakubovskyi}, D. and {Kirsch}, M.~G.~F. and {Miceli}, M. and 
	{Orlando}, S. and {Telezhinsky}, I.},
    title = "{Aspect angle for interstellar magnetic field in SN 1006}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0811.2319},
 keywords = {acceleration of particles , radiation mechanisms: non-thermal , shock waves , cosmic rays , ISM: individual: SN 1006 , supernova remnants},
     year = 2009,
    month = mar,
   volume = 393,
    pages = {1034-1040},
      doi = {10.1111/j.1365-2966.2008.14251.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.393.1034P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{penston_mnras_150_1970,
   author = {{Penston}, M.~V. and {Brown}, F.~E.},
    title = "{The doud-intercloud phase-change in the interstellar medium}",
  journal = {\mnras},
     year = 1970,
   volume = 150,
    pages = {373},
   adsurl = {http://adsabs.harvard.edu/abs/1970MNRAS.150..373P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{postnov_lrr_9_2006,
   author = {{Postnov}, K.~A. and {Yungelson}, L.~R.},
    title = "{The Evolution of Compact Binary Star Systems}",
  journal = {Living Reviews in Relativity},
   eprint = {arXiv:astro-ph/0701059},
 keywords = {relativity in astrophysics, binary systems, gravitational wave sources, supernovae, neutron stars, black holes, white dwarfs, AM CVn stars},
     year = 2006,
    month = dec,
   volume = 9,
    pages = {6},
   adsurl = {http://adsabs.harvard.edu/abs/2006LRR.....9....6P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{pound_apss_307_2007,
   author = {{Pound}, M.~W. and {Kane}, J.~O. and {Ryutov}, D.~D. and {Remington}, B.~A. and 
	{Mizuta}, A.},
    title = "{Pillars of Heaven}",
  journal = {\apss},
 keywords = {Eagle Nebula, Radio astronomy, Hydrodynamic models, Aperture synthesis},
     year = 2007,
    month = jan,
   volume = 307,
    pages = {187-190},
      doi = {10.1007/s10509-006-9214-9},
   adsurl = {http://adsabs.harvard.edu/abs/2007Ap%26SS.307..187P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pikelner_sovietastrlet_12_1969,
   author = {{Pikel'Ner}, S.~B. and {Shcheglov}, P.~V.},
    title = "{Gas Motions in Diffuse Nebulae and Stellar Wind.}",
  journal = {\sovast},
     year = 1969,
    month = apr,
   volume = 12,
    pages = {757},
   adsurl = {http://adsabs.harvard.edu/abs/1969SvA....12..757P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{piran_revmodphys_76_2004,
   author = {{Piran}, T.},
    title = "{The physics of gamma-ray bursts}",
  journal = {Reviews of Modern Physics},
   eprint = {arXiv:astro-ph/0405503},
     year = 2004,
    month = oct,
   volume = 76,
    pages = {1143-1210},
      doi = {10.1103/RevModPhys.76.1143},
   adsurl = {http://adsabs.harvard.edu/abs/2004RvMP...76.1143P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pudritz_prpl_277P_2007,
   author = {{Pudritz}, R.~E. and {Ouyed}, R. and {Fendt}, C. and {Brandenburg}, A.
	},
    title = "{Disk Winds, Jets, and Outflows: Theoretical and Computational Foundations}",
  journal = {Protostars and Planets V},
   eprint = {astro-ph/0603592},
     year = 2007,
    pages = {277-294},
   adsurl = {http://adsabs.harvard.edu/abs/2007prpl.conf..277P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE R 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{2005ApJ...621L..69R,
   author = {{Rafikov}, R.~R.},
    title = "{Can Giant Planets Form by Direct Gravitational Instability?}",
  journal = {\apjl},
   eprint = {astro-ph/0406469},
 keywords = {Planets and Satellites: Formation, Solar System: Formation},
     year = 2005,
    month = mar,
   volume = 621,
    pages = {L69-L72},
      doi = {10.1086/428899},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...621L..69R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rafikov_apj_704_2009,
   author = {{Rafikov}, R.~R.},
    title = "{Properties of Gravitoturbulent Accretion Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0901.4739},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion disks, instabilities, planetary systems: protoplanetary disks, quasars: general},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {281-291},
      doi = {10.1088/0004-637X/704/1/281},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009ApJ...704..281R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rafikov_apj_662_2007,
   author = {{Rafikov}, R.~R.},
    title = "{Convective Cooling and Fragmentation of Gravitationally Unstable Disks}",
  journal = {\apj},
   eprint = {astro-ph/0609549},
 keywords = {Stars: Planetary Systems: Protoplanetary Disks, Planets and Satellites: Formation, Solar System: Formation},
     year = 2007,
    month = jun,
   volume = 662,
    pages = {642-650},
      doi = {10.1086/517599},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...662..642R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{radhakrishnan_japa_1980,
   author = {{Radhakrishnan}, V. and {Srinivasan}, G.},
    title = "{Evidence for a Large Population of Shocked Interstellar Clouds}",
  journal = {Journal of Astrophysics and Astronomy},
 keywords = {21 CM ABSORPTION, SHOCKED CLOUDS, SPIN TEMPERATURE, HIGH VELOCITIES},
     year = 1980,
    month = sep,
   volume = 1,
    pages = {47-66},
      doi = {10.1007/BF02727949},
   adsurl = {http://adsabs.harvard.edu/abs/1980JApA....1...47R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{raga_rmxaa_33_1997,
   author = {{Raga}, A.~C. and {Noriega-Crespo}, A. and {Cant{\'o}}, J. and 
	{Steffen}, W. and {van Buren}, D. and {Mellema}, G. and {Lundqvist}, P.
	},
    title = "{The Bow Shock and H II Regions around a Runaway O Star}",
  journal = {\rmxaa},
     year = 1997,
    month = oct,
   volume = 33,
    pages = {73-81},
   adsurl = {http://adsabs.harvard.edu/abs/1997RMxAA..33...73R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{raga_apj_300_1086,
   author = {{Raga}, A.~C.},
    title = "{'Stromgren region' analysis of cometary H II regions}",
  journal = {\apj},
 keywords = {COMETS, H II REGIONS, NEBULAE, STELLAR MOTIONS, ASTRONOMICAL MODELS, GAS IONIZATION, PHOTONS, STELLAR ENVELOPES},
     year = 1986,
    month = jan,
   volume = 300,
    pages = {745-748},
      doi = {10.1086/163849},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...300..745R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{raga_apjs_109_1997,
   author = {{Raga}, A.~C. and {Mellema}, G. and {Lundqvist}, P.},
    title = "{An Axisymmetric, Radiative Bow Shock Model with a Realistic Treatment of Ionization and Cooling}",
  journal = {\apjs},
   eprint = {arXiv:astro-ph/9610134},
 keywords = {ATOMIC DATA, METHODS: NUMERICAL, RADIATIVE TRANSFER, SHOCK WAVES, STARS: PRE-MAIN-SEQUENCE},
     year = 1997,
    month = apr,
   volume = 109,
    pages = {517},
      doi = {10.1086/312987},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJS..109..517R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rakowski_apj_590_2003,
   author = {{Rakowski}, C.~E. and {Ghavamian}, P. and {Hughes}, J.~P.},
    title = "{The Physics of Supernova Remnant Blast Waves. II. Electron-Ion Equilibration in DEM L71 in the Large Magellanic Cloud}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0303069},
 keywords = {ISM: Individual: Alphanumeric: DEM L71, ISM: Individual: Alphanumeric: SNR 0505-67.9, Shock Waves, ISM: Supernova Remnants, X-Rays: ISM},
     year = 2003,
    month = jun,
   volume = 590,
    pages = {846-857},
      doi = {10.1086/375162},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...590..846R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{reach_aj_131_2006,
   author = {{Reach}, W.~T. and {Rho}, J. and {Tappe}, A. and {Pannuti}, T.~G. and 
	{Brogan}, C.~L. and {Churchwell}, E.~B. and {Meade}, M.~R. and 
	{Babler}, B. and {Indebetouw}, R. and {Whitney}, B.~A.},
    title = "{A Spitzer Space Telescope Infrared Survey of Supernova Remnants in the Inner Galaxy}",
  journal = {\aj},
   eprint = {astro-ph/0510630},
 keywords = {Infrared: ISM, Shock Waves, ISM: Supernova Remnants},
     year = 2006,
    month = mar,
   volume = 131,
    pages = {1479-1500},
      doi = {10.1086/499306},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.1479R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{reach_apj_511_1999,
   author = {{Reach}, W.~T. and {Rho}, J.},
    title = "{Excitation and Disruption of a Giant Molecular Cloud by the Supernova Remnant 3C 391}",
  journal = {\apj},
   eprint = {astro-ph/9804142},
 keywords = {ISM: INDIVIDUAL: ALPHANUMERIC: 3C 391, ISM: STRUCTURE, RADIO LINES: ISM, ISM: SUPERNOVA REMNANTS, ISM: Individual: Alphanumeric: 3C 391, ISM: Structure, Radio Lines: ISM, ISM: Supernova Remnants},
     year = 1999,
    month = feb,
   volume = 511,
    pages = {836-846},
      doi = {10.1086/306703},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...511..836R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{rybicki_rap_1979,
   author = {{Rybicki}, G.~B. and {Lightman}, A.~P.},
    title = "{Radiative processes in astrophysics}",
 keywords = {Astrophysics, Radiative Transfer, Atomic Structure, Bremsstrahlung, Compton Effect, Covariance, Kinematics, Molecular Structure, Plasma Radiation, Radiation Distribution, Relativistic Effects, Synchrotron Radiation},
booktitle = {New York, Wiley-Interscience, 1979.~393 p.},
     year = 1979,
   adsurl = {http://adsabs.harvard.edu/abs/1979rpa..book.....R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{roepks_apj_668_2007,
   author = {{R{\"o}pke}, F.~K.},
    title = "{Flame-driven Deflagration-to-Detonation Transitions in Type Ia Supernovae?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0709.4095},
 keywords = {Hydrodynamics, Instabilities, Methods: Numerical, Stars: Supernovae: General, Turbulence},
     year = 2007,
    month = oct,
   volume = 668,
    pages = {1103-1108},
      doi = {10.1086/520830},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...668.1103R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{roger_mnras_423_2012,
   author = {{Rogers}, P.~D. and {Wadsley}, J.},
    title = "{The fragmentation of protostellar discs: the Hill criterion for spiral arms}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1111.1985},
 primaryClass = "astro-ph.EP",
 keywords = {hydrodynamics, radiative transfer, methods: numerical, protoplanetary discs, planetary systems},
     year = 2012,
    month = jun,
   volume = 423,
    pages = {1896-1908},
      doi = {10.1111/j.1365-2966.2012.21014.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.423.1896R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170604657R,
   author = {{Reiter}, M. and {Kiminki}, M.~M. and {Smith}, N. and {Bally}, J.
	},
    title = "{Proper motions of collimated jets from intermediate-mass protostars in the Carina Nebula}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1706.04657},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170604657R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{reid_apj_705_2009,
   author = {{Reid}, M.~J. and {Menten}, K.~M. and {Zheng}, X.~W. and {Brunthaler}, A. and 
	{Xu}, Y.},
    title = "{A Trigonometric Parallax of Sgr B2}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.3637},
 primaryClass = "astro-ph.GA",
 keywords = {astrometry, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, stars: formation},
     year = 2009,
    month = nov,
   volume = 705,
    pages = {1548-1553},
      doi = {10.1088/0004-637X/705/2/1548},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...705.1548R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{robitaille_aa_536_2011,
   author = {{Robitaille}, T.~P.},
    title = "{HYPERION: an open-source parallelized three-dimensional dust continuum radiative transfer code}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1112.1071},
 primaryClass = "astro-ph.IM",
 keywords = {methods: numerical, radiative transfer, scattering, polarization},
     year = 2011,
    month = dec,
   volume = 536,
      eid = {A79},
    pages = {A79},
      doi = {10.1051/0004-6361/201117150},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...536A..79R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{roepke_apj_660_2007,
   author = {{R{\"o}pke}, F.~K. and {Woosley}, S.~E. and {Hillebrandt}, W.
	},
    title = "{Off-Center Ignition in Type Ia Supernovae. I. Initial Evolution and Implications for Delayed Detonation}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0609088},
 keywords = {Hydrodynamics, Instabilities, Methods: Numerical, Stars: Supernovae: General, Turbulence},
     year = 2007,
    month = may,
   volume = 660,
    pages = {1344-1356},
      doi = {10.1086/512769},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660.1344R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{roepke_aa_420_2004,
   author = {{R{\"o}pke}, F.~K. and {Hillebrandt}, W. and {Niemeyer}, J.~C.
	},
    title = "{The cellular burning regime in type Ia supernova explosions. I. Flame propagation into quiescent fuel}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0312092},
 keywords = {stars: supernovae: general, hydrodynamics, instabilities},
     year = 2004,
    month = jun,
   volume = 420,
    pages = {411-422},
      doi = {10.1051/0004-6361:20035721},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...420..411R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{roepke_aa_421_2004,
   author = {{R{\"o}pke}, F.~K. and {Hillebrandt}, W. and {Niemeyer}, J.~C.
	},
    title = "{The cellular burning regime in type Ia supernova explosions. II. Flame propagation into vortical fuel}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0312203},
 keywords = {stars: supernovae: general, hydrodynamics, instabilities, turbulence},
     year = 2004,
    month = jul,
   volume = 421,
    pages = {783-795},
      doi = {10.1051/0004-6361:20035778},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...421..783R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rozyczka_apj_423_1994,
   author = {{Rozyczka}, M. and {Bodenheimer}, P. and {Bell}, K.~R.},
    title = "{A Numerical Study of Viscous Flows in Axisymmetric alpha -Accretion Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, RADIATIVE TRANSFER, STARS: FORMATION},
     year = 1994,
    month = mar,
   volume = 423,
    pages = {736},
      doi = {10.1086/173853},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...423..736R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rozyczka_274_MNRAS_1995,
   author = {{Rozyczka}, M. and {Tenorio-Tagle}, G.},
    title = "{The evolution of compact supernova remnants in a strongly magnetized medium}",
  journal = {\mnras},
 keywords = {ISM: JETS AND OUTFLOWS, ISM: MAGNETIC FIELDS, SUPERNOVA REMNANTS, GALAXIES: ACTIVE},
     year = 1995,
    month = jun,
   volume = 274,
    pages = {1157-1164},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.274.1157R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{rozyczka_aa_167_1986,
   author = {{Rozyczka}, M. and {Tenorio-Tagle}, G. and {Bodenheimer}, P.
	},
    title = "{Non-spherical supernova remnants. III - Oblique shock reflections and anomalous H I velocity features}",
  journal = {\aap},
 keywords = {Collisions, Interstellar Matter, Mach Reflection, Supernova Remnants, Adiabatic Conditions, Radiant Cooling, Two Dimensional Models},
     year = 1986,
    month = oct,
   volume = 167,
    pages = {120-128},
   adsurl = {http://adsabs.harvard.edu/abs/1986A%26A...167..120R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rosen_jcp_330_2017,
   author = {{Rosen}, A.~L. and {Krumholz}, M.~R. and {Oishi}, J.~S. and 
	{Lee}, A.~T. and {Klein}, R.~I.},
    title = "{Hybrid Adaptive Ray-Moment Method (HARM$^{2}$): A highly parallel method for radiation hydrodynamics on adaptive grids}",
  journal = {Journal of Computational Physics},
archivePrefix = "arXiv",
   eprint = {1607.01802},
 primaryClass = "astro-ph.IM",
 keywords = {Radiative transfer, Hydrodynamics, Parallelization, Long characteristics, Adaptive mesh refinement},
     year = 2017,
    month = feb,
   volume = 330,
    pages = {924-942},
      doi = {10.1016/j.jcp.2016.10.048},
   adsurl = {http://adsabs.harvard.edu/abs/2017JCoPh.330..924R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{rosen_mnras_463_2016,
   author = {{Rosen}, A.~L. and {Krumholz}, M.~R. and {McKee}, C.~F. and 
	{Klein}, R.~I.},
    title = "{An unstable truth: how massive stars get their mass}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1607.03117},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, instabilities, stars: formation, stars: massive, ISM: bubbles},
     year = 2016,
    month = dec,
   volume = 463,
    pages = {2553-2573},
      doi = {10.1093/mnras/stw2153},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.463.2553R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{rozyczka_mnras_261_1993,
   author = {{Rozyczka}, M. and {Tenorio-Tagle}, G. and {Franco}, J. and 
	{Bodenheimer}, P.},
    title = "{On the evolution of supernova remnants. III - Off-centred supernova explosions in pre-existing wind-driven bubbles}",
  journal = {\mnras},
 keywords = {Plasma Bubbles, Stellar Evolution, Stellar Winds, Supernova Remnants, Interstellar Matter, Stellar Structure},
     year = 1993,
    month = apr,
   volume = 261,
    pages = {674-680},
   adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.261..674R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rice_mnras_420_2012,
   author = {{Rice}, W.~K.~M. and {Forgan}, D.~H. and {Armitage}, P.~J.},
    title = "{Convergence of smoothed particle hydrodynamics simulations of self-gravitating accretion discs: sensitivity to the implementation of radiative cooling}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1111.3147},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, gravitation, instabilities, stars: formation},
     year = 2012,
    month = feb,
   volume = 420,
    pages = {1640-1647},
      doi = {10.1111/j.1365-2966.2011.20153.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420.1640R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rice_mnras_364_2005,
   author = {{Rice}, W.~K.~M. and {Lodato}, G. and {Armitage}, P.~J.},
    title = "{Investigating fragmentation conditions in self-gravitating accretion discs}",
  journal = {\mnras},
   eprint = {astro-ph/0509413},
 keywords = {accretion, accretion discs, gravitation, instabilities, stars: formation, galaxies: active, galaxies: spiral},
     year = 2005,
    month = nov,
   volume = 364,
    pages = {L56-L60},
      doi = {10.1111/j.1745-3933.2005.00105.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.364L..56R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rice_mnras_438_2014,
   author = {{Rice}, W.~K.~M. and {Paardekooper}, S.-J. and {Forgan}, D.~H. and 
	{Armitage}, P.~J.},
    title = "{Convergence of simulations of self-gravitating accretion discs - II. Sensitivity to the implementation of radiative cooling and artificial viscosity}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1311.7355},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion discs, gravitation, instabilities, planets and satellites: formation, stars: formation},
     year = 2014,
    month = feb,
   volume = 438,
    pages = {1593-1602},
      doi = {10.1093/mnras/stt2297},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.1593R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{richling_aa_327_1997,
   author = {{Richling}, S. and {Yorke}, H.~W.},
    title = "{Photoevaporation of protostellar disks. II. The importance of UV dust properties and ionizing flux.}",
  journal = {\aap},
 keywords = {RADIATION TRANSFER, STARS: CIRCUMSTELLAR MATTER, STARS: FORMATION OF, ISM: JETS AND OUTFLOWS, HII REGIONS},
     year = 1997,
    month = nov,
   volume = 327,
    pages = {317-324},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...327..317R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{richling_aa_340_1998,
   author = {{Richling}, S. and {Yorke}, H.~W.},
    title = "{Photoevaporation of protostellar disks. IV. Externally illuminated disks}",
  journal = {\aap},
 keywords = {ISM: H II REGIONS, STARS: FORMATION, STARS: CIRCUMSTELLAR MATTER, RADIATIVE TRANSFER},
     year = 1998,
    month = dec,
   volume = 340,
    pages = {508-520},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...340..508R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{richling_apj_539_2000,
   author = {{Richling}, S. and {Yorke}, H.~W.},
    title = "{Photoevaporation of Protostellar Disks. V. Circumstellar Disks under the Influence of Both Extreme-Ultraviolet and Far-Ultraviolet Radiation}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, Hydrodynamics, ISM: H II Regions, Line: Formation, Radiative Transfer, Stars: Formation},
     year = 2000,
    month = aug,
   volume = 539,
    pages = {258-272},
      doi = {10.1086/309198},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...539..258R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...421..615P,
   author = {{Pollack}, J.~B. and {Hollenbach}, D. and {Beckwith}, S. and 
	{Simonelli}, D.~P. and {Roush}, T. and {Fong}, W.},
    title = "{Composition and radiative properties of grains in molecular clouds and accretion disks}",
  journal = {\apj},
 keywords = {Accretion Disks, Astronomical Models, Cosmic Dust, Interstellar Matter, Molecular Clouds, Stellar Composition, Stellar Mass Accretion, Abundance, Grain Size, Iron, Olivine, Pyroxenes, Water},
     year = 1994,
    month = feb,
   volume = 421,
    pages = {615-639},
      doi = {10.1086/173677},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...421..615P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ruden_apj_375_1991,
   author = {{Ruden}, S.~P. and {Pollack}, J.~B.},
    title = "{The dynamical evolution of the protosolar nebula}",
  journal = {\apj},
 keywords = {Protostars, Solar Corona, Solar System Evolution, Star Formation, Angular Momentum, Gas Dynamics, Planetary Evolution},
     year = 1991,
    month = jul,
   volume = 375,
    pages = {740-760},
      doi = {10.1086/170239},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...375..740R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE S 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{sana_sci_337_2012,
   author = {{Sana}, H. and {de Mink}, S.~E. and {de Koter}, A. and {Langer}, N. and 
	{Evans}, C.~J. and {Gieles}, M. and {Gosset}, E. and {Izzard}, R.~G. and 
	{Le Bouquin}, J.-B. and {Schneider}, F.~R.~N.},
    title = "{Binary Interaction Dominates the Evolution of Massive Stars}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1207.6397},
 primaryClass = "astro-ph.SR",
     year = 2012,
    month = jul,
   volume = 337,
    pages = {444},
      doi = {10.1126/science.1223344},
   adsurl = {http://adsabs.harvard.edu/abs/2012Sci...337..444S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stamatellos_mnras_400_2009,
   author = {{Stamatellos}, D. and {Whitworth}, A.~P.},
    title = "{The role of thermodynamics in disc fragmentation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0908.2247},
 keywords = {accretion, accretion discs , hydrodynamics , radiative transfer , methods: numerical , stars: formation , stars: low-mass, brown dwarfs},
     year = 2009,
    month = dec,
   volume = 400,
    pages = {1563-1573},
      doi = {10.1111/j.1365-2966.2009.15564.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009MNRAS.400.1563S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seifried_mnras_417_2011,
   author = {{Seifried}, D. and {Banerjee}, R. and {Klessen}, R.~S. and {Duffin}, D. and 
	{Pudritz}, R.~E.},
    title = "{Magnetic fields during the early stages of massive star formation - I. Accretion and disc evolution}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1106.4485},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, magnetic fields, methods: numerical, stars: formation, stars: massive},
     year = 2011,
    month = oct,
   volume = 417,
    pages = {1054-1073},
      doi = {10.1111/j.1365-2966.2011.19320.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417.1054S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seifried_mnras_422_2012,
   author = {{Seifried}, D. and {Pudritz}, R.~E. and {Banerjee}, R. and {Duffin}, D. and 
	{Klessen}, R.~S.},
    title = "{Magnetic fields during the early stages of massive star formation - II. A generalized outflow criterion}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1109.4379},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, magnetic fields, methods: numerical, stars: formation, stars: massive, stars: winds, outflows},
     year = 2012,
    month = may,
   volume = 422,
    pages = {347-366},
      doi = {10.1111/j.1365-2966.2012.20610.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422..347S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seifried_mnras_432_2013,
   author = {{Seifried}, D. and {Banerjee}, R. and {Pudritz}, R.~E. and {Klessen}, R.~S.
	},
    title = "{Turbulence-induced disc formation in strongly magnetized cloud cores}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1302.4901},
 keywords = {accretion, accretion discs, MHD, methods: numerical, stars: formation},
     year = 2013,
    month = jul,
   volume = 432,
    pages = {3320-3331},
      doi = {10.1093/mnras/stt682},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.432.3320S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{peters_mnras_437_2014,
   author = {{Peters}, T. and {Klaassen}, P.~D. and {Seifried}, D. and {Banerjee}, R. and 
	{Klessen}, R.~S.},
    title = "{Morphologies of protostellar outflows: an ALMA view}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.7356},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, MHD, radiative transfer, stars: formation, ISM: jets and outflows, submillimetre: ISM},
     year = 2014,
    month = jan,
   volume = 437,
    pages = {2901-2908},
      doi = {10.1093/mnras/stt2104},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.437.2901P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seifried_mnras_446_2015,
   author = {{Seifried}, D. and {Banerjee}, R. and {Pudritz}, R.~E. and {Klessen}, R.~S.
	},
    title = "{Accretion and magnetic field morphology around Class 0 stage protostellar discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1408.2989},
 keywords = {accretion, accretion discs, MHD, methods: numerical, stars: formation},
     year = 2015,
    month = jan,
   volume = 446,
    pages = {2776-2788},
      doi = {10.1093/mnras/stu2282},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.2776S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seifried_mnras_571_2016,
   author = {{Seifried}, D. and {S{\'a}nchez-Monge}, {\'A}. and {Walch}, S. and 
	{Banerjee}, R.},
    title = "{Revealing the dynamics of Class 0 protostellar discs with ALMA}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1601.02384},
 primaryClass = "astro-ph.SR",
 keywords = {MHD, methods: numerical, stars: formation, accretion discs, methods: observational, techniques: interferometric},
     year = 2016,
    month = apr,
      doi = {10.1093/mnras/stw785},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.tmp..571S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{seifried_mnras_423_2012,
   author = {{Seifried}, D. and {Banerjee}, R. and {Pudritz}, R.~E. and {Klessen}, R.~S.
	},
    title = "{Disc formation in turbulent massive cores: circumventing the magnetic braking catastrophe}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.5302},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, MHD, methods: numerical, stars: formation},
     year = 2012,
    month = jun,
   volume = 423,
    pages = {L40-L44},
      doi = {10.1111/j.1745-3933.2012.01253.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.423L..40S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schleicher_aa_585_2016,
   author = {{Schleicher}, D.~R.~G. and {Bovino}, S. and {Latif}, M.~A. and 
	{Ferrara}, A. and {Grassi}, T.},
    title = "{The chemical evolution of self-gravitating primordial disks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1504.06296},
 keywords = {cosmology: theory, dark ages, reionization, first stars, accretion, accretion disks, astrochemistry, stars: formation, stars: Population III},
     year = 2016,
    month = jan,
   volume = 585,
      eid = {A11},
    pages = {A11},
      doi = {10.1051/0004-6361/201526356},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...585A..11S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schlegel_mnras_244_1990,
   author = {{Schlegel}, E.~M.},
    title = "{A new subclass of Type II supernovae?}",
  journal = {\mnras},
 keywords = {Stellar Evolution, Supernovae, Classifying, H Alpha Line, Stellar Spectra, Supernova 1987a},
     year = 1990,
    month = may,
   volume = 244,
    pages = {269-271},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.244..269S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schneiter_mnras_408_2010,
   author = {{Schneiter}, E.~M. and {Vel{\'a}zquez}, P.~F. and {Reynoso}, E.~M. and 
	{de Colle}, F.},
    title = "{An MHD study of SN 1006 and determination of the ambient magnetic field direction}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1006.1150},
 primaryClass = "astro-ph.SR",
 keywords = {MHD, radiation mechanisms: general, methods: numerical, supernovae: individual: SN 1006, ISM: supernova remnants},
     year = 2010,
    month = oct,
   volume = 408,
    pages = {430-435},
      doi = {10.1111/j.1365-2966.2010.17125.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408..430S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schonrich_mnras_403_2010,
   author = {{Sch{\"o}nrich}, R. and {Binney}, J. and {Dehnen}, W.},
    title = "{Local kinematics and the local standard of rest}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0912.3693},
 primaryClass = "astro-ph.GA",
 keywords = {stars: kinematics, Galaxy: disc, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, solar neighbourhood},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {1829-1833},
      doi = {10.1111/j.1365-2966.2010.16253.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403.1829S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{schure_mnras_435_2013,
   author = {{Schure}, K.~M. and {Bell}, A.~R.},
    title = "{Cosmic ray acceleration in young supernova remnants}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1307.6575},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, instabilities, MHD, cosmic rays, ISM: supernova remnants},
     year = 2013,
    month = oct,
   volume = 435,
    pages = {1174-1185},
      doi = {10.1093/mnras/stt1371},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435.1174S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sedov_MoIzN_1977,
   author = {{Sedov}, L.~I.},
    title = "{Similarity methods and dimensional analysis in mechanics /8th revised edition/}",
  journal = {Moscow Izdatel Nauka},
 keywords = {DIMENSIONAL ANALYSIS, MATHEMATICAL MODELS, MECHANICS (PHYSICS), SIMILARITY THEOREM, AERODYNAMIC CHARACTERISTICS, ASTROPHYSICS, COMBUSTION PHYSICS, GAS DYNAMICS, PIPE FLOW, TURBULENT FLOW, UNSTEADY FLOW, VISCOUS FLOW, WAVE PROPAGATION},
     year = 1977,
   adsurl = {http://adsabs.harvard.edu/abs/1977MoIzN....Q....S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{seok_apj_779_2013,
   author = {{Seok}, J.~Y. and {Koo}, B.-C. and {Onaka}, T.},
    title = "{A Survey of Infrared Supernova Remnants in the Large Magellanic Cloud}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1312.0460},
 primaryClass = "astro-ph.HE",
 keywords = {dust, extinction, ISM: supernova remnants, Magellanic Clouds },
     year = 2013,
    month = dec,
   volume = 779,
      eid = {134},
    pages = {134},
      doi = {10.1088/0004-637X/779/2/134},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779..134S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shakura_aa_24_1973,
   author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
    title = "{Black holes in binary systems. Observational appearance.}",
  journal = {\aap},
     year = 1973,
   volume = 24,
    pages = {337-355},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....24..337S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{shepherd_apj_472_1996,
   author = {{Shepherd}, D.~S. and {Churchwell}, E.},
    title = "{Bipolar Molecular Outflows in Massive Star Formation Regions}",
  journal = {\apj},
 keywords = {STARS: FORMATION, ISM: H II REGIONS, ISM: JETS AND OUTFLOWS, ISM: MOLECULES, STARS: PRE-MAIN-SEQUENCE},
     year = 1996,
    month = nov,
   volume = 472,
    pages = {225},
      doi = {10.1086/178057},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...472..225S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{shu_apj_687_2008,
   author = {{Mohanty}, S. and {Shu}, F.~H.},
    title = "{Magnetocentrifugally Driven Flows from Young Stars and Disks. VI. Accretion with a Multipole Stellar Field}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0806.4769},
 keywords = {circumstellar matter, stars: formation, stars: low-mass, brown dwarfs, stars: pre-main sequence },
     year = 2008,
    month = nov,
   volume = 687,
      eid = {1323-1338},
    pages = {1323-1338},
      doi = {10.1086/591924},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...687.1323M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shu_apj_459_1996,
   author = {{Shu}, F.~H. and {Najita}, J. and {Ostriker}, E.~C. and {Shang}, H.
	},
    title = "{Magnetocentrifugally Driven Flows from Young Stars and Disks. V. Collimation into Jets: Erratum}",
  journal = {\apjl},
 keywords = {ERRATA, ADDENDA},
     year = 1996,
    month = mar,
   volume = 459,
    pages = {L43},
      doi = {10.1086/309941},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...459L..43S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shu_apj_447_1995,
   author = {{Ostriker}, E.~C. and {Shu}, F.~H.},
    title = "{Magnetocentrifugally Driven Flows from Young Stars and Disks. IV. The Accretion Funnel and Dead Zone}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, MAGNETOHYDRODYNAMICS: MHD, STARS: PRE-MAIN-SEQUENCE},
     year = 1995,
    month = jul,
   volume = 447,
    pages = {813},
      doi = {10.1086/175920},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...447..813O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shu_apj_429_1994,
   author = {{Najita}, J.~R. and {Shu}, F.~H.},
    title = "{Magnetocentrifugally driven flows from young stars and disks. 3: Numerical solution of the sub-Alfvenic region}",
  journal = {\apj},
 keywords = {Astronomical Models, Centrifugal Force, Disk Galaxies, Magnetic Fields, Mass Flow, Protostars, Star Formation, Stellar Mass Accretion, T Tauri Stars, Axisymmetric Flow, Bernoulli Theorem, Boundary Conditions, Coordinate Transformations, Magnetohydrodynamic Flow, Numerical Analysis, Steady Flow, Stellar Winds},
     year = 1994,
    month = jul,
   volume = 429,
    pages = {808-825},
      doi = {10.1086/174365},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...429..808N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shu_apj_429_1994,
   author = {{Shu}, F.~H. and {Najita}, J. and {Ruden}, S.~P. and {Lizano}, S.
	},
    title = "{Magnetocentrifugally driven flows from young stars and disks. 2: Formulation of the dynamical problem}",
  journal = {\apj},
 keywords = {Astronomical Models, Centrifugal Force, Disk Galaxies, Formulations, Magnetic Fields, Mass Flow, Protostars, T Tauri Stars, Analytic Functions, Angular Momentum, Asymptotic Series, Axisymmetric Flow, Boundary Value Problems, Magnetohydrodynamic Flow, Numerical Analysis, Partial Differential Equations},
     year = 1994,
    month = jul,
   volume = 429,
    pages = {797-807},
      doi = {10.1086/174364},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...429..797S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shu_apj_429_1994,
   author = {{Shu}, F. and {Najita}, J. and {Ostriker}, E. and {Wilkin}, F. and 
	{Ruden}, S. and {Lizano}, S.},
    title = "{Magnetocentrifugally driven flows from young stars and disks. 1: A generalized model}",
  journal = {\apj},
 keywords = {Astronomical Models, Centrifugal Force, Disk Galaxies, Magnetic Fields, Mass Flow, Protostars, Stellar Mass Accretion, T Tauri Stars, Angular Momentum, Numerical Analysis, Stellar Winds, Terminal Velocity},
     year = 1994,
    month = jul,
   volume = 429,
    pages = {781-796},
      doi = {10.1086/174363},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...429..781S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{shu_apj_214_1977,
   author = {{Shu}, F.~H.},
    title = "{Self-similar collapse of isothermal spheres and star formation}",
  journal = {\apj},
 keywords = {Density Distribution, Gravitational Collapse, Isothermal Flow, Protostars, Star Formation, Stellar Structure, Critical Point, Runge-Kutta Method, Similarity Theorem, Steady State, Stellar Envelopes},
     year = 1977,
    month = jun,
   volume = 214,
    pages = {488-497},
      doi = {10.1086/155274},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...214..488S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shulyak_aap_428_2004,
   author = {{Shulyak}, D. and {Tsymbal}, V. and {Ryabchikova}, T. and {St{\"u}tz}, C. and 
	{Weiss}, W.~W.},
    title = "{Line-by-line opacity stellar model atmospheres}",
  journal = {\aap},
 keywords = {stars: atmospheres, stars: abundances, stars: chemically peculiar, stars: fundamental parameters, stars: individual: CU Vir, stars: individual: HD 124224},
     year = 2004,
    month = dec,
   volume = 428,
    pages = {993-1000},
      doi = {10.1051/0004-6361:20034169},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...428..993S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smith_mnras_424_2012,
   author = {{Smith}, R.~J. and {Hosokawa}, T. and {Omukai}, K. and {Glover}, S.~C.~O. and 
	{Klessen}, R.~S.},
    title = "{Variable accretion rates and fluffy first stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1112.4157},
 keywords = {stars: formation, stars: Population III, stars: pre-main-sequence, early Universe},
     year = 2012,
    month = jul,
   volume = 424,
    pages = {457-463},
      doi = {10.1111/j.1365-2966.2012.21211.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012MNRAS.424..457S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smith_MNRAS_339_2003,
   author = {{Smith}, M.~D. and {Rosen}, A.},
    title = "{The instability of fast shocks in molecular clouds}",
  journal = {\mnras},
 keywords = {hydrodynamics, instabilities, molecular processes, shock waves, ISM: lines and bands, ISM: molecules},
     year = 2003,
    month = feb,
   volume = 339,
    pages = {133-147},
      doi = {10.1046/j.1365-8711.2003.06155.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.339..133S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stamatellos_mnras_413_2011,
   author = {{Stamatellos}, D. and {Maury}, A. and {Whitworth}, A. and {Andr{\'e}}, P.
	},
    title = "{The lower limits of disc fragmentation and the prospects for observing fragmenting discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1012.3455},
 keywords = {accretion, accretion discs, hydrodynamics, radiative transfer, methods: numerical, brown dwarfs, stars: formation, stars: low-mass},
     year = 2011,
    month = may,
   volume = 413,
    pages = {1787-1796},
      doi = {10.1111/j.1365-2966.2011.18254.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413.1787S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stamatellos_apj_730_2011,
   author = {{Stamatellos}, D. and {Whitworth}, A.~P. and {Hubber}, D.~A.
	},
    title = "{The Importance of Episodic Accretion for Low-mass Star Formation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1103.1378},
 keywords = {accretion, accretion disks, brown dwarfs, hydrodynamics, methods: numerical, radiative transfer, stars: formation, stars: low-mass, stars: protostars},
     year = 2011,
    month = mar,
   volume = 730,
      eid = {32},
    pages = {32},
      doi = {10.1088/0004-637X/730/1/32},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...730...32S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stacy_mnras_403_2010,
   author = {{Stacy}, A. and {Greif}, T.~H. and {Bromm}, V.},
    title = "{The first stars: formation of binaries and small multiple systems}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0908.0712},
 keywords = {stars: formation, galaxies: formation, cosmology: theory, early Universe},
     year = 2010,
    month = mar,
   volume = 403,
    pages = {45-60},
      doi = {10.1111/j.1365-2966.2009.16113.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403...45S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stevens_apj_386_1992,
   author = {{Stevens}, I.~R. and {Blondin}, J.~M. and {Pollock}, A.~M.~T.
	},
    title = "{Colliding winds from early-type stars in binary systems}",
  journal = {\apj},
 keywords = {BINARY STARS, EARLY STARS, PLASMA INTERACTIONS, STELLAR WINDS, WOLF-RAYET STARS, X RAY STARS, HYDRODYNAMIC EQUATIONS, RADIATIVE TRANSFER, SHOCK WAVE INTERACTION, STELLAR LUMINOSITY, STELLAR MODELS},
     year = 1992,
    month = feb,
   volume = 386,
    pages = {265-287},
      doi = {10.1086/171013},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...386..265S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stroemgren_apj_89_1939,
   author = {{Str{\"o}mgren}, B.},
    title = "{The Physical State of Interstellar Hydrogen.}",
  journal = {\apj},
     year = 1939,
    month = may,
   volume = 89,
    pages = {526},
      doi = {10.1086/144074},
   adsurl = {http://adsabs.harvard.edu/abs/1939ApJ....89..526S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stoll_aa_572_2014,
   author = {{Stoll}, M.~H.~R. and {Kley}, W.},
    title = "{Vertical shear instability in accretion disc models with radiation transport}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1409.8429},
 primaryClass = "astro-ph.EP",
 keywords = {hydrodynamics, instabilities, accretion, accretion disks, radiative transfer},
     year = 2014,
    month = dec,
   volume = 572,
      eid = {A77},
    pages = {A77},
      doi = {10.1051/0004-6361/201424114},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...572A..77S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stone_apjs_80_1992,
   author = {{Stone}, J.~M. and {Norman}, M.~L.},
    title = "{ZEUS-2D: A radiation magnetohydrodynamics code for astrophysical flows in two space dimensions. I - The hydrodynamic algorithms and tests.}",
  journal = {\apjs},
 keywords = {Computational Astrophysics, Cosmic Plasma, Hydrodynamic Equations, Magnetohydrodynamic Flow, Self Consistent Fields, Computational Grids, Finite Difference Theory, Plasma Radiation, Poisson Equation, Radiative Transfer},
     year = 1992,
    month = jun,
   volume = 80,
    pages = {753-790},
      doi = {10.1086/191680},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJS...80..753S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Book{strunk_1918,
	title = "The elements of style",
	author = "W. Jr Strunk",
	edition = "New York",
	year = "1918"
}

@ARTICLE{spitzer_apj_164_1971,
   author = {{Spitzer}, Jr., L. and {Hart}, M.~H.},
    title = "{Random Gravitational Encounters and the Evolution of Spherical Systems. I. Method}",
  journal = {\apj},
     year = 1971,
    month = mar,
   volume = 164,
    pages = {399},
      doi = {10.1086/150855},
   adsurl = {http://adsabs.harvard.edu/abs/1971ApJ...164..399S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{spitzer_apj_166_1971,
   author = {{Spitzer}, Jr., L. and {Hart}, M.~H.},
    title = "{Random Gravitational Encounters and the Evolution of Spherical Systems. II. Models}",
  journal = {\apj},
     year = 1971,
    month = jun,
   volume = 166,
    pages = {483},
      doi = {10.1086/150977},
   adsurl = {http://adsabs.harvard.edu/abs/1971ApJ...166..483S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{spitzer_apj_173_1972,
   author = {{Spitzer}, Jr., L. and {Shapiro}, S.~L.},
    title = "{Random Gravitational Encounters and the Evolution of Spherical Systems. III. Halo}",
  journal = {\apj},
     year = 1972,
    month = may,
   volume = 173,
    pages = {529},
      doi = {10.1086/151442},
   adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...173..529S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{spitzer_apj_175_1972,
   author = {{Spitzer}, Jr., L. and {Thuan}, T.~X.},
    title = "{Random Gravitational Encounters and the Evolution of Spherical Systems. IV Isolated Systems of Identical Stars}",
  journal = {\apj},
     year = 1972,
    month = jul,
   volume = 175,
    pages = {31},
      doi = {10.1086/151537},
   adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...175...31S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@BOOK{spitzer_1962,
   author = {{Spitzer}, L.},
    title = "{Physics of Fully Ionized Gases}",
booktitle = {Physics of Fully Ionized Gases, New York: Interscience (2nd edition), 1962},
     year = 1962,
   adsurl = {http://adsabs.harvard.edu/abs/1962pfig.book.....S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{sutherland_apjs_88_1993,
   author = {{Sutherland}, R.~S. and {Dopita}, M.~A.},
    title = "{Cooling functions for low-density astrophysical plasmas}",
  journal = {\apjs},
 keywords = {Cooling Flows (Astrophysics), Cosmic Plasma, Nonequilibrium Ionization, One Dimensional Flow, Plasma Slabs, Radiative Transfer, Charge Exchange, Electron Impact, Grid Generation (Mathematics), Hydrogen Recombinations, Ionization, Mathematical Models, Metallicity, Photoionization, Radiative Recombination, Rarefied Plasmas, Resonance Lines},
     year = 1993,
    month = sep,
   volume = 88,
    pages = {253-327},
      doi = {10.1086/191823},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJS...88..253S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE T 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{takahashi_mnras_458_2016,
   author = {{Takahashi}, S.~Z. and {Tsukamoto}, Y. and {Inutsuka}, S.},
    title = "{A revised condition for self-gravitational fragmentation of protoplanetary discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1603.01402},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, gravitation, instabilities, planets and satellites: formation, protoplanetary discs},
     year = 2016,
    month = jun,
   volume = 458,
    pages = {3597-3612},
      doi = {10.1093/mnras/stw557},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.458.3597T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tsukamoto_mnras_446_2015,
   author = {{Tsukamoto}, Y. and {Takahashi}, S.~Z. and {Machida}, M.~N. and 
	{Inutsuka}, S.},
    title = "{Effects of radiative transfer on the structure of self-gravitating discs, their fragmentation and the evolution of the fragments}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.7271},
 primaryClass = "astro-ph.SR",
 keywords = {protoplanetary discs, stars: formation, stars: protostars},
     year = 2015,
    month = jan,
   volume = 446,
    pages = {1175-1190},
      doi = {10.1093/mnras/stu2160},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.1175T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tasker_apj_700_2009,
   author = {{Tasker}, E.~J. and {Tan}, J.~C.},
    title = "{Star Formation in Disk Galaxies. I. Formation and Evolution of Giant Molecular Clouds via Gravitational Instability and Cloud Collisions}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0811.0207},
 keywords = {galaxies: ISM, galaxies: spiral, galaxies: star clusters, ISM: clouds, ISM: structure, methods: numerical, stars: formation},
     year = 2009,
    month = jul,
   volume = 700,
    pages = {358-375},
      doi = {10.1088/0004-637X/700/1/358},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...700..358T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tasker_apj_730_2011,
   author = {{Tasker}, E.~J.},
    title = "{Star Formation in Disk Galaxies. II. The Effect Of Star Formation and Photoelectric Heating on the Formation and Evolution of Giant Molecular Clouds}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1101.1534},
 keywords = {galaxies: ISM, galaxies: spiral, galaxies: star clusters: general, ISM: clouds, ISM: structure, methods: numerical, stars: formation},
     year = 2011,
    month = mar,
   volume = 730,
      eid = {11},
    pages = {11},
      doi = {10.1088/0004-637X/730/1/11},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...730...11T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tenoriotagle_aa_145_1985,
   author = {{Tenorio-Tagle}, G. and {Bodenheimer}, P. and {Yorke}, H.~W.
	},
    title = "{Non-spherical supernova remnants. II - The interaction of remnants with molecular clouds}",
  journal = {\aap},
 keywords = {Hydrodynamic Equations, Interstellar Matter, Molecular Clouds, Supernova Remnants, Ionizing Radiation, Morphology, Stellar Winds},
     year = 1985,
    month = apr,
   volume = 145,
    pages = {70-80},
   adsurl = {http://adsabs.harvard.edu/abs/1985A%26A...145...70T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tenoriotagle_aa_148_1985,
   author = {{Tenorio-Tagle}, G. and {Rozyczka}, M. and {Yorke}, H.~W.},
    title = "{The Cygnus loop - A supernova breaking out of a molecular cloud?}",
  journal = {\aap},
 keywords = {Computational Astrophysics, Cygnus Constellation, H Alpha Line, Molecular Clouds, Supernova Remnants, X Ray Sources, Astronomical Models, Density Distribution, Hydrodynamics, Isophotes, Radio Sources (Astronomy)},
     year = 1985,
    month = jul,
   volume = 148,
    pages = {52-58},
   adsurl = {http://adsabs.harvard.edu/abs/1985A%26A...148...52T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tenoriotagle_aa_182_1987,
   author = {{Tenorio-Tagle}, G. and {Bodenheimer}, P. and {Rozyczka}, M.
	},
    title = "{Nonspherical supernova remnants. IV - Sequential explosions in OB associations}",
  journal = {\aap},
 keywords = {B Stars, O Stars, Stellar Models, Stellar Structure, Supernova Remnants, Boundary Value Problems, Hydrodynamic Equations, Stellar Envelopes, Stellar Evolution, Taylor Instability, Two Dimensional Flow},
     year = 1987,
    month = aug,
   volume = 182,
    pages = {120-126},
   adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...182..120T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tenoriotagle_mnras_244_1990,
   author = {{Tenorio-Tagle}, G. and {Bodenheimer}, P. and {Franco}, J. and 
	{Rozyczka}, M.},
    title = "{On the evolution of supernova remnants. I - Explosions inside pre-existing wind-driven bubbles}",
  journal = {\mnras},
 keywords = {Computational Astrophysics, Stellar Evolution, Stellar Mass Ejection, Stellar Winds, Supernova Remnants, Bubbles, Explosions, H Alpha Line, Kinetic Energy, Wind Velocity, X Ray Astronomy},
     year = 1990,
    month = jun,
   volume = 244,
    pages = {563-576},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.244..563T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tenoriotagle_mnras_251_1991,
   author = {{Tenorio-Tagle}, G. and {Rozyczka}, M. and {Franco}, J. and 
	{Bodenheimer}, P.},
    title = "{On the evolution of supernova remnants. II - Two-dimensional calculations of explosions inside pre-existing wind-driven bubbles}",
  journal = {\mnras},
 keywords = {Astronomical Models, Star Distribution, Supernova Remnants, Two Dimensional Models, Interstellar Matter, Stellar Mass Ejection, Stellar Winds, Supernovae, Turbulent Mixing},
     year = 1991,
    month = jul,
   volume = 251,
    pages = {318-329},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.251..318T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{torrelles_mnras_442_2014,
   author = {{Torrelles}, J.~M. and {Curiel}, S. and {Estalella}, R. and 
	{Anglada}, G. and {G{\'o}mez}, J.~F. and {Cant{\'o}}, J. and 
	{Patel}, N.~A. and {Trinidad}, M.~A. and {Girart}, J.~M. and 
	{Carrasco-Gonz{\'a}lez}, C. and {Rodr{\'{\i}}guez}, L.~F.},
    title = "{A very young, compact bipolar H$_{2}$O maser outflow in the intermediate-mass star-forming LkH{$\alpha$} 234 region}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.7273},
 primaryClass = "astro-ph.SR",
 keywords = {masers, stars: formation, ISM: individual objects: LkH{$\alpha$} 234, ISM: jets and outflows},
     year = 2014,
    month = jul,
   volume = 442,
    pages = {148-159},
      doi = {10.1093/mnras/stu847},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.442..148T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{testi_2003,
   author = {{Testi}, L.},
    title = "{Intermediate Mass Stars (Invited Review)}",
booktitle = {Galactic Star Formation Across the Stellar Mass Spectrum},
     year = 2003,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 287,
   editor = {{De Buizer}, J.~M. and {van der Bliek}, N.~S.},
    pages = {163-173},
   adsurl = {http://adsabs.harvard.edu/abs/2003ASPC..287..163T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{toala_apj_737_2011,
   author = {{Toal{\'a}}, J.~A. and {Arthur}, S.~J.},
    title = "{Radiation-hydrodynamic Models of the Evolving Circumstellar Medium around Massive Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.4493},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: bubbles, ISM: kinematics and dynamics, stars: massive, stars: mass-loss, stars: winds, outflows},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {100},
    pages = {100},
      doi = {10.1088/0004-637X/737/2/100},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737..100T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{toomre_apj_138_1963,
   author = {{Toomre}, A.},
    title = "{On the Distribution of Matter Within Highly Flattened Galaxies.}",
  journal = {\apj},
     year = 1963,
    month = aug,
   volume = 138,
    pages = {385},
      doi = {10.1086/147653},
   adsurl = {http://adsabs.harvard.edu/abs/1963ApJ...138..385T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{tomida_apj_801_2015,
   author = {{Tomida}, K. and {Okuzumi}, S. and {Machida}, M.~N.},
    title = "{Radiation Magnetohydrodynamic Simulations of Protostellar Collapse: Nonideal Magnetohydrodynamic Effects and Early Formation of Circumstellar Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1501.04102},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, ISM: jets and outflows, magnetohydrodynamics: MHD, radiative transfer, stars: formation},
     year = 2015,
    month = mar,
   volume = 801,
      eid = {117},
    pages = {117},
      doi = {10.1088/0004-637X/801/2/117},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...801..117T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tomida_apj_714_2010,
   author = {{Tomida}, K. and {Tomisaka}, K. and {Matsumoto}, T. and {Ohsuga}, K. and 
	{Machida}, M.~N. and {Saigo}, K.},
    title = "{Radiation Magnetohydrodynamics Simulation of Proto-stellar Collapse: Two-component Molecular Outflow}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1001.4796},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, magnetohydrodynamics: MHD, radiative transfer, stars: formation},
     year = 2010,
    month = may,
   volume = 714,
    pages = {L58-L63},
      doi = {10.1088/2041-8205/714/1/L58},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714L..58T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tomley_apj_382_1991,
   author = {{Tomley}, L. and {Cassen}, P. and {Steiman-Cameron}, T.},
    title = "{On the evolution of gravitationally unstable protostellar disks}",
  journal = {\apj},
 keywords = {Gravitational Collapse, Many Body Problem, Protostars, Star Formation, Stellar Evolution, Angular Momentum, Astronomical Models, Computational Astrophysics, Interstellar Matter, Stellar Envelopes, T Tauri Stars},
     year = 1991,
    month = dec,
   volume = 382,
    pages = {530-543},
      doi = {10.1086/170740},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...382..530T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tziamtzis_aa_527_2011,
   author = {{Tziamtzis}, A. and {Lundqvist}, P. and {Gr{\"o}ningsson}, P. and 
	{Nasoudi-Shoar}, S.},
    title = "{The outer rings of SN 1987A}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1008.3387},
 primaryClass = "astro-ph.SR",
 keywords = {line: profiles, ISM: supernova remnants, ISM: individual objects: SN 1987A},
     year = 2011,
    month = mar,
   volume = 527,
      eid = {A35},
    pages = {A35},
      doi = {10.1051/0004-6361/201015576},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...527A..35T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tesileanu_aa_488_2008,
   author = {{Te{\c s}ileanu}, O. and {Mignone}, A. and {Massaglia}, S.},
    title = "{Simulating radiative astrophysical flows with the PLUTO code: a non-equilibrium, multi-species cooling function}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0807.3657},
 keywords = {radiation mechanisms: thermal, line: formation, ISM: Herbig-Haro objects, ISM: jets and outflows, methods: numerical, magnetohydrodynamics (MHD)},
     year = 2008,
    month = sep,
   volume = 488,
    pages = {429-440},
      doi = {10.1051/0004-6361:200809461},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...488..429T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{toledo_mnras_442_2014,
   author = {{Toledo-Roy}, J.~C. and {Esquivel}, A. and {Vel{\'a}zquez}, P.~F. and 
	{Reynoso}, E.~M.},
    title = "{A 3D numerical model for Kepler's supernova remnant}",
  journal = {\mnras},
 keywords = {hydrodynamics, radiation mechanisms: thermal, methods: numerical, ISM: supernova remnants, X-rays: ISM},
     year = 2014,
    month = jul,
   volume = 442,
    pages = {229-238},
      doi = {10.1093/mnras/stu880},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.442..229T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{truelove_apj_495_1998,
   author = {{Truelove}, J.~K. and {Klein}, R.~I. and {McKee}, C.~F. and 
	{Holliman}, II, J.~H. and {Howell}, L.~H. and {Greenough}, J.~A. and 
	{Woods}, D.~T.},
    title = "{Self-gravitational Hydrodynamics with Three-dimensional Adaptive Mesh Refinement: Methodology and Applications to Molecular Cloud Collapse and Fragmentation}",
  journal = {\apj},
 keywords = {GRAVITATION, HYDRODYNAMICS, ISM: CLOUDS, METHODS: NUMERICAL, STARS: FORMATION, Gravitation, Hydrodynamics, ISM: Clouds, Methods: Numerical, Stars: Formation},
     year = 1998,
    month = mar,
   volume = 495,
    pages = {821-852},
      doi = {10.1086/305329},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...495..821T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{truelove_apjs_120_1999,
   author = {{Truelove}, J.~K. and {McKee}, C.~F.},
    title = "{Evolution of Nonradiative Supernova Remnants}",
  journal = {\apjs},
 keywords = {HYDRODYNAMICS, SHOCK WAVES, ISM: SUPERNOVA REMNANTS, STARS: SUPERNOVAE: GENERAL},
     year = 1999,
    month = feb,
   volume = 120,
    pages = {299-326},
      doi = {10.1086/313176},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJS..120..299T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{tsukamoto_mnras_446_2015,
   author = {{Tsukamoto}, Y. and {Takahashi}, S.~Z. and {Machida}, M.~N. and 
	{Inutsuka}, S.},
    title = "{Effects of radiative transfer on the structure of self-gravitating discs, their fragmentation and the evolution of the fragments}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.7271},
 primaryClass = "astro-ph.SR",
 keywords = {protoplanetary discs, stars: formation, stars: protostars},
     year = 2015,
    month = jan,
   volume = 446,
    pages = {1175-1190},
      doi = {10.1093/mnras/stu2160},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.1175T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE U 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{uchida_pasj_61_2009,
   author = {{Uchida}, H. and {Tsunemi}, H. and {Katsuda}, S. and {Kimura}, M. and 
	{Kosugi}, H.},
    title = "{Ejecta Distributions of Heavy Elements in the Cygnus Loop}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {0901.3433},
 keywords = {ISM: abundances, ISM: individual (Cygnus Loop), ISM: supernova remnants, X-rays: ISM},
     year = 2009,
    month = feb,
   volume = 61,
    pages = {301-},
      doi = {10.1093/pasj/61.2.301},
   adsurl = {http://adsabs.harvard.edu/abs/2009PASJ...61..301U},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE V 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@INPROCEEDINGS{vanburen_aspc_35_1993,
   author = {{van Buren}, D.},
    title = "{Stellar Wind Bow Shocks}",
booktitle = {Massive Stars:  Their Lives in the Interstellar Medium},
     year = 1993,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 35,
   editor = {{Cassinelli}, J.~P. and {Churchwell}, E.~B.},
    month = jan,
    pages = {315},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1993ASPC...35..315V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanburen_apj_329_1988,
   author = {{van Buren}, D. and {McCray}, R.},
    title = "{Bow shocks and bubbles are seen around hot stars by IRAS}",
  journal = {\apjl},
 keywords = {Bow Waves, Early Stars, Hot Stars, Infrared Stars, Interstellar Matter, Plasma Bubbles, Stellar Winds, Cosmic Dust, H Ii Regions, Infrared Astronomy Satellite, Radiation Pressure, Stellar Luminosity},
     year = 1988,
    month = jun,
   volume = 329,
    pages = {L93-L96},
      doi = {10.1086/185184},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...329L..93V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanbeveren_ssrv_56_1991,
   author = {{Vanbeveren}, D.},
    title = "{Massive close binaries - Observations and evolutionary computations}",
  journal = {\ssr},
 keywords = {Binary Stars, Stellar Mass, Stellar Mass Accretion, Stellar Mass Ejection, Stellar Winds, Supernovae, Stellar Evolution, Wolf-Rayet Stars, X Ray Binaries},
     year = 1991,
    month = may,
   volume = 56,
    pages = {249-311},
      doi = {10.1007/BF00196630},
   adsurl = {http://adsabs.harvard.edu/abs/1991SSRv...56..249V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vandishoeck_aa_279_1993,
   author = {{van Dishoeck}, E.~F. and {Jansen}, D.~J. and {Phillips}, T.~G.
	},
    title = "{Submillimeter observations of the shocked molecular gas associated with the supernova remnant IC 443}",
  journal = {\aap},
 keywords = {Astronomical Models, Interstellar Gas, Molecular Gases, Molecular Spectra, Radio Astronomy, Shock Wave Interaction, Submillimeter Waves, Supernova Remnants, Abundance, Astronomical Spectroscopy, Hydrodynamics, Line Spectra, Mathematical Models, Radio Spectra},
     year = 1993,
    month = nov,
   volume = 279,
    pages = {541-566},
   adsurl = {http://adsabs.harvard.edu/abs/1993A%26A...279..541V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanallen_apj_71_2003,
   author = {{van Allen}, J.~A.},
    title = "{Gravitational assist in celestial mechanics-a tutorial}",
  journal = {American Journal of Physics},
 keywords = {Educational aids, Relativity and gravitation, Celestial mechanics, Celestial mechanics, Surveys and tutorial papers; resource letters, Spaceborne and space research instruments, apparatus, and components, Lunar, planetary, and deep-space probes, Experimental tests of gravitational theories},
     year = 2003,
    month = may,
   volume = 71,
    pages = {448-451},
      doi = {10.1119/1.1539102},
   adsurl = {http://adsabs.harvard.edu/abs/2003AmJPh..71..448V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{vanmarle_revmexaa_22_2004,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{Wind-Blown Bubbles around Massive Stars. The effects of stellar wind and photo-ionization on the circumstellar Medium}",
 keywords = {H II regions, stars: Circumstellar matter, Stars: mass loss, Stars: winds, outflows},
booktitle = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
     year = 2004,
   series = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
   volume = 22,
   editor = "{G.~Garcia-Segura, G.~Tenorio-Tagle, J.~Franco, \& H.~W.~Yorke
	}",
    month = dec,
    pages = {136-139},
   adsurl = {http://adsabs.harvard.edu/abs/2004RMxAC..22..136V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@PHDTHESIS{vanmarle_phd_2006,
   author = {{van Marle}, A.~J.},
    title = "{Models for the circumstellar medium of long gamma-ray burst progenitor candidates}",
 keywords = {afterglow, gamma-ray burst, circumstellar medium, stellar wind, hydrodynamics},
   school = {Utrecht University},
     year = 2006,
    month = May,
   adsurl = {http://adsabs.harvard.edu/abs/2006PhDT........80V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_apj_734_2011,
   author = {{van Marle}, A.~J. and {Meliani}, Z. and {Keppens}, R. and {Decin}, L.
	},
    title = "{Computing the Dust Distribution in the Bow Shock of a Fast-moving, Evolved Star}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1105.2387},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, infrared: ISM, ISM: abundances, ISM: kinematics and dynamics, stars: winds, outflows},
     year = 2011,
    month = jun,
   volume = 734,
      eid = {L26},
    pages = {L26},
      doi = {10.1088/2041-8205/734/2/L26},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...734L..26V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_444_2005,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{Constraints on gamma-ray burst and supernova progenitors through circumstellar absorption lines}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0507659},
 keywords = {, stars: winds, outflows, stars: Wolf-Rayet, stars: supernovae: general, gamma rays: bursts, line: profiles, ISM: bubbles},
     year = 2005,
    month = dec,
   volume = 444,
    pages = {837-847},
      doi = {10.1051/0004-6361:20053520},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...444..837V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_469_2007,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{Constraints on gamma-ray burst and supernova progenitors through circumstellar absorption lines. II. Post-LBV Wolf-Rayet stars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.2073},
 keywords = {stars: winds, outflows, stars: Wolf-Rayet, stars: supernovae: general, gamma rays: bursts, line: profiles, ISM: bubbles},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {941-948},
      doi = {10.1051/0004-6361:20077207},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..941V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_460_2006,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Achterberg}, A. and 
	{Garc{\'{\i}}a-Segura}, G.},
    title = "{Forming a constant density medium close to long gamma-ray bursts}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0605698},
 keywords = {stars: Wolf-Rayet, stars: winds, outflows, gamma rays: bursts, ISM: bubbles, hydrodynamics},
     year = 2006,
    month = dec,
   volume = 460,
    pages = {105-116},
      doi = {10.1051/0004-6361:20065709},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...460..105V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_mnras_407_2010,
   author = {{van Marle}, A.~J. and {Smith}, N. and {Owocki}, S.~P. and {van Veelen}, B.
	},
    title = "{Numerical models of collisions between core-collapse supernovae and circumstellar shells}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1004.2791},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, methods: numerical, stars: mass-loss, supernovae: general, stars: winds, outflows, ISM: supernova remnants},
     year = 2010,
    month = oct,
   volume = 407,
    pages = {2305-2327},
      doi = {10.1111/j.1365-2966.2010.16851.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407.2305V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_537_2012,
   author = {{Cox}, N.~L.~J. and {Kerschbaum}, F. and {van Marle}, A.-J. and 
	{Decin}, L. and {Ladjal}, D. and {Mayer}, A.},
    title = "{A far-infrared survey of bow shocks and detached shells around AGB stars and red supergiants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.5486},
 primaryClass = "astro-ph.GA",
 keywords = {stars: AGB and post-AGB, circumstellar matter, infrared: ISM, hydrodynamics, stars: mass-loss, stars: winds, outflows},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A35},
    pages = {A35},
      doi = {10.1051/0004-6361/201117910},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A..35C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_527_2011,
   author = {{van Marle}, A.~J. and {Keppens}, R. and {Meliani}, Z.},
    title = "{Thin shell morphology in the circumstellar medium of massive binaries}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1011.1734},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, binaries: general, circumstellar matter, stars: massive, stars: winds, outflows},
     year = 2011,
    month = mar,
   volume = 527,
      eid = {A3},
    pages = {A3},
      doi = {10.1051/0004-6361/201015517},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...527A...3V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{vanmarle_asp_355_2006,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{The Impact of a Luminous Blue Variable on its Circumstellar Medium}",
booktitle = {Stars with the B[e] Phenomenon},
     year = 2006,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 355,
   editor = "{M.~Kraus \& A.~S.~Miroshnichenko}",
    month = dec,
    pages = {203},
   adsurl = {http://adsabs.harvard.edu/abs/2006ASPC..355..203V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_comp&fluids_2010pdf,
   author = {{van Marle}, A.~J. and {Keppens}, R.},
    title = "{Radiative cooling in numerical astrophysics: the need for adaptive mesh refinement}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1011.2610},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2010,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1011.2610V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_561_2014,
   author = {{van Marle}, A.~J. and {Decin}, L. and {Meliani}, Z.},
    title = "{Can the magnetic field in the Orion arm inhibit the growth of instabilities in the bow shock of Betelgeuse?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1312.5877},
 primaryClass = "astro-ph.SR",
 keywords = {magnetohydrodynamics (MHD), instabilities, circumstellar matter, stars: individual: alpha Orionis, ISM: bubbles, ISM: magnetic fields},
     year = 2014,
    month = jan,
   volume = 561,
      eid = {A152},
    pages = {A152},
      doi = {10.1051/0004-6361/201321968},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...561A.152V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_bull_srs_liege_80_2011,
   author = {{van Marle}, A.~J. and {Keppens}, R. and {Meliani}, Z.},
    title = "{3-D simulations of shells around massive stars}",
  journal = {Bulletin de la Societe Royale des Sciences de Liege},
archivePrefix = "arXiv",
   eprint = {1102.0104},
 primaryClass = "astro-ph.SR",
     year = 2011,
    month = jan,
   volume = 80,
    pages = {310-315},
   adsurl = {http://adsabs.harvard.edu/abs/2011BSRSL..80..310V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_apjl_734_2011,
   author = {{van Marle}, A.~J. and {Meliani}, Z. and {Keppens}, R. and {Decin}, L.
	},
    title = "{Computing the Dust Distribution in the Bow Shock of a Fast-moving, Evolved Star}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1105.2387},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, infrared: ISM, ISM: abundances, ISM: kinematics and dynamics, stars: winds, outflows},
     year = 2011,
    month = jun,
   volume = 734,
      eid = {L26},
    pages = {L26},
      doi = {10.1088/2041-8205/734/2/L26},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...734L..26V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanmarle_aa_478_2008,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Yoon}, S.-C. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{The circumstellar medium around a rapidly rotating, chemically homogeneously evolving, possible gamma-ray burst progenitor}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0711.4807},
 keywords = {gamma-rays: bursts, hydrodynamics, ISM: bubbles, stars: winds, outflows, stars: Wolf-Rayet},
     year = 2008,
    month = feb,
   volume = 478,
    pages = {769-778},
      doi = {10.1051/0004-6361:20078802},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...478..769V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@PhDThesis{ vanveelen_phd,
	title = "Supernovae interacting with their circumstellar medium",
	author = "van Veelen, B.",
	school = "Utrecht University",
	year = "2010",
	address = "Netherland"
}

@ARTICLE{vanveelen_aa_50._2009,
   author = {{van Veelen}, B. and {Langer}, N. and {Vink}, J. and {Garc{\'{\i}}a-Segura}, G. and 
	{van Marle}, A.~J.},
    title = "{The hydrodynamics of the supernova remnant Cassiopeia A. The influence of the progenitor evolution on the velocity structure and clumping}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.1197},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, stars: winds, outflows, stars: supernovae: general, stars: supernovae: individual: Cas A},
     year = 2009,
    month = aug,
   volume = 503,
    pages = {495-503},
      doi = {10.1051/0004-6361/200912393},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...503..495V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vaidya_apj_742_2011,
   author = {{Vaidya}, B. and {Fendt}, C. and {Beuther}, H. and {Porth}, O.
	},
    title = "{Jet Formation from Massive Young Stars: Magnetohydrodynamics versus Radiation Pressure}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1108.4924},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, ISM: jets and outflows, magnetohydrodynamics: MHD, methods: numerical, radiative transfer, stars: formation, stars: massive},
     year = 2011,
    month = nov,
   volume = 742,
      eid = {56},
    pages = {56},
      doi = {10.1088/0004-637X/742/1/56},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742...56V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ARA&A..45..565M,
   author = {{McKee}, C.~F. and {Ostriker}, E.~C.},
    title = "{Theory of Star Formation}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0707.3514},
     year = 2007,
    month = sep,
   volume = 45,
    pages = {565-687},
      doi = {10.1146/annurev.astro.45.051806.110602},
   adsurl = {http://adsabs.harvard.edu/abs/2007ARA%26A..45..565M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vazquez_apj_630_2005,
   author = {{V{\'a}zquez-Semadeni}, E. and {Kim}, J. and {Ballesteros-Paredes}, J.
	},
    title = "{Star Formation Efficiency in Driven, Supercritical, Turbulent Clouds}",
  journal = {\apjl},
   eprint = {astro-ph/0507637},
 keywords = {ISM: Clouds, Magnetohydrodynamics: MHD, Stars: Formation, Turbulence},
     year = 2005,
    month = sep,
   volume = 630,
    pages = {L49-L52},
      doi = {10.1086/491650},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...630L..49V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{velazquez_apj_601_2004,
   author = {{Vel{\'a}zquez}, P.~F. and {Martinell}, J.~J. and {Raga}, A.~C. and 
	{Giacani}, E.~B.},
    title = "{Effects of Thermal Conduction on the X-Ray and Synchrotron Emission from Supernova Remnants}",
  journal = {\apj},
 keywords = {Conduction, ISM: Magnetic Fields, Methods: Numerical, ISM: Supernova Remnants, X-Rays: ISM},
     year = 2004,
    month = feb,
   volume = 601,
    pages = {885-895},
      doi = {10.1086/380755},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...601..885V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{velazquez_apj_649_2006,
   author = {{Vel{\'a}zquez}, P.~F. and {Vigh}, C.~D. and {Reynoso}, E.~M. and 
	{G{\'o}mez}, D.~O. and {Schneiter}, E.~M.},
    title = "{Simulated X-Ray Emission for a Runaway Model of Kepler's Supernova Remnant}",
  journal = {\apj},
 keywords = {Hydrodynamics, ISM: individual (Kepler SNR), Methods: Numerical, Shock Waves, ISM: Supernova Remnants, X-Rays: ISM},
     year = 2006,
    month = oct,
   volume = 649,
    pages = {779-787},
      doi = {10.1086/506899},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...649..779V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{velusamy,
   author = {{Velusamy}, T.},
    title = "{Guest Stars - Historical Supernovae and Remnants}",
booktitle = {IAU Colloq. 91: History of Oriental Astronomy},
     year = 1987,
   editor = {{Swarup}, G. and {Bag}, A.~K. and {Shukla}, K.~S.},
    pages = {265},
   adsurl = {http://adsabs.harvard.edu/abs/1987hooa.coll..265V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vollmer_aa_491_2008,
   author = {{Vollmer}, B. and {Beckert}, T. and {Davies}, R.~I.},
    title = "{Starbursts and torus evolution in AGN}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0809.3397},
 keywords = {galaxies: active, galaxies: nuclei, ISM: clouds, ISM: structure, ISM: kinematics and dynamics},
     year = 2008,
    month = nov,
   volume = 491,
    pages = {441-453},
      doi = {10.1051/0004-6361:200810446},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...491..441V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vieser_472_aa_2007,
   author = {{Vieser}, W. and {Hensler}, G.},
    title = "{The evolution of interstellar clouds in a streaming hot plasma including heat conduction}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.3592},
 keywords = {ISM: clouds, conduction, hydrodynamics, instabilities},
     year = 2007,
    month = sep,
   volume = 472,
    pages = {141-153},
      doi = {10.1051/0004-6361:20042120},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...472..141V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vigh_apj_727_2011,
   author = {{Vigh}, C.~D. and {Vel{\'a}zquez}, P.~F. and {G{\'o}mez}, D.~O. and 
	{Reynoso}, E.~M. and {Esquivel}, A. and {Matias Schneiter}, E.
	},
    title = "{Asymmetries in the Expansion and Emission from Young Supernova Remnants}",
  journal = {\apj},
 keywords = {hydrodynamics, ISM: supernova remnants, methods: numerical, shock waves, supernovae: individual: Tycho},
     year = 2011,
    month = jan,
   volume = 727,
      eid = {32},
    pages = {32},
      doi = {10.1088/0004-637X/727/1/32},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...727...32V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{villaver_apj_748_2012,
   author = {{Villaver}, E. and {Manchado}, A. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{The Interaction of Asymptotic Giant Branch Stars with the Interstellar Medium}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1201.3378},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, ISM: kinematics and dynamics, ISM: structure, stars: AGB and post-AGB, stars: winds, outflows},
     year = 2012,
    month = apr,
   volume = 748,
      eid = {94},
    pages = {94},
      doi = {10.1088/0004-637X/748/2/94},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748...94V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{vink_asp_353_2006,
   author = {{Vink}, J.~S.},
    title = "{Massive star feedback -- from the first stars to the present}",
booktitle = {Stellar Evolution at Low Metallicity: Mass Loss, Explosions, Cosmology},
     year = 2006,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 353,
   eprint = {astro-ph/0511048},
   editor = {{Lamers}, H.~J.~G.~L.~M. and {Langer}, N. and {Nugis}, T. and 
	{Annuk}, K.},
    month = dec,
    pages = {113},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006ASPC..353..113V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vink_aa_362_2000,
   author = {{Vink}, J.~S. and {de Koter}, A. and {Lamers}, H.~J.~G.~L.~M.
	},
    title = "{New theoretical mass-loss rates of O and B stars}",
  journal = {\aap},
   eprint = {astro-ph/0008183},
 keywords = {STARS: EARLY-TYPE, STARS: MASS-LOSS, STARS: SUPERGIANTS, STARS: WINDS, OUTFLOWS, STARS: EVOLUTION},
     year = 2000,
    month = oct,
   volume = 362,
    pages = {295-309},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...362..295V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vink_aa_369_2001,
   author = {{Vink}, J.~S. and {de Koter}, A. and {Lamers}, H.~J.~G.~L.~M.
	},
    title = "{Mass-loss predictions for O and B stars as a function of metallicity}",
  journal = {\aap},
   eprint = {astro-ph/0101509},
 keywords = {STARS: EARLY-TYPE, STARS: MASS-LOSS, STARS: SUPERGIANTS, STARS: WINDS, STARS: EVOLUTION},
     year = 2001,
    month = apr,
   volume = 369,
    pages = {574-588},
      doi = {10.1051/0004-6361:20010127},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...369..574V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vink_aa_307_1996,
   author = {{Vink}, J. and {Kaastra}, J.~S. and {Bleeker}, J.~A.~M.},
    title = "{A new mass estimate and puzzling abundances of SNR Cassiopeia A.}",
  journal = {\aap},
 keywords = {ISM: ABUNDANCES, ISM: INDIVIDUAL OBJECTS: CAS A, ISM: SUPERNOVA REMNANTS, X-RAYS: ISM},
     year = 1996,
    month = mar,
   volume = 307,
    pages = {L41-L44},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...307L..41V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vink_aa_328_1997,
   author = {{Vink}, J. and {Kaastra}, J.~S. and {Bleeker}, J.~A.~M.},
    title = "{X-ray spectroscopy of the supernova remnant RCW 86. A new challenge for modeling the emission from supernova remnants}",
  journal = {\aap},
 keywords = {ATOMIC PROCESSES, ISM: ABUNDANCES, ISM: INDIVIDUAL OBJECTS: RCW 86, ISM: SUPERNOVA REMNANTS, X-RAYS: ISM},
     year = 1997,
    month = dec,
   volume = 328,
    pages = {628-633},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...328..628V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{broersen_mnras_441_2014,
   author = {{Broersen}, S. and {Chiotellis}, A. and {Vink}, J. and {Bamba}, A.
	},
    title = "{The many sides of RCW 86: a Type Ia supernova remnant evolving in its progenitor's wind bubble}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.5434},
 primaryClass = "astro-ph.HE",
 keywords = {supernovae: general, supernovae: individual: RCW 86, ISM: supernova remnants},
     year = 2014,
    month = jul,
   volume = 441,
    pages = {3040-3054},
      doi = {10.1093/mnras/stu667},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441.3040B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vink_aarv_20_2012,
   author = {{Vink}, J.},
    title = "{Supernova remnants: the X-ray perspective}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {1112.0576},
 primaryClass = "astro-ph.HE",
 keywords = {Supernova remnants, Supernovae, X-ray, Cosmic rays},
     year = 2012,
    month = dec,
   volume = 20,
    pages = {49},
      doi = {10.1007/s00159-011-0049-1},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26ARv..20...49V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vishniac_apj_428_1994,
   author = {{Vishniac}, E.~T.},
    title = "{Nonlinear instabilities in shock-bounded slabs}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9306025},
 keywords = {COSMOLOGY, HYDRODYNAMICS, INTERSTELLAR GAS, NONLINEARITY, NORMAL SHOCK WAVES, SLABS, STABILITY, ASTRONOMICAL MODELS, DIMENSIONAL ANALYSIS, GALACTIC EVOLUTION, STELLAR EVOLUTION, VORTICITY},
     year = 1994,
    month = jun,
   volume = 428,
    pages = {186-208},
      doi = {10.1086/174231},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...428..186V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_aa_552_2013,
   author = {{Vorobyov}, E.~I.},
    title = "{Formation of giant planets and brown dwarfs on wide orbits}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1302.1892},
 primaryClass = "astro-ph.EP",
 keywords = {protoplanetary disks, planets and satellites: formation, stars: formation, hydrodynamics, stars: protostars},
     year = 2013,
    month = apr,
   volume = 552,
      eid = {A129},
    pages = {A129},
      doi = {10.1051/0004-6361/201220601},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...552A.129V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_apj_723_2010,
   author = {{Vorobyov}, E.~I.},
    title = "{Embedded Protostellar Disks Around (Sub-)Solar Protostars. I. Disk Structure and Evolution}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1009.2073},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, hydrodynamics, ISM: clouds, protoplanetary disks, stars: formation},
     year = 2010,
    month = nov,
   volume = 723,
    pages = {1294-1307},
      doi = {10.1088/0004-637X/723/2/1294},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...723.1294V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{voroboyov_aa_557_2013,
   author = {{Vorobyov}, E.~I. and {Baraffe}, I. and {Harries}, T. and {Chabrier}, G.
	},
    title = "{The effect of episodic accretion on the phase transition of CO and CO$_{2}$ in low-mass star formation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1307.2271},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: low-mass, accretion, accretion disks, protoplanetary disks},
     year = 2013,
    month = sep,
   volume = 557,
      eid = {A35},
    pages = {A35},
      doi = {10.1051/0004-6361/201321775},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...557A..35V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{regaly_aa_601_2017,
   author = {{Reg{\'a}ly}, Z. and {Vorobyov}, E.},
    title = "{The circumstellar disk response to the motion of the host star}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1701.04751},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, stars: formation, stars: protostars, planet-disk interactions, protoplanetary disks, methods: numerical},
     year = 2017,
    month = may,
   volume = 601,
      eid = {A24},
    pages = {A24},
      doi = {10.1051/0004-6361/201629154},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017A%26A...601A..24R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_mnras_381_2007,
   author = {{Vorobyov}, E.~I. and {Basu}, S.},
    title = "{Self-regulated gravitational accretion in protostellar discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0709.2043},
 keywords = {accretion, accretion discs, hydrodynamics, instabilities, ISM: clouds, stars: formation},
     year = 2007,
    month = nov,
   volume = 381,
    pages = {1009-1017},
      doi = {10.1111/j.1365-2966.2007.12321.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.381.1009V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_apj_728_2011,
   author = {{Vorobyov}, E.~I.},
    title = "{Destruction of Massive Fragments in Protostellar Disks and Crystalline Silicate Production}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1101.3982},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, hydrodynamics, stars: formation, stars: protostars},
     year = 2011,
    month = feb,
   volume = 728,
      eid = {L45},
    pages = {L45},
      doi = {10.1088/2041-8205/728/2/L45},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...728L..45V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_mnras_433_2013,
   author = {{Vorobyov}, E.~I. and {Zakhozhay}, O.~V. and {Dunham}, M.~M.
	},
    title = "{Fragmenting protostellar discs: properties and observational signatures}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1306.4074},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, hydrodynamics, instabilities, stars: formation},
     year = 2013,
    month = aug,
   volume = 433,
    pages = {3256-3273},
      doi = {10.1093/mnras/stt970},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.3256V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vorobyov_apj_805_2015,
   author = {{Vorobyov}, E.~I. and {Basu}, S.},
    title = "{Variable Protostellar Accretion with Episodic Bursts}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1503.07888},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, ISM: clouds, stars: formation},
     year = 2015,
    month = jun,
   volume = 805,
      eid = {115},
    pages = {115},
      doi = {10.1088/0004-637X/805/2/115},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...805..115V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE W 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{WareingZijlstraOBrien_2007_MNRAS_382_1233_AGB_bowshocks,
   author = {{Wareing}, C.~J. and {Zijlstra}, A.~A. and {O'Brien}, T.~J.},
    title = "{The interaction of planetary nebulae and their asymptotic giant branch progenitors with the interstellar medium}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0709.2848},
 keywords = {hydrodynamics, stars: AGB and post-AGB, stars: mass-loss, planetary nebulae: general, ISM: structure},
     year = 2007,
    month = dec,
   volume = 382,
    pages = {1233-1245},
      doi = {10.1111/j.1365-2966.2007.12459.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382.1233W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wareing_apj_660_2007,
   author = {{Wareing}, C.~J. and {Zijlstra}, A.~A. and {O'Brien}, T.~J.},
    title = "{Vortices in the Wakes of Asymptotic Giant Branch Stars}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0703732},
 keywords = {Stars: Circumstellar Matter, Hydrodynamics, ISM: Structure, Stars: AGB and Post-AGB, Stars: Mass Loss, Turbulence},
     year = 2007,
    month = may,
   volume = 660,
    pages = {L129-L132},
      doi = {10.1086/518308},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660L.129W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wang_MNRAS_261_1993,
   author = {{Wang}, L. and {Dyson}, J.~E. and {Kahn}, F.~D.},
    title = "{The nature of the Napoleon's Hat nebula of SN 1987A}",
  journal = {\mnras},
 keywords = {NEBULAE, STELLAR ENVELOPES, STELLAR EVOLUTION, STELLAR MASS EJECTION, SUPERNOVA 1987A, BUBBLES, INTERSTELLAR MATTER, STELLAR MODELS, STELLAR WINDS},
     year = 1993,
    month = mar,
   volume = 261,
    pages = {391-395},
   adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.261..391W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wang_nature_1992,
   author = {{Wang}, L. and {Mazzali}, P.~A.},
    title = "{Dynamical development of a ring-like structure in the supernova 1987A nebula}",
  journal = {\nat},
 keywords = {STELLAR EVOLUTION, STELLAR STRUCTURE, STELLAR WINDS, SUPERNOVA REMNANTS, SUPERNOVA 1987A, BLUE STARS, PLANETARY NEBULAE, STELLAR MODELS, STELLAR ROTATION, WOLF-RAYET STARS},
     year = 1992,
    month = jan,
   volume = 355,
    pages = {58-61},
      doi = {10.1038/355058a0},
   adsurl = {http://adsabs.harvard.edu/abs/1992Natur.355...58W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wampler_apj_362_1990,
   author = {{Wampler}, E.~J. and {Wang}, L. and {Baade}, D. and {Banse}, K. and 
	{D'Odorico}, S. and {Gouiffes}, C. and {Tarenghi}, M.},
    title = "{Observations of the nebulosities near SN 1987A}",
  journal = {\apjl},
 keywords = {Astronomical Spectroscopy, Cosmic Dust, Interstellar Gas, Nebulae, Supernovae, Astronomical Observatories, Charge Coupled Devices, Galactic Evolution, Pixels, Stellar Luminosity, Ultraviolet Spectra},
     year = 1990,
    month = oct,
   volume = 362,
    pages = {L13-L16},
      doi = {10.1086/185836},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...362L..13W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wolfire_apj_587_2003,
   author = {{Wolfire}, M.~G. and {McKee}, C.~F. and {Hollenbach}, D. and 
	{Tielens}, A.~G.~G.~M.},
    title = "{Neutral Atomic Phases of the Interstellar Medium in the Galaxy}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0207098},
 keywords = {ISM: Clouds, ISM: General, ISM: Structure},
     year = 2003,
    month = apr,
   volume = 587,
    pages = {278-311},
      doi = {10.1086/368016},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...587..278W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{williams_apj_741_2011,
   author = {{Williams}, B.~J. and {Blair}, W.~P. and {Blondin}, J.~M. and 
	{Borkowski}, K.~J. and {Ghavamian}, P. and {Long}, K.~S. and 
	{Raymond}, J.~C. and {Reynolds}, S.~P. and {Rho}, J. and {Winkler}, P.~F.
	},
    title = "{RCW 86: A Type Ia Supernova in a Wind-blown Bubble}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1108.1207},
 primaryClass = "astro-ph.GA",
 keywords = {cosmic rays, dust, extinction, ISM: supernova remnants},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {96},
    pages = {96},
      doi = {10.1088/0004-637X/741/2/96},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741...96W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wit_aa_425_2004,
   author = {{de Wit}, W.~J. and {Testi}, L. and {Palla}, F. and {Vanzi}, L. and 
	{Zinnecker}, H.},
    title = "{The origin of massive O-type field stars.  I. A search for clusters}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0405348},
 keywords = {stars: early-type, stars: formation},
     year = 2004,
    month = oct,
   volume = 425,
    pages = {937-948},
      doi = {10.1051/0004-6361:20040454},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...425..937D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wit_aa_437_2005,
   author = {{de Wit}, W.~J. and {Testi}, L. and {Palla}, F. and {Zinnecker}, H.
	},
    title = "{The origin of massive O-type field stars: II. Field O stars as runaways}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0503337},
 keywords = {stars: early-type, stars: formation, Galaxy: stellar content, stars: kinematics},
     year = 2005,
    month = jul,
   volume = 437,
    pages = {247-255},
      doi = {10.1051/0004-6361:20042489},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437..247D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{whalen_apj_682_2008,
   author = {{Whalen}, D. and {van Veelen}, B. and {O'Shea}, B.~W. and {Norman}, M.~L.
	},
    title = "{The Destruction of Cosmological Minihalos by Primordial Supernovae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.3698},
 keywords = {Cosmology: Theory, Cosmology: Early Universe, Hydrodynamics, Stars: Early-Type, Stars: Supernovae: Individual},
     year = 2008,
    month = jul,
   volume = 682,
    pages = {49-67},
      doi = {10.1086/589643},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...682...49W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{whiteoak_aas_118_1996,
   author = {{Whiteoak}, J.~B.~Z. and {Green}, A.~J.},
    title = "{The MOST supernova remnant catalogue (MSC).}",
  journal = {\aaps},
 keywords = {ISM: SUPERNOVA REMNANTS, RADIO CONTINUUM: ISM, ATLASES, CATALOGUES, SURVEYS},
     year = 1996,
    month = aug,
   volume = 118,
    pages = {329-380},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..118..329W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{weaver_apj_218_1977,
   author = {{Weaver}, R. and {McCray}, R. and {Castor}, J. and {Shapiro}, P. and 
	{Moore}, R.},
    title = "{Interstellar bubbles. II - Structure and evolution}",
  journal = {\apj},
 keywords = {INTERSTELLAR GAS, PLASMA INTERACTIONS, STELLAR WINDS, ADIABATIC FLOW, BUBBLES, CONDUCTIVE HEAT TRANSFER, EARLY STARS, ENERGY DISSIPATION, HYDRODYNAMICS, ION DENSITY (CONCENTRATION), RADIATIVE TRANSFER, STELLAR MOTIONS},
     year = 1977,
    month = dec,
   volume = 218,
    pages = {377-395},
      doi = {10.1086/155692},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...218..377W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{weaver_errata_1978,
   author = {{Weaver}, R. and {McCray}, R. and {Castor}, J. and {Shapiro}, P. and 
	{Moore}, R.},
    title = "{Errata: Interstellar Bubbles. II. Structure and Evolution}",
  journal = {\apj},
     year = 1978,
    month = mar,
   volume = 220,
    pages = {742},
      doi = {10.1086/155960},
   adsurl = {http://adsabs.harvard.edu/abs/1978ApJ...220..742W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wilkin_459_apj_1996,
   author = {{Wilkin}, F.~P.},
    title = "{Exact Analytic Solutions for Stellar Wind Bow Shocks}",
  journal = {\apjl},
 keywords = {STARS: MASS LOSS, HYDRODYNAMICS, SHOCK WAVES, ISM: BUBBLES},
     year = 1996,
    month = mar,
   volume = 459,
    pages = {L31},
      doi = {10.1086/309939},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...459L..31W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{williams_apj_770_2013,
   author = {{Williams}, B.~J. and {Borkowski}, K.~J. and {Ghavamian}, P. and 
	{Hewitt}, J.~W. and {Mao}, S.~A. and {Petre}, R. and {Reynolds}, S.~P. and 
	{Blondin}, J.~M.},
    title = "{Azimuthal Density Variations around the Rim of Tycho's Supernova Remnant}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.0567},
 primaryClass = "astro-ph.HE",
 keywords = {dust, extinction, ISM: supernova remnants},
     year = 2013,
    month = jun,
   volume = 770,
      eid = {129},
    pages = {129},
      doi = {10.1088/0004-637X/770/2/129},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770..129W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wiersma_mnras_393_2009,
   author = {{Wiersma}, R.~P.~C. and {Schaye}, J. and {Smith}, B.~D.},
    title = "{The effect of photoionization on the cooling rates of enriched, astrophysical plasmas}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0807.3748},
 keywords = {atomic processes , plasmas , cooling flows , galaxies: formation , intergalactic medium},
     year = 2009,
    month = feb,
   volume = 393,
    pages = {99-107},
      doi = {10.1111/j.1365-2966.2008.14191.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.393...99W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wit_aa_437_2005,
   author = {{de Wit}, W.~J. and {Testi}, L. and {Palla}, F. and {Zinnecker}, H.
	},
    title = "{The origin of massive O-type field stars: II. Field O stars as runaways}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0503337},
 keywords = {stars: early-type, stars: formation, Galaxy: stellar content, stars: kinematics},
     year = 2005,
    month = jul,
   volume = 437,
    pages = {247-255},
      doi = {10.1051/0004-6361:20042489},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437..247D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{woosley_rvmp_74_2002,
   author = {{Woosley}, S.~E. and {Heger}, A. and {Weaver}, T.~A.},
    title = "{The evolution and explosion of massive stars}",
  journal = {Reviews of Modern Physics},
 keywords = {Nucleosynthesis in novae supernovae and other explosive environments, Supernovae, Hydrostatic stellar nucleosynthesis, Elementary particle processes, Stellar structure interiors evolution nucleosynthesis ages, Neutron stars, Relativity and gravitation},
     year = 2002,
    month = nov,
   volume = 74,
    pages = {1015-1071},
      doi = {10.1103/RevModPhys.74.1015},
   adsurl = {http://adsabs.harvard.edu/abs/2002RvMP...74.1015W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{whiteoak_aas_118_1996,
   author = {{Whiteoak}, J.~B.~Z. and {Green}, A.~J.},
    title = "{The MOST supernova remnant catalogue (MSC).}",
  journal = {\aaps},
 keywords = {ISM: SUPERNOVA REMNANTS, RADIO CONTINUUM: ISM, ATLASES, CATALOGUES, SURVEYS},
     year = 1996,
    month = aug,
   volume = 118,
    pages = {329-380},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..118..329W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{wurster_mnras_457_2016,
   author = {{Wurster}, J. and {Price}, D.~J. and {Bate}, M.~R.},
    title = "{Can non-ideal magnetohydrodynamics solve the magnetic braking catastrophe?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1512.01597},
 primaryClass = "astro-ph.SR",
 keywords = {magnetic fields, MHD, methods: numerical, stars: formation},
     year = 2016,
    month = mar,
   volume = 457,
    pages = {1037-1061},
      doi = {10.1093/mnras/stw013},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.457.1037W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wright_aj_140_2010,
   author = {{Wright}, E.~L. and {Eisenhardt}, P.~R.~M. and {Mainzer}, A.~K. and 
	{Ressler}, M.~E. and {Cutri}, R.~M. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and 
	{Padgett}, D. and {McMillan}, R.~S. and {Skrutskie}, M. and 
	{Stanford}, S.~A. and {Cohen}, M. and {Walker}, R.~G. and {Mather}, J.~C. and 
	{Leisawitz}, D. and {Gautier}, III, T.~N. and {McLean}, I. and 
	{Benford}, D. and {Lonsdale}, C.~J. and {Blain}, A. and {Mendez}, B. and 
	{Irace}, W.~R. and {Duval}, V. and {Liu}, F. and {Royer}, D. and 
	{Heinrichsen}, I. and {Howard}, J. and {Shannon}, M. and {Kendall}, M. and 
	{Walsh}, A.~L. and {Larsen}, M. and {Cardon}, J.~G. and {Schick}, S. and 
	{Schwalm}, M. and {Abid}, M. and {Fabinsky}, B. and {Naes}, L. and 
	{Tsai}, C.-W.},
    title = "{The Wide-field Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit Performance}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1008.0031},
 primaryClass = "astro-ph.IM",
 keywords = {infrared: general, space vehicles, surveys},
     year = 2010,
    month = dec,
   volume = 140,
      eid = {1868},
    pages = {1868-1881},
      doi = {10.1088/0004-6256/140/6/1868},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....140.1868W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE Y 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{yoon_mnras_380_2007,
   author = {{Yoon}, S.-C. and {Podsiadlowski}, P. and {Rosswog}, S.},
    title = "{Remnant evolution after a carbon-oxygen white dwarf merger}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0704.0297},
 keywords = {accretion, accretion discs, stars: evolution, supernovae: general, white dwarfs},
     year = 2007,
    month = sep,
   volume = 380,
    pages = {933-948},
      doi = {10.1111/j.1365-2966.2007.12161.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.380..933Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yoon_apj_717_2012,
   author = {{Yoon}, S.-C. and {Cantiello}, M.},
    title = "{Evolution of Massive Stars with Pulsation-driven Superwinds During the Red Supergiant Phase}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1005.4925},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: massive, stars: mass-loss, supergiants, supernovae: general},
     year = 2010,
    month = jul,
   volume = 717,
    pages = {L62-L65},
      doi = {10.1088/2041-8205/717/1/L62},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...717L..62Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yoon_443_aa_2005,
   author = {{Yoon}, S.-C. and {Langer}, N.},
    title = "{Evolution of rapidly rotating metal-poor massive stars towards gamma-ray bursts}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0508242},
 keywords = {stars: rotation, stars: evolution, stars: Wolf-Rayet, supernovae: general, gamma rays: bursts},
     year = 2005,
    month = nov,
   volume = 443,
    pages = {643-648},
      doi = {10.1051/0004-6361:20054030},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...443..643Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yorke_aa_315_1996,
   author = {{Yorke}, H.~W. and {Welz}, A.},
    title = "{Photoevaporation of protostellar disks. I. The evolution of disks around early B stars.}",
  journal = {\aap},
 keywords = {RADIATION TRANSFER, STARS: CIRCUMSTELLAR MATTER, STARS: FORMATION OF, ISM: JETS AND OUTFLOWS, HII REGIONS},
     year = 1996,
    month = nov,
   volume = 315,
    pages = {555-564},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...315..555Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yusefzadeh_apj_585_2003,
   author = {{Yusef-Zadeh}, F. and {Wardle}, M. and {Rho}, J. and {Sakano}, M.
	},
    title = "{OH (1720 MHz) Masers and Mixed-Morphology Supernova Remnants}",
  journal = {\apj},
   eprint = {astro-ph/0211191},
 keywords = {ISM: Clouds, ISM: General, Shock Waves, ISM: Supernova Remnants, X-Rays: ISM},
     year = 2003,
    month = mar,
   volume = 585,
    pages = {319-323},
      doi = {10.1086/345932},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...585..319Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yu_apj_194_1974,
   author = {{Yu}, G.},
    title = "{The interstellar wake of the solar wind}",
  journal = {\apj},
 keywords = {GAS COOLING, INTERPLANETARY MAGNETIC FIELDS, INTERSTELLAR SPACE, SOLAR WIND, WAKES, HYDROGEN, INTERSTELLAR GAS, INTERSTELLAR MAGNETIC FIELDS, MAGNETIC EFFECTS, MAGNETIC FIELD CONFIGURATIONS, PLASMA DYNAMICS, SHOCK WAVE PROPAGATION, SUBSONIC FLOW},
     year = 1974,
    month = nov,
   volume = 194,
    pages = {187-202},
      doi = {10.1086/153235},
   adsurl = {http://adsabs.harvard.edu/abs/1974ApJ...194..187Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE Z 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{zapata_apj_698_2009,
   author = {{Zapata}, L.~A. and {Ho}, P.~T.~P. and {Schilke}, P. and {Rodr{\'{\i}}guez}, L.~F. and 
	{Menten}, K. and {Palau}, A. and {Garrod}, R.~T.},
    title = "{A Ring/Disk/Outflow System Associated with W51 North: A Very Massive Star in the Making}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0904.0325},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, instrumentation: interferometers, ISM: jets and outflows, molecular data, stars: formation, stars: individual: W51 North W51N},
     year = 2009,
    month = jun,
   volume = 698,
    pages = {1422-1428},
      doi = {10.1088/0004-637X/698/2/1422},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...698.1422Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zanni_aa_469_2007,
   author = {{Zanni}, C. and {Ferrari}, A. and {Rosner}, R. and {Bodo}, G. and 
	{Massaglia}, S.},
    title = "{MHD simulations of jet acceleration from Keplerian accretion disks. The effects of disk resistivity}",
  journal = {\aap},
   eprint = {astro-ph/0703064},
 keywords = {accretion, accretion disks, ISM: jets and outflows, galaxies: jets, magnetohydrodynamics (MHD), methods: numerical},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {811-828},
      doi = {10.1051/0004-6361:20066400},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..811Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zavlin_aa_331_1998,
   author = {{Zavlin}, V.~E. and {Pavlov}, G.~G. and {Trumper}, J.},
    title = "{The neutron star in the supernova remnant PKS 1209-52}",
  journal = {\aap},
   eprint = {astro-ph/9709267},
 keywords = {STARS: NEUTRON, SUPERNOVAE: INDIVIDUAL PKS 1209-52, X-RAYS: STARS, RADIATION MECHANISMS: THERMAL},
     year = 1998,
    month = mar,
   volume = 331,
    pages = {821-828},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...331..821Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zhekov_na_3_1998,
   author = {{Zhekov}, S.~A. and {Myasnikov}, A.~V.},
    title = "{1D gasdynamics of wind-blown bubbles: effects of thermal conduction}",
  journal = {\na},
 keywords = {Hydrodynamics, Conduction, Shock waves, ISM, bubbles, Hydrodynamics, Circumstellar shells, clouds, and expanding envelopes; circumstellar masers},
     year = 1998,
    month = mar,
   volume = 3,
    pages = {57-73},
      doi = {10.1016/S1384-1076(97)00043-2},
   adsurl = {http://adsabs.harvard.edu/abs/1998NewA....3...57Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zinchenko_apj_810_2015,
   author = {{Zinchenko}, I. and {Liu}, S.-Y. and {Su}, Y.-N. and {Salii}, S.~V. and 
	{Sobolev}, A.~M. and {Zemlyanukha}, P. and {Beuther}, H. and 
	{Ojha}, D.~K. and {Samal}, M.~R. and {Wang}, Y.},
    title = "{The Disk-outflow System in the S255IR Area of High-mass Star Formation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1507.05642},
 keywords = {astrochemistry, HII regions, instrumentation: interferometers, ISM: clouds, ISM: molecules, stars: formation},
     year = 2015,
    month = sep,
   volume = 810,
      eid = {10},
    pages = {10},
      doi = {10.1088/0004-637X/810/1/10},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...810...10Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zinnecker_araa_45_2007,
   author = {{Zinnecker}, H. and {Yorke}, H.~W.},
    title = "{Toward Understanding Massive Star Formation}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0707.1279},
     year = 2007,
    month = sep,
   volume = 45,
    pages = {481-563},
      doi = {10.1146/annurev.astro.44.051905.092549},
   adsurl = {http://adsabs.harvard.edu/abs/2007ARA%26A..45..481Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zhu_apj_746_2012,
   author = {{Zhu}, Z. and {Hartmann}, L. and {Nelson}, R.~P. and {Gammie}, C.~F.
	},
    title = "{Challenges in Forming Planets by Gravitational Instability: Disk Irradiation and Clump Migration, Accretion, and Tidal Destruction}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.6943},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, instabilities, planet-disk interactions, planets and satellites: formation, protoplanetary disks},
     year = 2012,
    month = feb,
   volume = 746,
      eid = {110},
    pages = {110},
      doi = {10.1088/0004-637X/746/1/110},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...746..110Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




